Efficient Ranking Function-Based Termination Analysis with Bi-Directional Feedback

Synthesizing ranking functions is a common technique for proving the termination of loops. A ranking function must be bounded and decrease by a specified amount with each iteration for all reachable program states. However, the set of reachable program states is often unknown, and loop invariants are typically used to overapproximate it. So, proving the termination of a loop requires searching for both a ranking function and a loop invariant. Existing ranking function-based termination analysis techniques can be broadly categorized as (i) those that synthesize the ranking function and invariants independently, (ii) those that combine invariant synthesis with ranking function synthesis into a single query, and (iii) those that offer limited feedback from ranking function synthesis to guide invariant synthesis. These approaches either suffer from having too large a search space or inefficiently exploring the smaller, individual search spaces. In this work, we present a novel termination analysis framework Syndicate, which exploits bi-directional feedback to guide the searches for both ranking functions and invariants, increasing the number of programs that can be proven to terminate and reduces the average time needed to prove termination compared to baselines. Syndicate is general and allows different instantiations of templates, subprocedures, and parameters, offering users the flexibility to optimize the ranking function synthesis. Depending on the templates used, Syndicate is relatively complete and efficient, outperforming existing techniques that achieve at most one of these guarantees. Notably, despite a simpler approach compared to the baselines, Syndicate's performance is either comparable to or better than existing tools in terms of the number of benchmarks proved and average runtime.

==> sections/algo-backup.tex <==
\section{Syndicate Framework}
\label{sec:theory}

\subsection{Sound and Complete Algorithm}
\label{sec:main-algorithm}

Let us fix a set of invariants $\tempi$ and set of potential ranking functions $\tempr$. We will assume that $\stat$ (the set of program states) is in $\tempi$ and that $\tempi$ is closed under intersection, i.e., if $\inv_1,\inv_2 \in \tempi$ then $\inv_1 \cap \inv_2 \in \tempi$.
%
Let us also fix a program $\pgm$, a loop $\looppgm = \texttt{while } \beta \texttt{ do } \pgm_1 \texttt{ od}$ inside $\pgm$, and a set of initial states $\ini$. The goal is to synthesize ranking functions from $\tempr$ and invariants from $\tempi$ that demonstrate that every loop inside $\pgm$, including $\looppgm$, terminates. The algorithm must be \emph{sound} and \emph{complete} --- ranking functions and invariants identified must constitute a correct proof of termination, and if there is a proof of termination using invariants in $\tempi$ and ranking functions from $\tempr$ then the algorithm must succeed. We first establish such a result under assumptions about the sets $\tempi$ and $\tempr$ and some computability assumptions about sub-procedures of our main algorithm. We then present algorithms for the sub-procedures that satisfy the computability assumptions needed for the soundness and completeness result.

Our algorithm maintains an annotated program $\annopgm$ of $\pgm$ (i.e., $\core{\annopgm} = \pgm$) that is correct w.r.t the initial set, i.e., $\ini \models \annopgm$. The search for a ranking function to establish the termination of a loop of $\pgm$ leads to a progressive refinement of the invariant annotations in $\annopgm$. Since the invariants in $\annopgm$ progressively become smaller, a ranking function that proves the termination of a loop continues to be sound as the invariants change. This allows one to consider loops in $\pgm$ in any order.

To prove the termination of a single loop in $\pgm$, sample pairs of states from the beginning and end of a loop iteration are used to generate a candidate ranking function $\rf$. Checking the correctness $\rf$ may lead to either the refinement of the loop invariants in $\annopgm$ or the identification of additional pairs of states over which any ranking function must decrease or both. Thus, the algorithm makes progress by either constructing a more precise model for the semantics of the program or by eliminating additional potential ranking functions.
%
To make the above algorithm sketch more concrete, we introduce a partial order ($\less$) and a meet operation ($\meet$) for the set of annotated programs ($\annopgm$).

Let $\annopgm$ be an annotated program such that $\core{\annopgm} = \pgm$. 
We will use $\annopgm[\looppgm]$ to denote an annotated subprogram of $\annopgm$ that corresponds to the loop $\looppgm$ in $\annopgm$. 
For annotated programs $\annopgm_1,\annopgm_2 \in \anno(\pgm)$ (i.e., $\core{\annopgm_1} = \core{\annopgm_2} = \pgm$), we say $\annopgm_1 \less \annopgm_2$ if for each loop in $\pgm$, the invariant annotating this loop in $\annopgm_1$ is contained in the corresponding invariant in $\annopgm_2$; the formal definition is deferred to Appendix~\ref{app:defns}. If $\annopgm_1 \less \annopgm_2$ and $\annopgm_1 \neq \annopgm_2$ then we say $\annopgm_1 \strctless \annopgm_2$. Next, $\annopgm_1 \meet \annopgm_2$ denotes the annotated program where each loop is annotated by the intersection of the invariants annotating the loop in $\annopgm_1$ and $\annopgm_2$.

In Appendix~\ref{appendix:proofs}, we show that if there are two annotated programs $\annopgm_1, \annopgm_2 \in \anno(\pgm)$ such that they are valid w.r.t the initial set, i.e.,  $\ini \models \annopgm_1$ and $\ini \models \annopgm_2$, then the meet of $\annopgm_1$ and $\annopgm_2$ is also valid w.r.t the initial set, i.e., $\ini \models \annopgm_1 \meet \annopgm_2$. Further, if $\annopgm_1$ and a ranking function $\rf$ are valid w.r.t to the initial set, i.e. $\ini \models \annopgm_1, \rf$, and $\annopgm_2$ is a valid annotated program w.r.t $\ini$ and $\annopgm_2 \less \annopgm_1$, then the pair $\annopgm_2, \rf$ is also valid w.r.t $\ini$. This is presented as the following.
\begin{proposition}
\label{prop:correct-refine}
Let $\annopgm_1,\annopgm_2 \in \anno(\pgm)$ be two annotated programs. 
% such that $\annopgm_1 \less \annopgm_2$. Let $\rf$ be a ranking function and let $\inv_1,\inv_2 \subseteq \stat$ be two sets of program states reached at the start of loop $\looppgm$ in $\annopgm_1$ and $\annopgm_2$, respectively, from the initial set $\ini$. Then the following two observations hold.
\begin{enumerate}
\item If $\ini \models \annopgm_1$ and $\ini \models \annopgm_2$, then $\ini \models \annopgm_1 \meet \annopgm_2$.
\item If $\ini \models \annopgm_1$, $\ini \models \annopgm_2,f$ and $\annopgm_1 \less \annopgm_2$, then $\ini \models \annopgm_1,f$.
\end{enumerate}
\end{proposition}
% \begin{proof}[Proof Sketch]
%     (1) This can be proved by induction on the structure of $\pro$, with base case being $\pro = \alpha$, for which $\anno_1 = \anno_2 = \anno_1 \meet \anno_2 = \alpha$. \\
%     Now, say $\pro$ is of the form $\texttt{while}(\beta) \texttt{ do }\annopgm_{11} \texttt{ od}$. \\
%     Let $\annopgm{_1} \equiv \invar_1 \; @ \; \texttt{while}(\beta) \texttt{ do }\annopgm_{11} \texttt{ od}$ \\
%     Let $ \annopgm{_2} \equiv\invar_2 \; @ \; \texttt{while}(\beta) \texttt{ do }\annopgm_{21} \texttt{ od}$ \\
%     $\ini \models \annopgm_1 \implies \ini \subseteq  \invar_1 \; \wedge \; \invar_1 \cap \bracs{\beta} \circ \bracs{\annopgm_{11}} \subseteq  \invar_1 \; \wedge \invar_1 \cap \bracs{\beta} \models \annopgm_{11}$ \\
%      $\ini \models \annopgm_2 \implies \ini \subseteq  \invar_2 \; \wedge \; \invar_2 \cap \bracs{\beta} \circ \bracs{\annopgm_{21}} \subseteq  \invar_2 \; \wedge \invar_2 \cap \bracs{\beta} \models \annopgm_{21}$ \\   
%      Using these and the fact that ($s \models \anno \wedge s' \subseteq s \implies s' \models \anno$, proved in Proof~\ref{aplemma:less}), we get\\
%      $(\ini \subseteq \invar_1 \cap \invar_2) \; \wedge \; (\invar_1 \cap \invar_2 \cap \bracs{\beta} \models \annopgm_{11}) \; \wedge \; (\invar_1 \cap \invar_2 \cap \bracs{\beta} \models \annopgm_{21})$ \\
%      which proves $S \models \anno_1 \meet \anno_2$ from the Inductive Hypothesis.
     
%      The proofs for other cases can be found in Proof~\ref{aplemma:conj}. \\
     
% (2) Let $\annopgm{_1} \equiv \invar_1 \ @ \ \texttt{while }(\beta) \texttt{ do }\annopgm'_1 \texttt{ od}$.\\
% Let $\annopgm{_2} \equiv \invar_2 \ @ \ \texttt{while }(\beta) \texttt{ do }\annopgm'_2 \texttt{ od}$.\\
% $\ini \models \annopgm_2,f \implies \; \forall (s,s') \in \id{\inv_2 \cap \bracs{\beta}}\relcomp\bracs{\annopgm'_2}$, $\rf(s) \geq 0$ and $\rf(s) - \rf(s') \geq 1$\\
% $(\annopgm_1 \less \annopgm_2 \implies \invar_1 \subseteq \invar_2) \; \wedge \; (\annopgm_1 \less \annopgm_2 \implies \annopgm'_1 \less \annopgm'_2 \implies \bracs{\annopgm'_1} \subseteq \bracs{\annopgm'_2})$\\

% From these, it follows that $\id{\inv_1 \cap \bracs{\beta}}\relcomp\bracs{\annopgm'_1} \subseteq \id{\inv_2 \cap \bracs{\beta}}\relcomp\bracs{\annopgm'_2}$ \\
% And so 
% $\forall (s,s') \in \id{\inv_1 \cap \bracs{\beta}}\relcomp\bracs{\annopgm'_1}, \rf(s) \geq 0$ and $\rf(s) - \rf(s') \geq 1$ also holds. This proves that $\ini \models \annopgm_1,f$.

% \end{proof}
% \begin{proof}[Proof Sketch]
% The observations follow from the definitions of correctness.
% \end{proof}

% \begin{lemma}
% \label{ref:help1}
% Let $\annopgm_1,\annopgm_2 \in \anno(\pgm)$. If $\ini \models \annopgm_1$ and $\ini \models \annopgm_2$, then $\ini \models \annopgm_1 \meet \annopgm_2$.
% \end{lemma}

% \begin{lemma}
% \label{ref:help2}
% Let $\annopgm_1,\annopgm_2 \in \anno(\pgm)$. If $\ini \models \annopgm_1$, $\ini \models \annopgm_2,f$ and $\annopgm_1 \less \annopgm_2$, then $\ini \models \annopgm_1,f$.
% \end{lemma}

% \begin{lemma}
% \label{lem:meet}
% Let $\annopgm_1,\annopgm_2 \in \anno(\pgm)$ and $\rf$ be a ranking function. If $\ini \models \annopgm_1$ and $\ini \models \annopgm_2, \rf$ then $\ini \models (\annopgm_1 \meet \annopgm_2), \rf$.
% \end{lemma}
\begin{lemma}
\label{lem:meet}
Let $\annopgm_1,\annopgm_2 \in \anno(\pgm)$ and $\rf$ be a ranking function. If $\ini \models \annopgm_1$ and $\ini \models \annopgm_2, \rf$ then $\exists \anno_3 \less \anno_1$ and $\ini \models \anno_3, \rf$.
\end{lemma}
\begin{proof}
    Consider $\anno_3 = \anno_1 \meet \anno_2 \less \anno_1$. It follows from Proposition~\ref{prop:correct-refine} that $\ini \models \anno_3, f$. 
\end{proof}
% \begin{proof}
%     $\ini \models (\annopgm_1 \meet \annopgm_2)$ follows from lemma~\ref{ref:help1}. As $(\annopgm_1 \meet \annopgm_2) \less \annopgm_2$ and $\ini \models \annopgm_2, \rf$,  $\ini \models (\annopgm_1 \meet \annopgm_2), f$ now follows from lemma~\ref{ref:help2}.
% % \end{proof}

% Proof for Lemma~\ref{lem:meet} follows from Proposition~\ref{prop:correct-refine}.



\myparagraph{\toolname} Let us consider a situation where our algorithm is trying to prove the termination of a loop $\looppgm = \texttt{while } \beta \texttt{ do } \pgm_1 \texttt{ od}$ inside program $\pgm$. The algorithm has an annotated program $\annopgm \in \anno(\pgm)$ such that $\ini \models \annopgm$; this is can be easily achieved by labeling each loop in $\pgm$ with $\stat$, the set of all program states. The algorithm also maintains a finite set $\rp \subseteq \stat \times \stat$ such that for any correct annotation $\annopgm'$ of $\pgm$, $\rp \subseteq \id{\inv'\cap\bracs{\beta}}\relcomp\bracs{\annopgm'[\pgm_1]}$, where $\inv'$ is the annotation of $\looppgm$ in $\annopgm'$. In other words, the pairs in $\rp$ are in the semantics of the loop body $\pgm_1$ of every correct annotation of $\pgm$. We associate with $\rp$ a set of ranking functions ($\func(\rp, \tempr)$) from the template $\tempr$, such that each function of that set is bounded and reduces for all elements in $\rp$, i.e., $\func(\rp, \tempr) \triangleq \setpred{f \in \tempr}{\forall (s, s') \in \rp, f(s) \geq 0 \wedge f(s) - f(s') \geq 1}$. 

The algorithm, shown in Algorithm~\ref{general-algorithm}, iteratively generates a candidate ranking function and then uses it to refine the algorithm state if the candidate ranking function is not valid. Lines 4-9 of Algorithm~\ref{general-algorithm} describe the phase of generating a ranking function. The function $\gc$ picks a ranking function from the set $\func(\rp, \tempr)$, if one exists. The function $\checkr$ (line 10) then checks if $\rf$ is correct for $\annopgm[\looppgm]$. In our implementation, both $\gc$ and $\checkr$ are implemented by reducing it to the satisfiability of a logical formula. We assume that if $\checkr$ fails, $\gcounter$ produces a \emph{counter-example} (line 13). The counter-example is a pair of states $(c,c')$ such that (a) $(c,c') \in \bracs{\annopgm[\pgm_1]}$, (b) $c \in \inv \cap \bracs{\beta}$, where $\inv$ is the invariant labeling $\looppgm$ in $\annopgm$, and (c) either $\rf(c) < 0$ or $\rf(c) - \rf(c') < 1$. 

If $\rf$ is not a valid ranking function for $\looppgm$ then the counter-example $(c,c')$ is used to refine the program state (line 14). The counter-example can be eliminated in one of two ways. Either the invariants in $\annopgm$ are refined so that $c$ is not an entry state of loop $\looppgm$, or $(c,c')$ is not in the semantics of the body $\pgm_1$, or a new ranking function is synthesized that behaves correctly on the pair $(c,c')$. $\s{refine}$ (line 14) tries to eliminate $(c,c')$ by refining the invariants in $\annopgm$. The crucial property we require of $\s{refine}$ is as follows.
\begin{enumerate}
    \item If $\s{refine}(\annopgm,(c,c'),\rp)$ returns $(\true, \annopgm')$ then it must be the case $\annopgm' \strctless \annopgm$ and $\ini \models \annopgm'$.
    \item If $\s{refine}(\annopgm,(c,c'),\rp)$ returns $(\false, \annopgm')$ then $\annopgm' = \annopgm$ and for every correct $\annopgm''$ with $\annopgm'' \strctless \annopgm$, $(c,c') \in \id{\inv'' \cap \bracs{\beta}}\relcomp\bracs{\annopgm''[\pgm_1]}$ where $\inv''$ is the invariant labelling $\looppgm$ in $\annopgm''$. In other words, $(c,c')$ is in the semantics of the body of the loop $\looppgm$ in every refinement of $\annopgm$.
\end{enumerate}
If $\s{refine}$ is unable to refine (case 2 above) then we add $(c,c')$ to the set $\rp$ to get a new set $\rp_{\s{new}}$. We observe that in this case, $\rp_{\s{new}}$ continues to satisfy the property that we required of $\rp$.
%

% \begin{lemma}
%     \label{lem:n1}
%     If $\core{\anno_1} = \core{\anno_2} = \pro$, $\ini \models \anno_1$ and $\ini \models \anno_2$, then $\ini \models (\anno_1 \meet \anno_2)$
% \end{lemma}

\begin{lemma}
    \label{lem:refine}
    Suppose $\s{refine}(\annopgm,(c,c'),\rp)$ returns $(\false, \annopgm)$. Consider any annotated program $\annopgm' \in \anno(\pgm)$ such that $\ini \models \annopgm'$. Let $\inv'$ be the annotation of $\looppgm$ in $\annopgm'$. Then $(c,c') \in \id{\inv'\cap\bracs{\beta}}\relcomp\bracs{\annopgm'[\pgm_1]}$.
\end{lemma}

\begin{proof}
    Suppose the claim is not true, i.e., for some correct annotated program $\annopgm'$, $(c,c') \not\in \id{\inv'\cap\bracs{\beta}}\relcomp\bracs{\annopgm'[\pgm_1]}$. Consider the program $\annopgm \meet \annopgm' \strctless \annopgm$. By Lemma~\ref{lem:meet}, $\annopgm \meet \annopgm'$ is correct and $(c,c')$ is not valid pair for the semantics of the loop body $\pgm_1$. In such a case $\s{refine}$ must return $\true$ giving us the desired contradiction.
\end{proof}

By processing counter-example $(c,c')$, our algorithm always makes progress. There are two cases to consider. If $\s{refine}$ returns $\true$ then we have a new correct annotated program $\annopgm'$ that refines $\annopgm$. On the other hand, if $\s{refine}$ returns $\false$ then we have new set $\rp_{\s{new}}$ with the property that $\func(\rp_{\s{new}},\tempr) \subsetneq \func(\rp, \tempr)$. This is because $\rf \in \func(\rp, \tempr)\setminus\func(\rp_{\s{new}},\tempr)$ since $\rf$ is not a valid ranking function for the pair $(c,c')$. Thus, in this case $\func(\rp_{\s{new}},\tempr)$ has become smaller.

\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-0.5cm}
    \begin{minipage}{\linewidth}
        \begin{algorithm}[H]
            \caption{Termination of Outermost Loop}
            \label{general-algorithm}
            \begin{algorithmic}[1]
                \Procedure{$\mathsf{find\_rank}$}{$\rp, \annopgm$}
                \State $\text{is\_refined} \gets \false$
                    \While{\true }
                        \If{$\neg\text{is\_refined}$}
                            \State $\text{gen},f \gets \gc(\rp)$
                            \If{$\neg \text{gen}$}
                                \State \Return False
                            \EndIf
                        \EndIf
                        \If{$\checkr(f, \anno)$} 
                            \State \Return True
                        \EndIf
                        \State $(c,c') \gets \gcounter(f, \annopgm)$
                        \State $\text{is\_refined}, \; \annopgm \gets \mathsf{refine}(\annopgm, (c,c'), t)$
                        \If{$\neg \text{is\_refined}$}
                            \State $\rp \gets \rp \cup \{c\}$
                        \EndIf
                        % \State \Return $\mathsf{find\_rank}$($\rp, \anno, f, \neg \text{is\_refined}$)
                    \EndWhile 
                \EndProcedure
            \end{algorithmic}
        \end{algorithm}
    \end{minipage}
     \vspace{-0.6cm}
\end{wrapfigure}

% Algorithm~\ref{general-algorithm} can be shown to be sound and complete for proving the termination of loop $\looppgm$ of $\pgm$.
Algorithm~\ref{general-algorithm} can be shown to be sound and complete for proving the termination of loop $\looppgm$ of $\pgm$. In this context, soundness means that if our algorithm returns $\true$, then there exists a ranking function and an invariant in their respective templates that can prove the termination of the program. Conversely, completeness means that if there is a function $f \in \tempr$ and $\invar \in \tempi$ such that $f$ can be proved valid using $\invar$, then Algorithm~\ref{general-algorithm} will prove termination.

\begin{theorem}
    \label{thm:main}
    Suppose there exist effective procedures for the functions $\gc$, $\checkr$, $\gcounter$, and $\s{refine}$. Further, suppose the set $\tempr$ is finite, and $\tempi$ is closed under intersection and has no infinite descending chains (with respect to the subset relation). Then Algorithm~\ref{general-algorithm} is a sound and complete method to prove the termination of loop $\looppgm$ of $\pgm$.
\end{theorem}

\begin{proof}[Proof Sketch]
    Soundness of the algorithm follows from the soundness of $\gc$ and $\checkr$. Suppose there is a ranking function $\rf^*$ and an annotated program $\annopgm^*$ such that $\annopgm^*$ is a correct annotation of $\pgm$ and $\rf^*$ is a valid ranking function that proves the termination of $\looppgm$. Let $(\annopgm,\rp)$ be the state of the algorithm at any point. Observe that because of the property that the algorithm maintains of $\rp$, $\rf^* \in \func(\rp,\tempr)$. By Lemma~\ref{lem:meet} there is a correct annotated program $\annopgm' \less \annopgm$ such that $\rf^*$ proves the termination of $\looppgm$ in $\annopgm'$. Finally, the assumptions on $\tempi$ and $\tempr$ mean that $\func(\rp,\tempr)$ and $\annopgm\downarrow = \setpred{\annopgm'}{\annopgm' \less \annopgm}$ are both finite sets and hence there can only be finitely many steps of refinement. Thus Algorithm~\ref{general-algorithm} will terminate with the right answer.
\end{proof}

A couple of remarks before concluding this section. Since Algorithm~\ref{general-algorithm} is sound and complete to prove the termination of any loop in $\pgm$, it can be used repeatedly for different loops to conclude the termination of $\pgm$. Next, we assumed that the templates used for invariants and ranking functions were the same for every loop. However, the ideas can be seen to easily work even if different invariant sets and ranking functions are used for different loops in the program.


\subsection{Refining Algorithm State}
\label{sec:sub-algorithms}
We will describe procedures for $\gc$, $\checkr$, $\gcounter$, and $\s{refine}$ that satisfy the assumptions needed for soundness and completeness of Algorithm~\ref{general-algorithm}. For these procedures we will use SMT queries to generate and check the soundness of ranking functions for a given loop in a program. We can define $\tempr$ as a finite template for ranking functions. For the function $\gc$, given $t$, we can generate an SMT query encoding a symbolic ranking function in $\tempr$ that satisfies the reducing and bounded conditions of a valid ranking function for all of the pairs of states in $t$. Finding a satisfying assignment to this query is equivalent to finding a candidate ranking function and if there is not satisfying assignment, then there is no ranking function in $\tempr$ that is valid for the the under-approximation, $t$, and, therefore, there is no ranking function in $\tempr$ that is valid for the loop. This follows the semantics of $\gc$ described in Section~\ref{sec:main-algorithm}. For this function to be decidable, one must be able to describe the set of all ranking functions in $\tempr$ and express the bounded and reducing conditions on these ranking functions in a decidable SMT theory. Some examples of templates that lead to the SMT queries being decidable are the set of linear functions over the program variables, the set of polynomial functions over the program variables using real-valued coefficients, and the set of lexicographic functions where each component is a polynomial function using real-valued coefficients.

We can also use an SMT query for a function that implements the semantics of both $\checkr$ and $\gcounter$. $\checkr$ takes as input $f$ and $\anno$. We check the validity of $f$ given $\anno$ using symbolic execution. First, we define a symbolic state at the start of one iteration of the loop, $(x_1, \cdots, x_n)$ and add the condition $(x_1, \cdots, x_n) \in \invar$ where $\invar$ is the invariant of the loop we are analyzing, retrieved from $\anno$. Then, we symbolically execute the loop body using $\anno$.  For each loop in the body of the outer loop, we define new symbolic variables, $(x_{1,j}, \cdots, x_{n,j})$ to represent the state at the exit of the inner loop, adding the condition $(x_{1,j}, \cdots, x_{n,j}) \in \invar_i \cap \llbracket \neg \beta_i \rrbracket$, where $\invar_i$ and $\beta_i$ are the invariant and loop guard of the inner loop from $\anno$. We define symbolic variables representing the state at the end of the iteration, $(x'_1, \cdots, x'_n)$ and set these symbolic variables equal to the output of symbolically executing the loop body on $(x_1, \cdots, x_n)$. Checking the validity of $f$ using $\anno$ is reduced to determining the satisfiability of the formula: $ (f((x_1, \cdots, x_n))-f((x'_1, \cdots, x'_n)) \le 0) \vee (f((x_1, \cdots, x_n)) < 0) $. If this formula is unsatisfiable, then we have proven the validity of $f$ because we have established that $f$ is bounded and reducing on possible state of the loop. If this formula is unsatisfiable, we return True. Otherwise, we return False. In Algorithm~\ref{general-algorithm}, $\gcounter$ is only called when $\checkr$ returns False. In this case, from the SMT query in $\checkr$, we have a satisfying assignment to $(x_1, \cdots, x_n)$ and $(x'_1, \cdots, x'_n)$. The counter-example, $(c,c')$, returned by $\gcounter(f, \anno)$ is  $(x_1, \cdots, x_n),(x'_1, \cdots, x'_n))$. For this algorithm to be decidable, the SMT encoding of the program has to fit into a decidable SMT theory.


We will now describe an algorithm that implements the semantics of the $\s{refine}$ function and follows the properties defined in Section~\ref{sec:main-algorithm}. Since we defined $\checkr$ to symbolically execute $(x_1, \cdots, x_n)$ by defining symbolic states,$(x_{1,j}, \cdots, x_{n,j})$, at the end of each inner loop, instead of only storing $(c,c')$,  $\checkr$ can store $(c_1, \cdots, c_m)$, where $c_1 = c$, $c_m = c'$ and $c_j = (x_{1,j}, \cdots, x_{n,j})$ for all $j \in [1,m]$. This sequence of states will be used to define $\s{refine}$, shown in Algorithm~\ref{algorithm1}.

First, we will define how the $\s{refine}$ function works when considering one non-nested loop and then we will extend it to loops with arbitrary nesting. When refining the invariant for a non-nested loop given a candidate ranking function, $f$, and a counter-example, $(c,c')$, for $f$ to be a valid ranking function, $c$ has to not be a reachable state the beginning of one iteration of the outer loop. In our algorithm state, for a non-nested loop, we have an annotated program with one invariant, $\inv$. First we try to refine $\invar$ to $\invar'$ s.t. $\invar' \subseteq \invar \setminus \{c\}$. For this, we first try to find an invariant, $\invar''$, that is a valid invariant and excludes the state $c$ and if this is possible, we return $\invar \cap \invar''$. Note that $\invar \cap \invar'' \in \tempi$ because the $\tempi$ is closed under intersection and $\invar \cap \invar'' \subseteq \invar \setminus \{c\}$. To find $\invar''$, we iteratively generate possible invariants and then check the validity of them until either we have found a valid invariant that excludes $c$ or proved that no such invariant exists. We show this procedure in Algorithm~\ref{algorithm1}. In lines 4 and 15, we generate new possible invariants. In line 6, we check the validity of the invariant. In lines 10-14, based on the output of the validity check we update the information used to generate new invariants.

To generate a possible invariant that excludes $c$, we want to generate a set from $\tempi$ that excludes $c$ and includes the states we know are reachable, $\dom(t)$. After we generate a possible invariant, $\invar_1$,  we check whether it includes $\ini$ and is inductive.  If $\invar_1$ does not include $\ini$, we obtain a state, $c'' \in \ini$, s.t. $c'' \notin \invar_1$. When we generate the next possible invariant, $\invar_2$, we add the condition $c'' \in \invar''$. This condition is added by adding $c''$ to $r$. If, on the other hand, $\invar'$ is not inductive, we obtain a counter-example, $(c''_1,c''_2)$ s.t. $c''_1 \in \invar_1 \wedge c''_2 \notin \invar_1$ and $c''_2$ is the state after executing the loop body on the state $c''$. In this case, to ensure we generate a different possible invariant, $\invar_2$, we add the condition $c''_1 \in \invar_2 \implies c''_2 \in \invar_2$. Note that the conditions we add in each iteration of generating possible invariants are true for all valid invariants of a loop.

For nested loops, we try to eliminate one state, $c_i$ for $i \in [1,m]$, from the invariant at the program point corresponding to $c_i$. To accomplish this, we can start with $c_m$ and use the algorithm for $\s{refine}$ for non-nested loops to either exclude $c_m$ from $\invar_m$ or return False. If refining $\invar_m$ fails, we can move on to $\invar_{m-1}$ and try to refine it to exclude $c_{m-1}$. 

Formally, we use $r$ to represent an under-approximation of the reachable states at the beginning of the loop and $inv_c$ to represent the set of pairs of states we obtained as counter-examples in previous iterations of checking the validity of possible invariants.
Initially, $r$ is set to the domain of $t$ since we know these are all reachable states and $inv_c$ is set to an empty set. Then, we use the following SMT query to find a candidate for $\invar''$:

   $$\Big( s_d \notin \invar'' \Big) \wedge \Big( \bigwedge_{s \in r} s \in \invar'' \Big) \wedge\Big( \bigwedge_{(s,s') \in inv_c} s \in \invar'' \implies s' \in \invar'' \Big)$$ 

To check the validity of the candidate invariant, we use the following SMT query:
$$\Big( s \in \ini \cdot s \notin \invar'' \Big) \vee \Big( s \in \invar'', \llbracket \prog \rrbracket s \notin I'' \Big)$$
$\ini$ is the set of states that are reachable after executing the code before the loop and $\prog$ is the body of the loop. 
% In this query, the symbolic variables are the program variables in $s$. $\invar''$ is the candidate invariant we generated and since there is no loop in $\prog$, we can symbolically execute $\prog$. 
The first condition is satisfiable iff there is a state reachable before the loop that is not included in $\invar''$. The second condition is satisfiable iff $\invar''$ is not inductive. If this query is unsatisfiable, then $\invar''$ is a valid invariant. In this case, we refine $\invar$ to $\invar' = \invar \cap \invar''$ (line 6 in Algorithm~\ref{algorithm1}).

If the SMT query checking the validity of $\invar''$ is satisfiable, $\gcounterinv$ either returns a state $c''$ that is part of the initially reachable states and not in $\invar''$ or returns a pair of states $c''_1,c''_2$ where $c''_1 \in \invar'' \wedge c''_2 \notin I''$ and $c''_2 = \llbracket \prog \rrbracket c''_1$. In the former case, we add this state to $r$ (line 11). In the latter case, we add this state to $inv_c$ (line 13). This ensures that in future iterations of generating possible invariants within the Refine Phase, we will never generate the same invariant twice. With updated $r$ and $inv_c$, we repeat the process of generating and checking a new possible invariant. This process always terminates because we cannot output the same candidate invariant twice and the template we use is finite.

\textbf{Nested Loops} In the case of nested loops, we need to find $\anno' < \anno$, where $\anno$ is the annotated loop program in our algorithm state. 
As discussed earlier, in this instantation of our framework, $\checkr$ will return $(c_1, \cdots, c_m)$ instead of only $(c,c')$. So, we have counter-examples, $c_j$, for each invariant, $\invar_j$, in the program. For each invariant, we maintain the set, $r_j$ and $inv_{c_j}$. $r_j$ is initialized to the set of states after the loop associated with $\invar_j$ obtained for the initial program execution traces and $inv_{c_j}$ is initialized to an empty set. We use an SMT query to generate a candidate invariant, $\invar'_j$ for one of the loops in the doubly annotated program $\annoc$ that excludes the counter-example, $c_j$ associated with $\invar_j$. Formally, we find a satisfying assignment to the constants in $\invar'_j$ for some $j$ such that 
$$\bigvee_j \Big( \neg c_j \in \invar_j \wedge \bigwedge_{s \in r_j} s \in \invar_j \wedge (\bigwedge_{(s,s') \in inv_{c_j}} s \in \invar_j \implies s' \in \invar_j ) \Big) $$
Once we find candidate invariants for all of the loops such that for one of the loops $\invar'_j$ excludes $c_j$, we check the validity of $\invar'_j$ for the loop associated with $\invar_j$. This validity check is done the same way as in the single loop case, and the counter-examples are either added to $r_j$ or $inv_{c_j}$ accordingly. We repeatedly generate candidates to refine at least one of the invariants until one is found or there does not exist any valid invariant for any of the loops that exclude the corresponding counter-example, $c_j$. In the latter case, we have shown that there is a sequence of reachable states w.r.t. the corresponding invariant templates that transition from $c$ to $c'$. Therefore, $(c,c')$ is in the semantics of the body of the loop for every possible refinement of $\anno$. In this case, we return False. This process always terminates because, similar to the single loop case, we can never output the same candidate invariant for the same loop and there are a finite number of invariants in each invariant template and a finite number of loops.

For the SMT queries that generate invariants that are true on $t$ and not true on $c_i$, one must be able to describe the set of all invariants in $\tempi$ and express whether an invariant includes a state in a decidable SMT theory. For the SMT queries that check the validity of invariants at a point in the program to be decidable, the SMT encoding of the program has to fit into a decidable SMT theory.

\begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-1.3cm}
    \begin{minipage}{\linewidth}
        \begin{algorithm}[H]
    \centering
    \caption{Algorithm for Refine State}\label{algorithm1}
    \begin{algorithmic}[1]
\Procedure{$\mathsf{refine}$}{$\anno, (c, c'), t$}
    \State $\mathsf{inv_c}$ = []
    \State $r = \dom(\rp)$ 
    \State $\anno', \text{gen} \gets \gi(r, (c, c'), \mathsf{inv_c})$
    \While{\text{gen}}
        \If{$\checki(\anno')$} 
            \State \Return True, $\anno \meet \anno'$
        \EndIf
        \State $c'', \mathsf{for\_pre} \gets \gcounterinv(\anno')$
        \If{$\mathsf{for\_pre}$}
            \State $r \gets r \cup \{c''\}$
        \Else
            \State $\mathsf{inv_c} \gets \mathsf{inv_c} \cup \{c''\}$ 
        \EndIf
        \State $\anno', \text{gen} \gets \gi(r, (c, c'), \mathsf{inv_c})$
    \EndWhile
    \State \Return False, $\anno$
\EndProcedure
\end{algorithmic}
\end{algorithm}
    \end{minipage}
    \vspace{-1cm}
\end{wrapfigure}


\begin{theorem}
    \label{thm:main}
    If the set $\tempr$ is finite, and $\tempi$ is closed under intersection and has no infinite descending chains (with respect to the subset relation), and the SMT queries described in Section~\ref{sec:sub-algorithms} fit into a decidable SMT theory, then Algorithm~\ref{general-algorithm} is a sound and complete method to prove the termination of loop $\looppgm$ of $\pgm$.
\end{theorem}

\rmv{
\vspace*{0.5in}
\textbf{OLD SECTION. NEEDS TO BE REMOVED AFTER THE STUFF HAS BEEN REWRITTEN.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
    \centering
    \begin{subfigure}{\textwidth}
        $
        \begin{array}{c}
            % \hspace{3cm}
            \inferrule*[lab={\footnotesize{\textsc{Atomic statements}}}]
            {
            % \consume{c, \alpha} = c'
            }
            {
            \alpha \lessi \alpha 
            } 
            \hspace{1cm}
            \inferrule*[lab={\footnotesize{\textsc{Loop}}}]
            {
            \invar_1 \subseteq \invar_2 \quad 
            \anno'_1 \lessi \anno'_2
            }
            {
            \Big(\invar_1 \ @ \ \texttt{while}(\beta) \texttt{ do }\anno'_1 \texttt{ od }\Big) \lessi \Big(\invar_2 \ @ \ \texttt{while}(\beta) \texttt{ do }\anno'_2 \texttt{ od }
            \Big)} 
            \\\\ 
            \inferrule*[lab={\footnotesize{\textsc{Sequence}}}]
            {
            \anno'_1 \lessi \anno'_2 \quad
            \anno''_1 \lessi \anno''_2
            }
            {
            \anno'_1 ; \anno''_1 \lessi \anno'_2 ; \anno''_2
            } 
            \hspace{1cm}
            \inferrule*[lab={\footnotesize{\textsc{If}}}]
            {
            \anno'_1 \lessi \anno'_2 \quad
            \anno''_1 \lessi \anno''_2
            }
            {
            \Big(\texttt{if}(\beta) \texttt{ then } \anno'_1 \texttt{ else }\anno''_1\Big) \lessi \Big(\texttt{if}(\beta) \texttt{ then } \anno'_2 \texttt{ else }\anno''_2
            \Big)} 
        \end{array}
    $
    \caption{$\anno_1 \lessi \anno_2$}
    \label{fig:annoless}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\textwidth}
        \resizebox{\textwidth}{!}{
    $
        \begin{array}{c}
            % \hspace{3cm}
            \inferrule*[lab={\footnotesize{\textsc{Atomic statements}}}]
            {
            % \consume{c, \alpha} = c'
            }
            {
            \alpha \meeti \alpha = \alpha  
            } 
            \hspace{1cm}
            \inferrule*[lab={\footnotesize{\textsc{Loop}}}]
            {
            \invar = \invar_1 \cap \invar_2 \quad 
            \anno = \anno'_1 \meeti \anno'_2
            }
            {
            \Big(\invar_1 \ @ \ \texttt{while}(\beta) \texttt{ do }\anno'_1 \texttt{ od }\Big) \meeti \Big(\invar_2 \ @ \ \texttt{while}(\beta) \texttt{ do }\anno'_2 \texttt{ od}\Big) = \\\\
            \invar \ @ \ \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od }
            } 
            \\\\ 
            \inferrule*[lab={\footnotesize{\textsc{Sequence}}}]
            {
            \anno' = \anno'_1 \meeti \anno'_2 \\\\
            \anno'' = \anno''_1 \meeti \anno''_2
            }
            {
            \anno'_1 ; \anno''_1 \meeti \anno'_2 ; \anno''_2 = \anno' ; \anno''
            } 
            \hspace{1cm}
            \inferrule*[lab={\footnotesize{\textsc{If}}}]
            {
            \anno' = \anno'_1 \meeti \anno'_2 \quad
            \anno'' = \anno''_1 \meeti \anno''_2
            }
            {
            \Big(\texttt{if}(\beta) \texttt{ then } \anno'_1 \texttt{ else }\anno''_1 \Big)\meeti \Big(\texttt{if}(\beta) \texttt{ then } \anno'_2 \texttt{ else }\anno''_2\Big) = \\\\
            \texttt{if}(\beta) \texttt{ then } \anno' \texttt{ else }\anno''
            } 
        \end{array}
    $
    }
    \caption{$\anno_1 \meeti  \anno_2$}
    \label{fig:annomeet}
    \end{subfigure}
    \caption{Main caption for the entire figure}
    \label{fig:anno}
\end{figure}

% \begin{definition}
%     An invariant template $\tempi$ is a given set of candidate invariants.
% \end{definition}

% \begin{definition}
%     A ranking function template $\tempr$ is a given set of candidate ranking functions.
% \end{definition}
In this algorithm, we work with invariants that are elements of a predetermined set, denoted as $\tempi$. This set (or template) is fixed before starting the algorithm.
% For instance, in the running example from Section~\ref{sec:overview}, the template was the invariants that can be represented as a conjunction of constraints of the form $d_0 + \sum_id_ix_i \ge 0$ where $x_i$ are the program variables and $d_i \in \mathbb{Z}$. 

Given a program, $\prog$ and a template of invariants, $\tempi$, we define a meet semi-lattice, $\lati(\prog, \tempi) = \langle \anno(\prog), \lessi, \meeti \rangle$, over the set of annotated programs $\anno(\prog)$ s.t. $\forall \anno \in \anno(\prog) \cdot \core{\anno} = \prog$ and the annotated invariants $\invar \in \tempi$. The meet and ordering $(\meeti, \lessi)$ are defined in Figure~\ref{fig:anno}.

% Given two candidate invariants, $\invar_1$ and $\invar_2$, we  define a relation, $\preceq_{\invar}$, such that $\invar_1 \preceq_{\invar} \invar_2 \triangleq \invar_1 \subseteq \invar_2$. This defines a partial order over $\tempi$. We also define an operation, $\wedge_{\invar}$, over the two invariants as $\invar_1 \wedge_{\invar} \invar_2 \triangleq \invar_1 \cap \invar_2$. This gives us a semi-lattice over $\tempi$. When we are analyzing nested loops, we define a lattice over $\tempi^1 \times \cdots \times \tempi^n$, where $\tempi^i$ is the template of invariants for the $i$-th loop. For two elements of this lattice, $(\invar_1^1, \cdots, \invar_1^n), (\invar_2^1, \cdots, \invar_2^n)$, $(\invar_1^1, \cdots, \invar_1^n) \preceq_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq \bigwedge_i \invar_1^i \subseteq \invar_2^i$ and $(\invar_1^1, \cdots, \invar_1^n) \wedge_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq (\invar_3^1, \cdots, \invar_3^n)$ where $\invar_3^i \triangleq \invar_1^i \cap \invar_2^i$.

% \begin{definition}
%     $\lati$ is a meet semi-lattice such that $\lati = (\anno, \preceq_{\invar}, \wedge_{\invar})$, where 
%     % $(\invar_1^1, \cdots, \invar_1^n) \preceq_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq \bigwedge_i \invar_1^i \subseteq \invar_2^i$ and $(\invar_1^1, \cdots, \invar_1^n) \wedge_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq (\invar_3^1, \cdots, \invar_3^n)$ where $\invar_3^i \triangleq \invar_1^i \cap \invar_2^i$
% \end{definition}

Similarly, the algorithm also takes as input a template of candidate ranking functions, $\tempr$. We only analyze ranking functions from this template. Formally, $\tempr$, is a set of functions $f: S \rightarrow \mathbb{R}$. For instance, in the example in Section~\ref{sec:overview}, we use the set of functions of the form $\max(a_0 + \sum_i a_ix_i,0) + \max(b_0 + \sum_i b_ix_i,0)$ where $x_i$ are the program variables and $a_i,b_i \in \mathbb{Z}$.

Given a template of ranking function, $\tempr$, we define a meet semi-lattice over of the powerset of $\tempr$, i.e., $\latr(\tempr) = \langle \power(\tempr), \lessr, \meetr \rangle$. 
Given two sets, $F_1, F_2 \in \mathcal{P}(\tempr)$, $F_1 \lessr F_2 \triangleq F_1 \subseteq F_2$, and $F_1 \meetr F_2 \triangleq F_1 \cap F_2$. 
 
% \begin{definition}
%     $\latrfs$ is a meet semi-lattice on  $\mathcal{P}(\tempr)$: $\latrfs = (\mathcal{P} ({\tempr})\preceq_{F}, \wedge_{F})$, where $\mathcal{F}_1 \preceq_{F} \mathcal{F}_2 \triangleq \mathcal{F}_1 \subseteq \mathcal{F}_2$ and $\mathcal{F}_1 \wedge_{F} \mathcal{F}_2 \triangleq \mathcal{F}_1 \cap \mathcal{F}_2$
% \end{definition}

To avoid clutter, we use $\meet$ for both $\meeti$ and $\meetr$, and similarly, we use $\less$ for both $\lessi$ and $\lessr$. The reader can disambiguate based on context.

\textbf{Reachability w.r.t. Template:} 
Given a set of initial states, $\ini$, the set of reachable states $\reach$ at the beginning of a loop program $L$ is defined in Definition~\ref{def:bgroundreach}. 
The set of reachable program states at a point is canonical to the strongest invariant at that point.  
Since all our invariants are restricted to the template $\tempi$, we introduce the notion of $\reach(\prog, \tempi)$ as the set of all reachable states \textit{w.r.t the template $\tempi$}. 
Consider, $\tempi' \subseteq \tempi$, which is the set of all valid invariants w.r.t the program $\prog$ in $\tempi$. We define the set of reachable states w.r.t $\tempi$ as $\reach(\prog, \tempi) = \bigcap \tempi'$.

\begin{definition}
    \label{def:rp}
    For an initial set of states $\ini$, a loop program $L$ and a template of invariants $\tempi$, the set of reachable states of w.r.t $\tempi$ is defined as $$\reach(\ini, L, \tempi) \triangleq \bigcap \Big(\{\bracs{\anno_i} \ | \ \core{\anno_i} = L \text{ and } \ini \models \anno_i \}\Big)$$
\end{definition}

% Consider a program, $P$, \texttt{while $B_1$ do $P_1$ while $B_2$ do $P_2$ od $P_3$ od } where $P_1,P_2,P_3$ are loop-free. If we have invariants, $I_1$ and $I_2$ are invariants for the outer and inner loop respectively. 
% Consider $\trans' = I'_1 \circ P_1 \circ (I_2 \times  I_2) \circ P_3 $, where $I'_1 = \{ (X,X) \ | \ X \in \invar_1 \}$. Observe that the relation $\trans'$ over-approximates the transition relation induced by the program $P$. 
% Similarly, given any program, if we abstract all the loops in the program with their respective invariants, the transition system of the program can be over-approximated by the relation defined by the loop-free parts of the program and the invariants corresponding to the loops. 
% So, at each step of our algorithm, 

\subsection{Algorithm State}
Given a loop program $(L = \texttt{while}(\beta) \texttt{ do }\pro \texttt{ od})$ and an initial set of states, $\init$, we try to find a ranking function and an invariant that can prove its termination. We fix the template of invariants $\tempi$ and ranking functions $\tempr$ before executing the algorithm.
At each step of our algorithm, the state is given by a subset of the exact transition relation $\rp$ ($\rp \subseteq \bracs \pro$), and an annotated program $\anno$ s.t. $\core{\anno} = L$ and $\ini \models \anno$. We associate with $\rp$ a set of ranking functions ($\func(\rp, \tempr)$) from the template $\tempr$, s.t. each function of that set is bounded and reduces for all elements in $\rp$, i.e., $\func(\rp, \tempr) \triangleq \{f \in \tempr \ | \ \forall (s, s') \in \rp, f(s) \geq 0 \wedge f(s) - f(s') \geq 1\}$. So, at each step of the algorithm, we are at a point in the lattice $\latr(\tempr)$ given by $\func(\rp, \tempr)$. Also, in the lattice $\lati(L, \tempi)$, we are at $\anno$.

\subsection{Iterative Algorithm Step}

% \begin{wrapfigure}{l}{0.3\textwidth}
% \small 
% \begin{algorithm}[H]
%     \centering
%     \caption{Full Algorithm}\label{algorithm}
%     \begin{algorithmic}[1]
% \Procedure{$\mathsf{find\_rank}$}{$\rp, \anno$}
%     \State $\text{gen},f \gets \gc(\rp)$
%     \If{$\neg \text{gen}$}
%         \State \Return False
%     \EndIf
%     \If{$\checkr(f, \anno)$} 
%         \State \Return True
%     \EndIf
%     \While{$\true$}
%         \State $(c,c') \gets \gcounter(f, \anno)$
%         \State $\text{is\_refined}, \; \anno \gets \mathsf{refine}(\anno, (c,c'), t)$
%         \If{$\text{is\_refined}$}
%             \If{$\checkr(f, \anno)$} 
%                 \State \Return True
%             \EndIf
%         \Else
%             \State $\rp \gets \rp \cup \{c\}$
%             \State \Return $\mathsf{find\_rank}(\rp_{new}, \; \anno)$ 
%         \EndIf
%     \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-1.3cm}
    \begin{minipage}{\linewidth}
        \begin{algorithm}[H]
            \caption{Termination of Outermost Loop}
            \label{general-algorithm}
            \begin{algorithmic}[1]
                \Procedure{$\mathsf{find\_rank}$}{$\rp, \annopgm$}
                \State $is\_updated \gets \true$
                    \While{\true }
                        \If{$\text{is\_updated}$}
                            \State $\text{gen},f \gets \gc(\rp)$
                            \If{$\neg \text{gen}$}
                                \State \Return False
                            \EndIf
                        \EndIf
                        \If{$\checkr(f, \anno)$} 
                            \State \Return True
                        \EndIf
                        \State $(c,c') \gets \gcounter(f, \annopgm)$
                        \State $\text{is\_refined}, \; \annopgm \gets \mathsf{refine}(\annopgm, (c,c'), t)$
                        \If{$\neg \text{is\_refined}$}
                            \State $\rp \gets \rp \cup \{c\}$
                        \EndIf
                        % \State \Return $\mathsf{find\_rank}$($\rp, \anno, f, \neg \text{is\_refined}$)
                    \EndWhile 
                \EndProcedure
            \end{algorithmic}
        \end{algorithm}
    \end{minipage}
    % \vspace{-0.5cm}
\end{wrapfigure}
Our algorithm iteratively performs the generate candidate phase and a refine state phase, where we first try to generate a candidate ranking function, and then try to refine our algorithm state. We execute these steps alternatively until we find a valid ranking function. In the following, we present details of these steps and show that at each refine step, we move downwards in one of the two semi-lattices. 

% Given a loop with loop-free body, $P$, our algorithm has a state $\langle \rp, \invar \rangle$. $\rp$ is an under-approximation of $\llbracket P \rrbracket$ initialized from a set of execution traces of $P$ and $\invar$ is an over-approximation of $\reachp$ initialized with \true.  Then, we iteratively perform the Generate Candidate phase and the Refine State.


% To prove termination, we have to find a valid ranking function and an invariant. Given a transition relation for a loop, $t \subseteq \trans$ where $dom(t) \in \reach$, $F_{\tempr}(t)$ contains all of the ranking functions in $\tempr$ that satisfy the necessary condition for being valid w.r.t. $dom(t), t$. Therefore, if a ranking function that is valid w.r.t. $\reach, \trans$ exists, then it has to be in $F_{\tempr}(t)$. According to the definitions above, as we go down in $\latr$, the elements of $\mathcal{P}(\tempr)$ shrink, thereby reducing the search space for a valid ranking function. As we add elements to $t$, we create a more precise under-approximation of $\reach$, and $F_{\tempr}(t)$ goes down in $\latr$. Similarly, as we go down in  $\lati$ while also maintaining the validity of the invariant, the invariant keeps getting stronger, which creates a better over-approximation of $\reach$. 

% Now, we will present the algorithm and explain how it goes down in $\latr$ and $\lati$.



 % Given a transition relation, $t \subseteq S \times S$, we define $F_{\tempr}(t)$ as the set of functions, $f \in \tempr$, such that $t \subseteq sat(f)$. 

 %    $$F_{\tempr}(t) = \{f \in \tempr \ | \  \forall (x,x') \in t, f(x) - f(x') \ge 1 \wedge f(x) \ge 0 \wedge f(x') \ge 0 \}$$
 

\noindent
\textbf{Generate Candidate Phase. }
This phase is shown in lines 2-10 of Algorithm~\ref{general-algorithm}.
If $\func(\rp, \tempr)$ is empty, there is no valid ranking function in $\tempr$. Otherwise, we choose an element, $f \in \func(\rp, \tempr)$. Then, we check the validity of $f$ using $\ini \models \anno, f$. We do this by 
symbolic variables to represent the state at the beginning of the loop ($s$). Then we symbolically execute the loop body for all constructs other than a \texttt{while} construct. This is because we cannot simply execute any loop symbolically because the number of iterations that we need to execute is unknown. So, we declare new symbolic variables at the end of each loop body which represent the output of the loop, and assume that the symbolic program state satisfies the invariant at that loop, but the loop guard is false. This gives us a doubly-annotated program $\annoc$, where each loop is associated with an invariant and a symbolic program state. Using these symbolic variables, and symbolic execution, we compute the program state ($s'$) at the end of one iteration of the loop body of $L$. Then, we check if there exists a state $s \in \invar \cap \bracs{\beta}$ for the query:
\begin{equation}
\label{eq:query1}
    \neg \Big( \big(f(s) - f(s') \geq 1\big) \wedge \big(f(s) \geq 0 \big)\Big)
\end{equation}
% by translating it into an SMT query. We define symbolic variables to represent the state at the beginning of the loop and symbolically execute the loop body $P$ to obtain the program state at the end of the loop, $X'$. 
If $f$ is valid w.r.t. $\invar, \trans$, we have proved that the loop terminates. If the validity check fails, we continue to the Refine Phase with a counter-example $(c, c')$.

\noindent
\textbf{Refine State Phase. } 
This phase is shown in lines 11-15 of Algorithm~\ref{general-algorithm}.
We come to this phase if we get an assignment $c, c'$ to $X$ and $X'$ respectively in the Query~\ref{eq:query1}. Since the query is generated in terms of the symbolic variables at each loop, we will get assignments to all the intermediate symbolic variables. So, we get a doubly-annotated program $\annoc$ s.t. $\consume{c, \annoc} = c'$ and $\ini \models \annoc$, where $\consume{c, \annoc}$ is defined as:
\begin{align*}
    \consume{c, \alpha} &\triangleq \bracs{\alpha} c \\ 
    \consume{c, \invar \ @ \ \texttt{while}(\beta) \texttt{ do }\annoc \texttt{ od } c'} &\triangleq c' \text{ if }(c \in \invar) \wedge (c' \in \invar \cap \bracs{\neg \beta})\\
    \consume{c, \annoc_1 ; \annoc_2} &\triangleq \consume{\consume{c, \annoc_1}, \annoc_2} \\
    \consume{c, \texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2} &\triangleq \left\{ \begin{array}{rcl}
        \consume{c, \annoc_1} & \text{if } c \in \bracs{\beta} \\
        \consume{c, \annoc_2} &  \text{otherwise} 
        \end{array}\right. 
\end{align*}
% We obtain $c$ where $c \in \invar$ as a counter-example to $f$ from the validity check presented above. So, $c$ is a program state such that 
% \begin{equation} \Big(f(c) - f( \llbracket P \rrbracket c) < 1 \Big) \vee \Big( f(c) < 0 \Big) \end{equation}
At this step, there may be two cases - (i) the counter-example was spurious, i.e., the counter-example is not reachable w.r.t $\tempi$, but the invariants in $\anno$ were not strong enough to remove it, (ii) the ranking function is incorrect. So, we first try to refine the annotated program $\anno$. If we cannot refine, then the counter-example is added to $\rp$. 
% Using $c$, we check if there is a valid invariant, $\invar' \in \tempi$, which is stronger than $\invar$ and excludes $c$. If $\invar'$  exists, we can refine $\invar$ to $\invar'$. Otherwise, we cannot refine $\invar$.
\begin{equation}
\label{eq:refine-sem}
    % \refine(\ini, (c,c'), \alpha) &\triangleq \false, \alpha \\
    \refine(\ini, (c,c'), L)  \triangleq \left\{ \begin{array}{rcl}
        \true, L' & \text{where } (L' \prec L ) \wedge (\ini \models L')\\
        \false, L & \text{if } \exists \annoc \cdot \core{\annoc} = L \wedge \consume{c, \annoc} = c' \ \wedge \  \not\exists L' \cdot L' < \annoc
        \end{array}\right. \\
\end{equation}
 % If we find $\invar'$, then the algorithm state is updated to $\langle \rp, \invar' \rangle$. If there is no such invariant, then the algorithm state is updated to $\langle \rp \cup \{c\}, \invar \rangle$.

% \end{enumerate}

% When considering nested loops, first we prove the termination of the innermost loop, which results in $f$ and $\invar$, a ranking function and invariant for the innermost loop. We do not need to store the ranking function, but we store $\invar$. We keep doing this recursively. So, when proving the termination of a loop with a body, $P$, that has $n-1$ nested loops, we will get $n-1$ invariants as an output of proving their individual terminations, $\overline{\invar}_2, \cdots, \overline{\invar}_n$. Instead of $\langle \rp, \invar \rangle$, our program state will be  $\langle \rp, \invar^{\dagger} \rangle$ where $\invar^{\dagger} = (\invar_1, \cdots, \invar_n)$ and $\invar_i$ is an invariant for the $i$-th loop. It is initialized $\langle \true, \overline{\invar}_2, \cdots, \overline{\invar}_n \rangle$. Now, we will explain the 2 phases for handling nested loops:
% \begin{enumerate}
%     \item \textbf{Generate Candidate Phase:} A candidate ranking function, $f$, is generated in the same way as in the case of a single loop. However, for the validity check, we cannot simply symbolically execute the body of the loop. This is because although all of the inner loops terminate, we do not know the number of iterations that they run for. As shown in Section~\ref{sec:background}, from a program and invariants for the loops in a program, we can over-approximate $ \llbracket P \rrbracket X $. To achieve this, we declare a new symbolic program state, $X_i$, as an output to each inner loop and assume that $X_i \in \invar_i$ 
%     % Here, we choose an arbitrary element from $F_{\tempr}(\rp)$ as a candidate ranking function. If $F_{\tempr}(r^{\dagger})$ is empty, then the algorithm terminates concluding that there is no ranking function in $\tempr$ w.r.t. an invariant in $\tempi, \llbracket P \rrbracket X$.
%     % Since all the $\invar_i$ are not guaranteed to be the strongest invariants of their respective loops, we do not have the exact representation of $ \llbracket P \rrbracket X $. However, 
%      Then, we check the validity of $f$. Again, if the validity is proven, the algorithm has proved termination, and otherwise, the algorithm proceeds to the Refine State Phase. 
    
%     \item \textbf{Refine State Phase:} We obtain a counter-example, $c^{\dagger} = (c_1,\cdots, c_n)$, from the validity check. $c_1$ is a program state at the beginning of the outermost loop and each $c_i$ is a program state at the end of the $i$-th loop. Using $c_n$, we can compute $c'_1$, which is a program state at the end of the outermost loop. 
%     \begin{equation}
%         \Big( f(c_1) - f(c'_1) < 1 \Big) \vee \Big( f(c_1) < 0 \Big)
%     \end{equation}
    
%     We use this counter-example to refine $\idd$ to an invariant, $\idd_{new} \in \tempi^1 \times \cdots \times \tempi^n$ $\idd_{new} = (\invar'_1, \cdots, \invar'_n) = refine(\idd, c^{\dagger} )$ and has the following property:
%     \begin{equation}
%     \label{eq:refine-sem}
%     \Big(\bigvee_i \invar'_i \subseteq \invar_i \setminus \{c_i\} \Big) \wedge \Big(\bigwedge_i \invar'_i \subseteq \invar_i \Big) \wedge \Big(\invar_i' \text{ are valid invariants} \Big) 
%     \end{equation}
%     If $\idd$ cannot be refined, we add $c_1, c'_1$ to $\rp$. \\
% \end{enumerate}

% our algorithm has a state, $\langle r^{\dagger}, \invar^{\dagger} \rangle$ where $r^{\dagger} = \{ \langle X_1, \cdots, X_n \rangle \ | \ X_i \text{is a program state at the beginning of each loop} \}$ and $\invar^{\dagger} = \langle \invar_1 \cdots, \invar_n \rangle$.  $r^{\dagger}$ is initialized using a set of program traces, while $\id$ is initialized as $\langle \true, $
% $dom(t) \subseteq \reachp \subseteq \invar$. When considering nested loops, since the inner loop is approximated by an invariant, instead of only storing a subset of $\reach$, $r$, we have to store a subset of $\trans$, $t$. Since $dom(t)$ gives us $r$, we only store $t$ in the algorithm state.  First, we initialize $t$ with pairs of states sampled before and after the loop from execution traces of the program, and we initialize $\invar$ to the set of all states. Then, we iteratively perform the generate candidate phase and the refine state phase. In the following, we explain these phases in terms of $\reachp$ and the corresponding movement in the lattices, $\lati$ and $\latr$.
% \begin{enumerate}
    % \item \textbf{Generate Candidate Phase:} If $F_{\tempi}(t)$ is empty, there is no possible ranking function in $\tempr$ that is valid w.r.t. $\invar', \trans$ where $\invar' \in \tempi$. Otherwise, we sample a ranking function, $f$, from $F_{\tempr}(t)$. Then, we check the validity of $f$ w.r.t. $\invar, \trans$. If $f$ is valid w.r.t. $\invar, \trans$, we have proved that the loop terminates. If the validity check fails, we continue to the Refine State Phase.
    % \item \textbf{Refine State Phase:} We obtain $c \in \trans$ as a counter-example to $f$ from the validity check. We sample a invariant, $\invar' \in \tempi$, such that $\invar'$ is valid w.r.t. the loop and  

% \end{enumerate}


\textbf{Movement in the Lattices}
In the Refine Phase, we either move down in $\lati(\prog, \tempi)$ or move down in $\latr(\tempr)$. 
If the annotated program $L$ can be refined to $L'$,  
% If the invariant, $\invar = (\invar_1, \cdots, \invar_n)$, can be refined to $\invar' = (\invar'_1, \cdots, \invar'_n) \in \tempi^1 \times \cdots \times \tempi^n$, 
then from Equation~\ref{eq:refine-sem}, we know that $L' \prec L$. 
% The specific path taken down the lattice is not known, but at each step when the invariant is refined, it takes at least one step down the semi-lattice $\lati(\prog, \tempi)$. 
We prove that if we have templates $\tempi^1, \cdots, \tempi^n$ such that each $\tempi^i$ is closed under intersection, and we have an annotated program, $L$, s.t. $\ini \models L$, and there exists an annotated program, $L^*$, and a given ranking function $f$, s.t., $\ini \models L^*, f$, then there is always an annotated program $L''$ s.t., $L'' \less L$ and $\ini \models L'', f$. 
% This is formally stated in Appendix~\ref{}.

\begin{lemma}
    \label{lemma:below}
    If (i) $f \in \tempr$, (ii) $\anno_1, \anno_2 \in \lati(L, \tempi)$ (iii) $\ini \models \anno_2$ (iv) $\ini  \models \anno_1, f$, (v) $\tempi$ is closed under intersection then $\exists \anno_3$ s.t. $\ini \models \anno_3, f$ and $\anno_3 \less \anno_2$.
\end{lemma}

\begin{lemma}
    \label{lemma:lati}
    If (i) $f \in \tempr$, (ii) $\big(\core{\anno} = L\big) \wedge \big(\ini \models \anno\big)$, (iii) $\exists \anno_* \cdot \big(\core{\anno_*} = L\big) \wedge \big(\ini  \models \anno_*, f\big)$, (iv)  $\tempi$ is closed under intersection and $\lati(L, \tempi)$ has no infinite descending chain, then repeated application of the refine phase (which always terminates in finite time) will find $\anno_1$ s.t.  $ \big(\core{\anno_1} = L \big) \wedge \big(\ini \models \anno_1, f\big)$
\end{lemma}

To prove this lemma, we prove that given a valid ranking function $f$, we keep going down in $\lati(L, \tempi)$ until we find an invariant that proves the ranking. Since there is always an invariant below in $\lati(L, \tempi)$ that can prove $f$ and $\lati(L, \tempi)$ does not have an infinite descending chain, we will eventually find an invariant that can prove $f$.



% \begin{lemma}
%     If 
%     \begin{enumerate}
%         \item $\tempi^1, \cdots, \tempi^n$ are all closed under intersection
%         \item $\invar_1, \cdots, \invar_n$ are each valid invariants for loops $1$ to $n$ respectively
%         \item $(\invar^*_1, \cdots, \invar^*_n)$ can be used to prove $f$
%     \end{enumerate}
%     Then there exists $(\invar'_1, \cdots, \invar'_n) \in \tempi^1 \times \cdots \times \tempi^n$ s.t.
%     \begin{enumerate}
%         \item $(\invar'_1, \cdots, \invar'_n) \preceq (\invar_1, \cdots, \invar_n)$
%         \item $\invar'_1, \cdots, \invar'_n$ are valid invariants for loops $1$ to $n$ respectively
%         \item $(\invar'_1, \cdots, \invar'_n)$ can be used to prove $f$
%     \end{enumerate}
% \end{lemma}

If we cannot refine the invariant, we create $\rp_{new} = \rp \cup \{(c,c')\}$. Since $\rp \subset \rp_{new}$ and $f \notin \func(\{(c,c'), \tempr\})$, so, $f \notin \func(\{\rp_{new}, \tempr\})$. Therefore, $\func(\{\rp_{new}, \tempr\}) \prec \func(\{\rp, \tempr\})$. We can also prove that if there is a function $f^* \in \tempr$, that is a valid ranking function for the loop, then $f^* \in F(\rp_{new})$. 
% Since we are going down in $\latr$, we are reducing the size of the search space for a correct ranking function.

\begin{lemma}
    \label{lemma:latf}
    If for $f \in \func(\{\rp, \tempr\}), \not\exists \anno \cdot \big(\core{\anno} = L\big) \wedge \big(\ini \models \anno, f\big)$, then then the repeated application of the refine phase will terminate and $\func(\{\rp_{new}, \tempr\}) \prec \func(\{\rp, \tempr\})$.
\end{lemma}

For this algorithm, we make the following assumptions about $\tempr$ and $\tempi$ - (i) $\tempr$ is finite, (ii) $\tempi$ is closed under intersection, (iii) there is no infinite descending chain in $\lati(L, \tempi)$, (iv) given $f$ and $\anno$, checking $\ini \models \anno, f$ falls in a decidable SMT theory, (v) given a set of pairs of states, $r$, we can find a ranking function, $f \in \func(\{r, \tempr\})$  or determine that no such ranking function exists in finite time, (vi) there is a function that can simulate the refine semantics as in Equation~\ref{eq:refine-sem}.

\begin{theorem}
    \label{theorem:find}
    If 
    \begin{enumerate}
        \item $\exists f^* \in \tempr, \exists \anno^* \cdot \big(\core{\anno^*} = L\big) \wedge (\ini \models \anno^*, f^*\big)$
        \item We have proved the termination of all the loops inside the loop body
        \item The algorithm assumptions above hold
    \end{enumerate}
    Then our algorithm will terminate with $f \in \tempr$ and $\anno$ s.t. $\big(\core{\anno} = L\big) \wedge (\ini \models \anno, f\big)$
\end{theorem}

To prove this theorem, we use Lemmas~\ref{lemma:lati} and ~\ref{lemma:latf}. We maintain $\rp$ and $\anno$ as the state of the algorithm. $\rp$ always contains reachable states w.r.t $\tempi$, so at each algorithm state, $f^* \in \func(\rp, \tempr)$. At each refine phase, we have a candidate function $f_1$, and a counter-example for that function $(c, c')$. If $f_1$ can be proved by some $\anno$, then using Lemma~\ref{lemma:lati}, we will find $\anno_2$ that proves $f_1$. Otherwise, using Lemma~\ref{lemma:latf}, we will go down in the lattice $\latr(\tempr)$. Since $\latr(\tempr)$ is finite and we go down in the lattice every time an invalid ranking function is generated as a candidate, the algorithm terminates. The algorithm can only terminate if $\func(\rp, \tempr) = \emptyset$ or if a ranking function $f_2$, is proved using an $\anno$. Since  $f^*$ is always in $\func(\rp, \tempr)$, it is never empty, so we will always find a valid ranking function.

\begin{theorem}
\label{theorem:terminate}
    If
    \begin{enumerate}
        \item $\forall f \in \tempr \ \not\exists \anno$ s.t. $\big(\core{\anno} = L\big) \wedge \big(\ini \models \anno, f\big)$
        \item The algorithm assumptions above hold
    \end{enumerate}
    Then our algorithm will terminate without finding a valid ranking function
\end{theorem}

This theorem is true because at each refine phase, we either go down in $\latr(\tempr)$ or $\lati(L, \tempi)$. Since both $\latr(\tempr)$ and $\lati(L, \tempi)$ do not contain any infinite descending chains, so eventually we will terminate. If there is no ranking function that can be proved, we will only terminate when $\func(\rp, \tempr)$ is empty.

Theorems~\ref{theorem:find} and ~\ref{theorem:terminate} are stated for the outermost loop with an arbitrary nesting of loops inside. The same theorem can be applied inductively to each inner loop.
Further, the theorems can be generalized to have different templates for ranking functions and invariants for each loop in the program.
 }

==> sections/algorithm.tex <==
\section{Algorithm}

% \begin{definition}
%     An invariant template $\tempi$ is a given set of candidate invariants.
% \end{definition}

% \begin{definition}
%     A ranking function template $\tempr$ is a given set of candidate ranking functions.
% \end{definition}

Our algorithm takes as input a template of candidate invariants. We only analyze invariants from this template. More formally, a template of candidate invariants, $\tempi$, is a set of candidate invariants, which are in turn sets of program states. For instance, in the running example from the previous section, the template was the sets of program states that can be represented as a conjunction of constraints of the form $c_0 + \sum_ic_ix_i \ge 0$ where $x_i$ are the program variables and $c_i \in \mathbb{Z}$. Given two candidate invariants, $\invar_1$ and $\invar_2$, we  define a relation, $\preceq_{\invar}$, such that $\invar_1 \preceq_{\invar} \invar_2 \triangleq \invar_1 \subseteq \invar_2$. This defines a partial order over $\tempi$. We also define an operation, $\wedge_{\invar}$, over the two invariants as $\invar_1 \wedge_{\invar} \invar_2 \triangleq \invar_1 \cap \invar_2$. This gives us a semi-lattice over $\tempi$. When we are analyzing nested loops, we define a lattice over $\tempi^1 \times \cdots \times \tempi^n$, where $\tempi^i$ is the template of invariants for the $i$-th loop. For two elements of this lattice, $(\invar_1^1, \cdots, \invar_1^n), (\invar_2^1, \cdots, \invar_2^n)$, $(\invar_1^1, \cdots, \invar_1^n) \preceq_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq \bigwedge_i \invar_1^i \subseteq \invar_2^i$ and $(\invar_1^1, \cdots, \invar_1^n) \wedge_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq (\invar_3^1, \cdots, \invar_3^n)$ where $\invar_3^i \triangleq \invar_1^i \cap \invar_2^i$.

\begin{definition}
    $\lati$ is a meet semi-lattice such that $\lati = (\tempi^1 \times \cdots \times \tempi^n, \preceq_{\invar}, \wedge_{\invar})$, where $(\invar_1^1, \cdots, \invar_1^n) \preceq_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq \bigwedge_i \invar_1^i \subseteq \invar_2^i$ and $(\invar_1^1, \cdots, \invar_1^n) \wedge_{\invar} (\invar_2^1, \cdots, \invar_2^n)  \triangleq (\invar_3^1, \cdots, \invar_3^n)$ where $\invar_3^i \triangleq \invar_1^i \cap \invar_2^i$
\end{definition}

Similarly, the algorithm also takes as input a template of candidate ranking functions. We only analyze ranking functions from this template. Formally, a template of candidate ranking functions, $\tempr$, is a set of functions $f: S \rightarrow \mathbb{R}$. In the example above, we use the set of functions of the form $\max(a_0 + \sum_i a_ix_i,0) + \max(b_0 + \sum_i b_ix_i,0)$ where $x_i$ are the program variables and $a_i,b_i \in \mathbb{Z}$.
Given two sets of candidate ranking functions, $F_1, F_2 \subseteq \mathcal{P}(\tempr)$, we define a relation, $\preceq_{F}$, such that $F_1 \preceq_{F} F_2 \triangleq F_1 \subseteq F_2$. We also define an operation, $\wedge_{F}$, as $F_1 \wedge_{F} F_2 \triangleq F_1 \cap F_2$. This gives us a lattice over the powerset of $\tempr$, $\latr$.
 
\begin{definition}
    $\latrfs$ is a meet semi-lattice on  $\mathcal{P}(\tempr)$: $\latrfs = (\mathcal{P} ({\tempr})\preceq_{F}, \wedge_{F})$, where $\mathcal{F}_1 \preceq_{F} \mathcal{F}_2 \triangleq \mathcal{F}_1 \subseteq \mathcal{F}_2$ and $\mathcal{F}_1 \wedge_{F} \mathcal{F}_2 \triangleq \mathcal{F}_1 \cap \mathcal{F}_2$
\end{definition}

To avoid clutter, we use $\wedge$ for both $\wedge_{\invar}$ and $\wedge_{F}$, and similarly, we use $\prec$ for both $\prec_{\invar}$ and $\prec_{F}$. the reader can disambiguate based on context.

To prove termination, we have to find a valid ranking function and an invariant. Given a transition relation for a loop, $t \subseteq \trans$ where $dom(t) \in \reach$, $F_{\tempr}(t)$ contains all of the ranking functions in $\tempr$ that satisfy the necessary condition for being valid w.r.t. $dom(t), t$. Therefore, if a ranking function that is valid w.r.t. $\reach, \trans$ exists, then it has to be in $F_{\tempr}(t)$. According to the definitions above, as we go down in $\latr$, the elements of $\mathcal{P}(\tempr)$ shrink, thereby reducing the search space for a valid ranking function. As we add elements to $t$, we create a more precise under-approximation of $\reach$, and $F_{\tempr}(t)$ goes down in $\latr$. Similarly, as we go down in  $\lati$ while also maintaining the validity of the invariant, the invariant keeps getting stronger, which creates a better over-approximation of $\reach$. 

Now, we will present the algorithm and explain how it goes down in $\latr$ and $\lati$.



 % Given a transition relation, $t \subseteq S \times S$, we define $F_{\tempr}(t)$ as the set of functions, $f \in \tempr$, such that $t \subseteq sat(f)$. 

 %    $$F_{\tempr}(t) = \{f \in \tempr \ | \  \forall (x,x') \in t, f(x) - f(x') \ge 1 \wedge f(x) \ge 0 \wedge f(x') \ge 0 \}$$
 
\textbf{Reachability w.r.t. Template:} The set of reachable program states at a point is canonical to the strongest invariant at that point.  
Since all our invariants are restricted to the template $\tempi$, we introduce the notion of $\reachp$ as the set of all reachable states \textit{with respect to our template} $\tempi$. Consider, $val_\mathcal{T}$, which is a subset of $\tempi$, defined as the set of all valid invariants w.r.t the program in $\tempi$. We define $\reachp = \bigcap val_\mathcal{T}$.

\begin{definition}
    \label{def:rp}
    Given $\tempi$, $\reachp$ is the set of states $X$ such that for all $\invar \in val_\mathcal{T} \cdot X \in \invar$.
\end{definition}

% Consider a program, $P$, \texttt{while $B_1$ do $P_1$ while $B_2$ do $P_2$ od $P_3$ od } where $P_1,P_2,P_3$ are loop-free. If we have invariants, $I_1$ and $I_2$ are invariants for the outer and inner loop respectively. 
% Consider $\trans' = I'_1 \circ P_1 \circ (I_2 \times  I_2) \circ P_3 $, where $I'_1 = \{ (X,X) \ | \ X \in \invar_1 \}$. Observe that the relation $\trans'$ over-approximates the transition relation induced by the program $P$. 
% Similarly, given any program, if we abstract all the loops in the program with their respective invariants, the transition system of the program can be over-approximated by the relation defined by the loop-free parts of the program and the invariants corresponding to the loops. 
% So, at each step of our algorithm, 

Given a loop with loop-free body, $P$, our algorithm has a state $\langle \rp, \invar \rangle$. $\rp$ is an under-approximation of $\llbracket P \rrbracket$ initialized from a set of execution traces of $P$ and $\invar$ is an over-approximation of $\reachp$ initialized with \true.  Then, we iteratively perform the Generate Candidate phase and the Refine State.

\textbf{Generate Candidate Phase:} If $F_{\tempr}(\rp)$ is empty, there is no possible ranking function in $\tempr$ that is valid w.r.t. $\reachp, \llbracket P \rrbracket$. Otherwise, we choose an arbitrary element, $f \in F_{\tempr}(\rp)$. Then, we check the validity of $f$ w.r.t. $\invar,  \llbracket P \rrbracket$ by using an SMT query. We define symbolic variables to represent the state at the beginning of the loop and symbolically execute the loop body $P$ to obtain the program state at the end of the loop, $X'$. Then, we check if there exists a state $X \in \invar$ for which $f(X) - f(X') < 1$ or $f(X) < 0$. 
If $f$ is valid w.r.t. $\invar, \trans$, we have proved that the loop terminates. If the validity check fails, we continue to the Refine Phase.

\textbf{Refine State Phase:} We obtain $c$ where $c \in \invar$ as a counter-example to $f$ from the validity check presented above. So, $c$ is a program state such that 
\begin{equation} \Big(f(c) - f( \llbracket P \rrbracket c) < 1 \Big) \vee \Big( f(c) < 0 \Big) \end{equation}
Using $c$, we check if there is a valid invariant, $\invar' \in \tempi$, which is stronger than $\invar$ and excludes $c$. If $\invar'$  exists, we can refine $\invar$ to $\invar'$. Otherwise, we cannot refine $\invar$.
\begin{equation}
    refine(\invar, c) = \left\{ \begin{array}{rcl}
    \invar' \text{ s.t. } (\invar' \subseteq \invar \setminus \{c\}) \wedge (\invar' \text{is a valid invariant})  & \text{if $\invar$ can be refined} \\
    \false & \text{if $\invar$ cannot be refined}
    \end{array}\right.
\end{equation}
 If we find $\invar'$, then the algorithm state is updated to $\langle \rp, \invar' \rangle$. If there is no such invariant, then the algorithm state is updated to $\langle \rp \cup \{c\}, \invar \rangle$.

% \end{enumerate}

When considering nested loops, first we prove the termination of the innermost loop, which results in $f$ and $\invar$, a ranking function and invariant for the innermost loop. We do not need to store the ranking function, but we store $\invar$. We keep doing this recursively. So, when proving the termination of a loop with a body, $P$, that has $n-1$ nested loops, we will get $n-1$ invariants as an output of proving their individual terminations, $\overline{\invar}_2, \cdots, \overline{\invar}_n$. Instead of $\langle \rp, \invar \rangle$, our program state will be  $\langle \rp, \invar^{\dagger} \rangle$ where $\invar^{\dagger} = (\invar_1, \cdots, \invar_n)$ and $\invar_i$ is an invariant for the $i$-th loop. It is initialized $\langle \true, \overline{\invar}_2, \cdots, \overline{\invar}_n \rangle$. Now, we will explain the 2 phases for handling nested loops:
\begin{enumerate}
    \item \textbf{Generate Candidate Phase:} A candidate ranking function, $f$, is generated in the same way as in the case of a single loop. However, for the validity check, we cannot simply symbolically execute the body of the loop. This is because although all of the inner loops terminate, we do not know the number of iterations that they run for. As shown in Section~\ref{sec:background}, from a program and invariants for the loops in a program, we can over-approximate $ \llbracket P \rrbracket X $. To achieve this, we declare a new symbolic program state, $X_i$, as an output to each inner loop and assume that $X_i \in \invar_i$ 
    % Here, we choose an arbitrary element from $F_{\tempr}(\rp)$ as a candidate ranking function. If $F_{\tempr}(r^{\dagger})$ is empty, then the algorithm terminates concluding that there is no ranking function in $\tempr$ w.r.t. an invariant in $\tempi, \llbracket P \rrbracket X$.
    % Since all the $\invar_i$ are not guaranteed to be the strongest invariants of their respective loops, we do not have the exact representation of $ \llbracket P \rrbracket X $. However, 
     Then, we check the validity of $f$. Again, if the validity is proven, the algorithm has proved termination, and otherwise, the algorithm proceeds to the Refine State Phase. 
    
    \item \textbf{Refine State Phase:} We obtain a counter-example, $c^{\dagger} = (c_1,\cdots, c_n)$, from the validity check. $c_1$ is a program state at the beginning of the outermost loop and each $c_i$ is a program state at the end of the $i$-th loop. Using $c_n$, we can compute $c'_1$, which is a program state at the end of the outermost loop. 
    \begin{equation}
        \Big( f(c_1) - f(c'_1) < 1 \Big) \vee \Big( f(c_1) < 0 \Big)
    \end{equation}
    
    We use this counter-example to refine $\idd$ to an invariant, $\idd_{new} \in \tempi^1 \times \cdots \times \tempi^n$ $\idd_{new} = (\invar'_1, \cdots, \invar'_n) = refine(\idd, c^{\dagger} )$ and has the following property:
    \begin{equation}
    \label{eq:refine-sem}
    \Big(\bigvee_i \invar'_i \subseteq \invar_i \setminus \{c_i\} \Big) \wedge \Big(\bigwedge_i \invar'_i \subseteq \invar_i \Big) \wedge \Big(\invar_i' \text{ are valid invariants} \Big) 
    \end{equation}
    If $\idd$ cannot be refined, we add $c_1, c'_1$ to $\rp$. \\
\end{enumerate}

% our algorithm has a state, $\langle r^{\dagger}, \invar^{\dagger} \rangle$ where $r^{\dagger} = \{ \langle X_1, \cdots, X_n \rangle \ | \ X_i \text{is a program state at the beginning of each loop} \}$ and $\invar^{\dagger} = \langle \invar_1 \cdots, \invar_n \rangle$.  $r^{\dagger}$ is initialized using a set of program traces, while $\id$ is initialized as $\langle \true, $
% $dom(t) \subseteq \reachp \subseteq \invar$. When considering nested loops, since the inner loop is approximated by an invariant, instead of only storing a subset of $\reach$, $r$, we have to store a subset of $\trans$, $t$. Since $dom(t)$ gives us $r$, we only store $t$ in the algorithm state.  First, we initialize $t$ with pairs of states sampled before and after the loop from execution traces of the program, and we initialize $\invar$ to the set of all states. Then, we iteratively perform the generate candidate phase and the refine state phase. In the following, we explain these phases in terms of $\reachp$ and the corresponding movement in the lattices, $\lati$ and $\latr$.
% \begin{enumerate}
    % \item \textbf{Generate Candidate Phase:} If $F_{\tempi}(t)$ is empty, there is no possible ranking function in $\tempr$ that is valid w.r.t. $\invar', \trans$ where $\invar' \in \tempi$. Otherwise, we sample a ranking function, $f$, from $F_{\tempr}(t)$. Then, we check the validity of $f$ w.r.t. $\invar, \trans$. If $f$ is valid w.r.t. $\invar, \trans$, we have proved that the loop terminates. If the validity check fails, we continue to the Refine State Phase.
    % \item \textbf{Refine State Phase:} We obtain $c \in \trans$ as a counter-example to $f$ from the validity check. We sample a invariant, $\invar' \in \tempi$, such that $\invar'$ is valid w.r.t. the loop and  

% \end{enumerate}


\textbf{Movement in the Lattices}
In the Refine Phase, we either move down in $\lati$ or move down in $\latr$. If the invariant, $\invar = (\invar_1, \cdots, \invar_n)$, can be refined to $\invar' = (\invar'_1, \cdots, \invar'_n) \in \tempi^1 \times \cdots \times \tempi^n$, then from Equation~\ref{eq:refine-sem}, we know that $(\bigvee_i \invar'_i \subseteq \invar_i \ \{c_i \}) \wedge (\bigwedge_i \invar'_i \subseteq \invar_i)$. So, $\invar' \prec \invar$. The specific path taken down the lattice is not known, but at each step when the invariant is refined, it takes one path down the lattice. We prove that if we have templates $\tempi^1, \cdots, \tempi^n$ such that each $\tempi^i$ is closed under intersection, and we have valid invariants, $(\invar_1, \cdots, \invar_n)$, and there is an invariant, $(\invar^*_1, \cdots, \invar^*_n)$, that can prove the the validity of a given ranking function $f$ for a loop, then there is always an invariant below $(\invar_1, \cdots, \invar_n)$ in $\lati$ that can prove that can prove the the validity of $f$. This is formally stated in Appendix~\ref{}.

\begin{lemma}
    \label{lemma:lati}
    If
    \begin{enumerate}
    \item we have a ranking function $f \in \tempr^1$
    \item there exists some $\idd_0 = (\invar^0_1, \cdots, \invar^0_n) \in \tempi^1 \times \cdots \times \tempi^n$ that can prove the validity of $f$
    \item we have $\idd_1 = (\invar^1_1, \cdots, \invar^1_n) \in \tempi^1 \times \cdots \times \tempi^n$ where each $\invar^1_i$ is a valid invariant for loop $i$
    \item each $\tempi^i$ is closed under intersection and $\lati$ has no infinite descending chain
    \end{enumerate}
    Then, repeatedly executing the refine phase (which always terminates in finite time), we will find $\idd_2 = (\invar^2_1, \cdots, \invar^2_n) \in \tempi^1 \times \cdots \times \tempi^n$ that can prove $f$ where each $\invar^2_i$ is a valid invariant for loop $i$ 
\end{lemma}

To prove this lemma, we prove that given a valid ranking function $f$, we keep going down in $\lati$ until we find an invariant that proves the ranking. Since there is always an invariant below in $\lati$ that can prove $f$ and $\lati$ does not have any infinite descending chains, we will eventually find an invariant that can prove $f$.

% \begin{lemma}
%     If 
%     \begin{enumerate}
%         \item $\tempi^1, \cdots, \tempi^n$ are all closed under intersection
%         \item $\invar_1, \cdots, \invar_n$ are each valid invariants for loops $1$ to $n$ respectively
%         \item $(\invar^*_1, \cdots, \invar^*_n)$ can be used to prove $f$
%     \end{enumerate}
%     Then there exists $(\invar'_1, \cdots, \invar'_n) \in \tempi^1 \times \cdots \times \tempi^n$ s.t.
%     \begin{enumerate}
%         \item $(\invar'_1, \cdots, \invar'_n) \preceq (\invar_1, \cdots, \invar_n)$
%         \item $\invar'_1, \cdots, \invar'_n$ are valid invariants for loops $1$ to $n$ respectively
%         \item $(\invar'_1, \cdots, \invar'_n)$ can be used to prove $f$
%     \end{enumerate}
% \end{lemma}

If we cannot refine the invariant, then we move down in $\latr$. In the Refine Phase, we obtain a counter-example, $c^{\dagger} = (c_1, \cdots, c_n)$, for the candidate ranking function, $f$. Using $c_n$, we compute the state $c'$ at the end of the outermost loop. We create $\rp_{new} = \rp \cup \{(c,c')\}$. Since $\rp \subset \rp_{new}$ and $(c,c') \notin sat(f)$, $F(\rp_{new}) \prec F(\rp)$. We can also prove that if there is a function $f^* \in \tempr^1$, that is valid ranking function for the loop, then $f^* \in F(\rp_{new})$. Since we are going down in $\latr$, we are reducing the size of the search space for a correct ranking function.

\begin{lemma}
    \label{lemma:latf}
    If we have a ranking function $f \in F(\rp_1)$ that cannot be proved with any invariant in $\tempi^1 \times \cdots \times \tempi^n$
    Then the repeated application of the refine phase will terminate refining $\rp_1$ to $\rp_2$ s.t. $F(\rp_2) \prec F(\rp_1)$
\end{lemma}

For this algorithm, we make the the following assumptions about $\tempr^1$ and $\tempi^1, \cdots, \tempi^n$: $\tempr^1$ is finite. $\tempi^1, \cdots, \tempi^n$ are all closed under intersection and there is no infinite descending chain in the lattice $\tempi$ defined on elements of $\tempi^1 \times \cdots \times \tempi^n$. Given a valid invariant $\invar_i$ and a program state $c_i$, it is possible to find a valid invariant $\invar'_i$ such that $\invar'_i \subseteq \invar_i \setminus \{c_i\}$ if such an invariant exists or determine that no such invariant exists within finite time. Given a subset of $\llbracket P \rrbracket$, $r$, where $dom(r) \in \reachp$ we can find a ranking function, $f \in \tempr^1$ from the set $F(r)$ or determine that no such ranking function exists in finite time. The validity-check of a ranking function w.r.t. a set of states and a transition relation falls in a decidable theory.

\begin{theorem}
    \label{theorem:find}
    If 
    \begin{enumerate}
        \item there exists a ranking function $f^* \in \tempr^1$, and an invariant $\invar_*^{\dagger} \in \tempi^1 \times \cdots \times \tempi^n$, s.t. $\invar_*^{\dagger}$ can prove the validity of $f^*$
        \item we have proved the terminations of all the loops inside the outermost loop
        \item The algorithm assumptions above hold
    \end{enumerate}
    Then our algorithm will terminate with $f \in \tempr^1$, $\idd \in \tempi^1 \times \cdots \times \tempi^n$ s.t. $\idd$ can prove the validity of $f$
\end{theorem}

To prove this theorem, we use Lemmas~\ref{lemma:lati} and ~\ref{lemma:latf}. We maintain $\rp$ and $\idd$ as the state of the algorithm. $\rp$ always contains reachable states, so at each algorithm state, $f^* \in F(\rp)$. At each refine phase, we have a candidate function $f_1$, and a counter-example for that function $c^{\dagger}$. If $f_1$ can be proved by some $\idd_0 \in \tempi^1 \times \cdots \times \tempi^n$, then using Lemma~\ref{lemma:lati}, we will find $\idd_2$ that proves $f$. Otherwise, using Lemma~\ref{lemma:latf}, we will go down in the lattice $\latr$. Since $\latr$ is finite and we go down in the lattice every time an invalid ranking function is generated as a candidate, the algorithm terminates. The algorithm can only terminate is $F(\rp) = \emptyset$ or if a ranking function $f_2$, is proved using an invariant. Since  $f^*$ is always in $F(\rp)$, it is never empty, so we will always find a valid ranking function.

\begin{theorem}
\label{theorem:terminate}
    If
    \begin{enumerate}
        \item There does not exist a ranking function, $f \in \tempr^1$ that can be proved with any invariant in $\tempi^1 \times \cdots \times \tempi^n$
        \item The algorithm assumptions above hold
    \end{enumerate}
    Then our algorithm will terminate without finding a valid ranking function
\end{theorem}

This theorem is true because at each refine phase, we either go down in $\latr$ or $\lati$. $\latr$ is finite and $\lati$ does not contain any infinite descending chains, so eventually we will terminate. If there is no ranking function that can be proved, we will only terminate when $F(\rp)$ is empty.

Theorems~\ref{theorem:find} and ~\ref{theorem:terminate} are stated for the outermost loop with an arbitrary nesting of loops inside. The same theorem can be applied inductively to each inner loop.

 
% \begin{algorithmic}[1]
% \Procedure{$\fr$}{$\rp, \invar$}
%     \State $f \gets \gc(\rp)$
%     \If{$\checkr(f, \invar)$} 
%         \State \Return t
%     \Else
%         % \State $c \gets \gcounter(f, \invar)$
%         % \State $\invar' \gets \invar$
%         % \State $c' \gets c$
%         \While{$\true$}
%             \State $c \gets \gcounter(f, \invar)$
%             \State $\text{is\_refined}, \; \invar \gets \mathsf{refine}(\invar, c)$
%             \If{$\text{is\_refined}$}
%                 \If{$\checkr(f, \invar)$} 
%                     \State \Return f
%                 % \Else 
%                 %     \State $c \gets \gcounter(f, \invar')$
%                 \EndIf
%             \Else
%                 \State $\rp \gets \rp \cup \{c\}$
%                 \State \Return $\fr(\rp_{new}, \; \invar)$ 
%             \EndIf
            
            
%         \EndWhile
%     \EndIf 
% \EndProcedure
% \end{algorithmic}


==> sections/exps_backup.tex <==
\section{Evaluation}
\label{sec:evaluation}

\subsection{Experimental Setup}

We implement the instantiation of the \toolname framework in Python as described in Section~\ref{sec:implementation}. The tool expects Java programs as inputs and if the program is termination, it returns the ranking functions and the loop invariants. The Z3-Java API is then used to check the validity of the returned ranking functions and the loop invariants.  All the experiments are performed on a 2.50 GHz 16 core 11th Gen Intel i9-11900H CPU with a main memory of 64 GB. 

\myparagraph{Benchmarks}

\begin{table}[h]
    \centering
    \begin{tabular}{l|ccc|r}
        \toprule
         & \textbf{Single-while} & \textbf{Nested-while} & \textbf{Others}  & \textbf{Total} \\
        \midrule
        Deterministic & 110 & 19 & 0 & 129 \\
        Non-Deterministic & 36 & 3 & 2 & 41 \\
        \hline
        Total & 146 & 22 & 2 & 170 
        \bottomrule
    \end{tabular}
    \caption{Example table with row and column headers}
    \label{tab:example}
\end{table}
\myparagraph{Baselines}

In our evaluation, we compare with state-of-the-art baselines: $\nu$Term~\cite{nuterm},  DynamiTe~\cite{dynamite}, Ultimate~\cite{ultimate}, and Aprove~\cite{aprove}. \\
\textbf{$\nu$Term. } 
This technique represents ranking functions via neural networks that are learned from randomly generated traces. The neural network is trained to maximize the difference between the output of two consecutive states. \\
% This training, however, is independent of the invariants needed to check the validity of the corresponding ranking function. Instead, they rely on predetermined candidate invariants and check their validity separately.  
\textbf{DynamiTe. } 
    This algorithm tries to prove the non-termination of programs by finding recurrent sets, failing which it generates a counter-example that is then used to find candidate ranking functions. To finally prove termination, the synthesis of required invariants is outsourced to an external invariant synthesis algorithm, DIG~\cite{dig}.\\
    % Again, the invariant synthesis is not guided by termination analysis or vice versa. \\
\textbf{Ultimate. }
    This algorithm decomposes programs into smaller sub-programs and constructs ranking functions for these sub-programs. After finding each ranking function, it checks whether the current set of sub-programs captures the behavior of the entire loop.  \\ 
\textbf{Aprove. }
    Aprove is an ensemble of several proof techniques based on heuristics for proving termination, including termination proofs through reduction orders and termination proofs through dependency pairs. 
% \begin{itemize}
%     \item \textbf{$\nu$Term. } 
%     This technique uses neural networks to learn ranking functions from randomly generated traces. The learned neural network acts as a ranking function which is trained such that the difference between the output of two consecutive states is maximized. This training, however, is independent of the invariants needed to check the validity of the corresponding ranking function. Instead, they rely on predetermined candidate invariants and check their validity separately. 
%     % This prevents $\nu$Term from using the invariants to guide the search for ranking functions or vice versa. Further, they cannot provide any completeness guarantees due to the use of neural networks to generate candidate ranking functions.   
%     % We compare our technique against $\nu$Term to study the effect of using invariants during the search for ranking functions. To do so, we use the templates that can represent the exact neural network architecture used by $\nu$Term. We also show ablation studies to analyze the effect of different templates.

%     \item  \textbf{DynamiTe. } 
%     This algorithm tries to prove the non-termination of programs by finding recurrent sets, failing which generates a counter-example that is then to a ranking function for termination. To finally prove termination, the synthesis of required invariants is outsourced to an external invariant synthesis algorithm, DIG~\cite{}. Again, the invariant synthesis is not guided by termination analysis or vice versa.

%     \item \textbf{Ultimate. }
%     This algorithm decomposes programs into smaller sub-programs and constructs termination arguments for these sub-programs. After generating each termination argument, it checks whether the decomposed modules capture the behavior of the entire loop. 

%     \item \textbf{Aprove. }
%     Aprove is an ensemble of several proof techniques based on heuristics for proving termination, including termination proofs through reduction orders and termination proofs through dependency pairs. 

    
% \end{itemize}
We study the benefits of the synergy between finding ranking functions and invariants by comparing our technique to $\nu$Term which is the most similar baseline to ours. This is because it also generates ranking functions of a specific form and checks their validity by leveraging invariants. However, these invariants are generated independently of the ranking function analysis. We use a subset of the total benchmarks for this experiment because $\nu$Term does not handle non-deterministic function calls. To further demonstrate the utility of the specific way we guide the searches of invariants and ranking functions, we compare with 3 other strategies of synergy.
% To do so, we use a template that can represent the exact neural network architecture used by $\nu$Term. 
We also show the overall comparison of the number of programs that can be proved to terminate using our technique vs. others. Lastly, we show case studies demonstrating the benefits of the synergy employed by our technique.

% \subsection{Experimental Setup}
% \textit{Benchmarks. }
We collect 171 challenging programs as benchmarks from the \textit{Term-crafted} set of SV-COMP\cite{svcomp}, the \textit{Aprove\_09} set from TermComp\cite{termcomp}, and \textit{$\nu$Term-advantage} from $\nu$Term\cite{nuterm}.  These benchmarks contain integer programs, with linear and non-linear assignments and loop guards, non-determinism, and nested loops of maximum depth 3. These benchmarks do not include function calls, except a call to generate a random integer, as our current implementation does not support them. The programs were originally in C but were translated to Java~\cite{nuterm}. The experiments for \toolname and $\nu$Term are run on the Java version while the experiments for Aprove, Ultimate, and DynamiTe are run on the equivalent C benchmarks. We use a timeout of 120 seconds for all of our experiments. When calculating the average time, we exclude the benchmarks for which the technique did not prove termination. 
% Aprove chooses between many termination proof techniques based on heuristics, including termination proofs through reduction orders and termination proofs through dependency pairs. Ultimate decomposes programs into smaller terminating programs and constructs termination arguments for these programs. After generating each termination argument, it checks whether the decomposed modules capture the behavior of the entire loop. DynamiTe has two subprocesses, one proving termination and another proving non-termination, where the recurrent sets that are disproved are used as samples to improve the ranking function search. It is supported by an external invariant synthesis algorithm, DIG~\cite{}.  Then, we compare overall termination analysis results with the other baselines. 
% 

% We use benchmarks from the term-crafted set of SV-COMP\cite{}, the Aprove_09 set from TermComp\cite{}, and nuTerm-advantage from $\nu$Term\cite{}.  These benchmarks were originally in C, but were translated to Java~\cite{}. The experiments for our code and $\nu$Term are run on the Java benchmarks while the experiments for Aprove, Ultimate and Dynamite are run on the equivalent C benchmarks. All of our experiments were run on a 2.50 GHz 16 core 11th Gen Intel i9-11900H CPU with a main memory of 64 GB.

% We will examine the following research questions:\\
% \textbf{(RQ1)} Does the synergy between searching for ranking functions and invariants help prove termination of programs?\\
% \textbf{(RQ2)} How does our approach compare to the state of the art termination analysis algorithm overall?\\
% \textbf{(RQ3)} How do the parameters and approximations affect our code's performance?

\subsection{Benefits of Synergy}
% To show the benefits of synergistically guiding the search of invariants and ranking functions, we compare our technique to $\nu$Term. 
% We compare our implementation with $\nu$Term because we can fix the ranking function templates for both approaches to be the same and observe the effects of having the ranking function and invariant searches guide each other. 
% 
The neural network (NN) used in $\nu$Term consists of an input layer with program variables as the input and a single output representing the value of the ranking function for the input state. The NN contains one hidden layer, which is fully connected with ReLU activation. Overall, the neural network architecture represents a ranking function of the form $\sum_{i=1}^m\max(a_{i,0} + \sum_{j=1}^n a_{i,j}x_j,0)$, where $n$ is the number of program variables, $m$ is the size of the hidden layer and $a_{i,j} \in \mathbb{Z}$. We implement this template in our framework with the restriction $\sum_{i,j}|a_{i, j}| \leq k$.
Both $\nu$Term and our approach start by sampling a set of execution traces.  We vary the sample size used for both techniques. We fix the number of $\max$ terms in the ranking function, $m$, to 2 and $k = 10,000$.

In Table~\ref{table:nuterm2}, we present a comparison illustrating the number of benchmarks proven within the timeout using our methodology compared to $\nu$Term, both with and without their respective invariant generation algorithms. In the case of sample size 1000, when the invariants are not utilized, both methods prove the termination of a comparable number of programs. However, our approach, which strategically combines the search for ranking functions and invariants, proves termination for 23 additional programs. In contrast, $\nu$Term, relying on independently generated invariants, achieves termination proofs for only 13 additional programs.
% 
Further, when synergistically finding the ranking function and invariants, the average time to find a valid ranking function for a program reduces from 4.52 s to 3.49 s. The time reduces because the overhead of finding invariants is offset by reducing the number of ranking functions that have to be checked until one can be proved. On the other hand, when generating invariants separately, as is the case for $\nu$Term, the average time increases from 3.81 s to 4.08 s.
% $\nu$Term uses a template $\sum_i\max(a_{i,0} + \sum_j a_{i,j}x_j,0)$ for ranking functions where $x_j$ are program variables, $a_{i,j}$ are integer constants, and $i$ is a constant representing how many terms the ranking function can have. 
% First, we experiment with varying $i$ from 1 to 4 to see how our code and $\nu$Term's code compare for these templates. We present the number of benchmarks that each approach can prove in under 60 s with their respective invariant search algorithms, having the ranking function and invariant guide each other in our case and validating heuristic based fixed invariants in the case of $\nu$Term. To highlight the effects of the synergy in our approach, we also present the number of benchmarks each approach can prove in under 60 s without using any invariants. We modify our implementation never refine the invariant and always add the counter-example to $\rp$ at each Refine Phase, thereby going down only in the lattice $\latr$ and not in $\lati$.
% % We also present the average time both approaches take to see how they scale as the ranking function template increases. This experiment is summarized in Table~\ref{}.
% We also test how many initial samples each approach needs to prove termination efficiently. We vary the number of initial samples and present the number of benchmarks proved within 60 s and the average time taken to prove a benchmark. For this experiment, we set $i=2$.


% \begin{table}
% \centering
% \captionsetup{justification=centering}
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{@{}l | c c | c c c r@{}}
% \toprule 
% \text{ } & \multicolumn{2}{c}{No Invariants} & \multicolumn{4}{c}{With Invariants} \\  
% \text{Template } & Our Code & $\nu$Term & Our Code & Avg. Time & $\nu$Term  & Avg. Time\\
% \hline
% $i=1$ &57&57&92& 2.80&76 &3.86\\
% $i=2$ &85&82&108&3.49 &95&4.08\\
% $i=3$ &81&85&101& 3.97& 100&3.89\\
% $i=4$ &75&88&98& 5.09&102 &4.25\\
% \midrule
% \end{tabular}
% }
% \caption{Total number of methods proved and average time for template with $i$ max terms with and without supoprt for invariants.}
% \label{table:bounds}
% \vspace{-7mm}
% \end{table}

% \begin{table}
% \centering
% \captionsetup{justification=centering}
% % \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{@{}l | c | c@{}}
% \toprule 
% Algorithm & Without Invariants & With Invariants \\  
% \hline
% Our algorithm &85&108\\
% $\nu$Term &82&95\\
% \midrule
% \end{tabular}
% % }
% \caption{Total number of programs proved by our algorithm vs. $\nu$Term - with and without invariants with the parameters - $m = 2, k=10,000, T=1000$}
% \label{table:nuterm2}
% % \vspace{-7mm}
% \end{table}

We implemented 3 baseline versions of $\toolname$ to demonstrate the benefits of the way we guide the invariant and ranking function searches. First, we compare \toolname with a version that does not use the counter-examples from checking the ranking function to guide the invariant generation algorithm. Then, we compare \toolname with a version that does not use the counter-examples from checking the validity of candidate invariants to guide the generation of new candidate ranking functions. Next, we search for both a ranking function and an invariant that can prove the ranking function in one CEGIS loop. 


\begin{table}
\centering
\captionsetup{justification=centering}
% \resizebox{0.75\textwidth}{!}{
\begin{tabular}{@{}l | r  r | r  r|  r  r|  rr@{}}
\toprule 
\multirow{3}{*}{No. of samples} & \multicolumn{4}{|c|}{\toolname} & \multicolumn{4}{|c}{$\nu$Term} \\ 
& \multicolumn{2}{|c|}{Without invariants} & \multicolumn{2}{|c|}{With invariants} & \multicolumn{2}{|c|}{Without invariants} & \multicolumn{2}{|c}{With invariants}\\
& N & T (s) & N & T (s) & N & T (s) & N & T (s)\\ 
\hline 
250 & 84 & 3.36  & 108 & 2.74 & 82 & 3.34  & 90 & 2.75  \\
500 & 85 & 4.29  & 107 & 3.18 & 85 & 3.12  & 94 & 2.77  \\
1000 & 85 & 4.52  & 108 & 3.49 & 82 & 3.81  & 95 & 4.08  \\
% \hline
% Our algorithm &85&108\\
% $\nu$Term &82&95\\
\midrule
\end{tabular}
% }
\caption{Total number of programs proved by our algorithm vs. $\nu$Term - with and without invariants with the parameters - $m = 2, k=10,000, T=1000$, timeout=60 s. $N$ is the number of programs proved and T is the average time taken to prove the termination of a program.}
\label{table:nuterm2}
% \label{table:nuterm2}
% \vspace{-7mm}
\end{table}

To further demonstrate the benefits of synergy, we will look at two example programs that \toolname could prove are terminating. In Figure~\ref{}, we show a program that benefits from the ranking function search guiding the invariant search. The ranking function for this benchmark is $\max(x+1,0)$. The weakest sufficient invariant to prove that this ranking function is correct is $x-y \ge 1$. However, there are stronger invariants that could be found for this loop, such as $x - y > 40$ and $x - y = 42$. 
 

\subsection{Comparison Against State-of-the-art Algorithms}
% We compare our approach to Aprove~\cite{aprove}, Ultimate~\cite{ultimate}, DynamiTe~\cite{dynamite}, and $\nu$Term~\cite{nuterm} by running them on all of the benchmarks in our set with a timeout of 60 s. 
For each termination analysis algorithm, we present the number of benchmarks that \toolname could prove but the existing algorithm could not prove and also the number of benchmarks the existing algorithm could prove and \toolname could not prove in Figure~\ref{fig:sub-second}. For $\nu$Term and \toolname, we use the sample size that gives the best performance. We use 250 samples for our approach and 1000 for $\nu$Term.
% \yascom{Maybe we can change this to 250 initial samples because we prove the same number of programs and are significantly faster?} 
Notably, there is no benchmark for which $\nu$Term proves termination and \toolname does not. This is evidence that our approach is relatively effective when the ranking function is in the template we used to instantiate our algorithm.

We also present the total number of benchmarks that each algorithm could prove and the average time to prove one benchmark in Table~\ref{fig:sub-first}. Overall, Aprove can prove the most number of benchmarks within 60 seconds and our code can prove the second most. Aprove supports a wide variety of techniques, so our work can be incorporated into theirs to improve the performance on the subset of benchmarks for which our approach works better. We analyze such a case in Figure~\ref{evaluation:code}. Both Aprove, Ultimate and $\nu$Term cannot prove the termination of this program within 60 seconds. 
% The argument for termination is straightforward because in figure~\ref{}, $x$ keeps reducing till $x < y$ and in figure~\ref{}, $y$ keeps increasing till $y \ge x$, but the non-linear assignment statements in these benchmarks make analyzing them more difficult. 
DynamiTe proves termination for this program but it takes 8.7 s to prove it. 
\toolname proves the termination of this loop in 1.73 seconds.  The nonlinearity in this program makes it challenging for termination analysis because it is difficult to find invariants that can be used to prove the ranking function. However, the synergy used in our technique can find the appropriate invariant and can guide the search for the ranking function.  
% We also analyze a program for which Aprove can prove termination and our approach cannot in Figure~\ref{evaluation:code}. There is no valid ranking function for this code in the template we chose. We verify this by running a non-approximated version of our code as described in Section~\ref{sec:implementation}.
 % Note that the algorithms used in DynamiTe, Ultimate, and Aprove are orthogonal to our approach and hence, can be combined in the future to give better results.

% \begin{figure}
%     \begin{subfigure}{0.4\textwidth}
%         \centering 
%         \begin{lstlisting}[numbers=left,basicstyle=\ttfamily\footnotesize,backgroundcolor=\color{backcolour}]
% int res = 0;
% while (x >= y && y > 1) {
%     res++;
%     x = x/y;
% }

% \end{lstlisting} 
%         \caption{Java Code from LogIterative}
%         \label{evaluation:logiter}
%     \end{subfigure}
%     % \vrule
%     \begin{subfigure}{0.4\textwidth}
%         \centering 
%         \begin{lstlisting}[numbers=left,basicstyle=\ttfamily\footnotesize,backgroundcolor=\color{backcolour}]
% int res = 1;
% int y = 2;
% if (x < 0 || y <= 1) return 0;
% else {
%     while (x > y) { 
%         y = y*y;
%         res = 2*res;
%     }
% }

% \end{lstlisting} 
%         \caption{Java Code from LogMult}
%     \label{evaluation:code}
%         % \label{evaluation:logmult}
%     \end{subfigure}
%     % \caption{Two programs that could not be proved to terminate with Aprove or Ultimate within 60s.}
% \end{figure}

\begin{figure}
    \begin{minipage}{0.4\textwidth}
        \centering 
        \begin{lstlisting}[numbers=left,basicstyle=\ttfamily\footnotesize,backgroundcolor=\color{backcolour}]
int res = 1;
int y = 2;
if (x < 0 || y <= 1) return 0;
else {
    while (x > y) { 
        y = y*y;
        res = 2*res;
    }
}

\end{lstlisting} 
        \caption{An example program that can be proven by \toolname and not by Aprove, Ultimate, or $\nu$Term}
    \label{evaluation:code}
    \end{minipage}
    % \vrule
    \hspace{1cm}
    \begin{minipage}{0.4\textwidth}
        % \begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{sections/graph3.png}  
    % \caption{For each existing termination analysis algorithm, we show the number of programs our algorithm could prove that the existing algorithm could not and the number of programs that the existing algorithm proved that our algorithm could not within a timeout of 60 seconds.}
    \caption{Comparison with Existing State-of-the-art Techniques}
    \label{fig:sub-second}
  % \end{minipage}%
        % \label{evaluation:logmult}
    \end{minipage}
    % \caption{Two programs that could not be proved to terminate with Aprove or Ultimate within 60s.}
\end{figure}
 
% \begin{table}
% \centering
% \captionsetup{justification=centering}
% \resizebox{0.4\textwidth}{!}{
% \begin{tabular}{@{}l | c r@{}}
% \toprule 
% \text{ } & Total Proved & Average Time \\  
% \hline
% Our Code & 108 & 3.487 s\\
% Aprove & 113 & 5.336 s\\
% Ultimate & 105 & 4.261 s\\
% DynamiTe & 84 & 17.394 s\\
% $\nu$Term & 95 & 4.077 s\\
% \midrule
% \end{tabular}
% }
% \caption{Total number of benchmarks proved and average time for state-of-the-art termination analysis algorithms using a timeout of 1 minute.}
% \label{table:bounds}
% \vspace{-7mm}
% \end{table}
\begin{table}[]
    \begin{tabular}{@{}l r r@{}}
      \toprule 
      \text{ } & \toolname &  $\nu$Term \\  
      \hline
      Total proved & \textbf{104} &  96 \\
      Average time (s) & \textbf{4.13}  & 4.11 \\
      % Ultimate & 105 & 4.261 s\\
      % DynamiTe & 84 & 17.394 s\\
      % $\nu$Term & 95 & 4.077 s\\
      \midrule
    \end{tabular}
    \captionof{table}{Total number of benchmarks proved and the average time for $\nu$Term and \toolname using a timeout of 2 minutes. Both used a template with 2 summands and 1000 traces.}
    \label{fig:sub-first}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{@{}l  r   r  r  r@{}}
      \toprule 
      \text{ } & \toolname &  DynamiTe & Ultimate & Aprove \\  
      \hline
      Total proved & \textbf{155} &  124 & 147& 146\\
      Average time (s) & \textbf{4.09}  & 26.12  & 7.86  & 4.53\\
      % Ultimate & 105 & 4.261 s\\
      % DynamiTe & 84 & 17.394 s\\
      % $\nu$Term & 95 & 4.077 s\\
      \midrule
    \end{tabular}
    \captionof{table}{Total number of benchmarks proved and the average time for state-of-the-art termination analysis algorithms using a timeout of 2 minutes.}
    \label{fig:sub-first}
\end{table}



\begin{table}
\centering
\captionsetup{justification=centering}
% \resizebox{0.75\textwidth}{!}{
\begin{tabular}{@{}l | r | r | r | r | rr@{}}
\toprule 
 & (1,1) & (1,2) & (1,3) & (2,1) & (2,2) \\
\hline
Full Synergy &  103 & 147 & 151 & 124 & 135 \\
Without $p$ counter-examples &  91 & 134 & 140  &  & 115  \\
Without $q$ counter-examples &  89 & 139  & 141 &  & 129  \\
% \hline
% Our algorithm &85&108\\
% $\nu$Term &82&95\\
\midrule
\end{tabular}
% }
\caption{Total number of programs proved by our algorithm vs. $\nu$Term - with and without invariants with the parameters - $m = 2, k=10,000, T=1000$, timeout=60 s. $N$ is the number of programs proved and T is the average time taken to prove the termination of a program.}
\label{table:nuterm2}
% \label{table:nuterm2}
% \vspace{-7mm}
\end{table}

% \begin{figure}[ht]
%   \begin{minipage}{.5\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{sections/graph.png}  
%     \caption{Put your sub-caption here}
%     \label{fig:sub-second}
%   \end{minipage}%
%   \begin{minipage}{.5\textwidth}
%     \centering
%     \begin{tabular}{@{}l | c | c | c | c | r@{}}
%       \toprule 
%       \text{ } & Our Code & $\nu$Term & DynamiTe & Ultimate & Aprove \\  
%       \hline
%       Total proved & 108 & 113 & 105 & 84 & 95\\
%       Average time & 2.74 s & 5.54 s & 4.26 s & 17.39 s & 4.08 s\\
%       % Ultimate & 105 & 4.261 s\\
%       % DynamiTe & 84 & 17.394 s\\
%       % $\nu$Term & 95 & 4.077 s\\
%       \bottomrule
%     \end{tabular}
%     \captionof{table}{Total number of benchmarks proved and average time for state-of-the-art termination analysis algorithms using a timeout of 1 minute.}
%     \label{fig:sub-first}
%   \end{minipage}
% \caption{Put your caption here}
% \label{fig:fig}
% \end{figure}

% \begin{figure}
%     \centering
%             \begin{lstlisting}[numbers=left,basicstyle=\ttfamily\footnotesize,backgroundcolor=\color{backcolour}]
%     while (x > 0) {
%         x = -2*x + 10;
%     }

% \end{lstlisting} 
%     \caption{An example program that can be proved by Aprove and DynamiTe, but not by our implementation.}
%     \label{fig:enter-label}
% \end{figure}


% First, we compare our implementation with $\nu$Term, a termination analysis framework that finds ranking functions in the form $\max(a_1x_1+a_2x_2 + \cdots + a_n, 0) + \max(b_1x_1+b_2x_2 + \cdots + b_n, 0) + \cdots$. In $\nu$Term, ranking functions are learnt in the form of small neural networks from a set of generated traces. Then, the validity of these ranking functions are checked using an SMT call. In this work, specific invariants functions in the forms $x_i > 0$ and $x_i \ge 0$ are proposed and checked. If any of these invariants are proved to be correct invariants, then they are used when checking the validity of the ranking function. In order to compare our code to $\nu$Term, we first compare the approaches without the invariant synthesis functionality. Then, we compare $\nu$Term with its static invariant generation to our code with its combined ranking function and invariant search. We will fix the ranking funciton templates to be equal, first with 2 max terms, then with 4 max terms. For each experiment, we present the total number of methods for which termination was proved and the average time to prove termination.

% We also compare our implementation to the state of the art termination analyses, Aprove, Ultimate, and Dynamite. For each of these frameworks, we present the total number of methods for which termination is proved, the number of methods the framework proved that our implementation could not and the number of methods that our implementation could prove that the framework could not.

% \begin{table}
% \centering
% \captionsetup{justification=centering}
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{@{}l | c c | c r@{}}
% \toprule
% \text{ } & \multicolumn{2}{c}{No Invariants} & \multicolumn{2}{c}{With Invariants} \\  
% \text{ } & Total Proved & Avg. Time & Total Proved & Avg. Time \\  
% \hline
% $\nu$Term &  \\
% SymTerm & \\
% \midrule
% \end{tabular}
% }
% \caption{Total number of methods proved and average time for template with 2 max terms.}
% \label{table:bounds}
% \vspace{-7mm}
% \end{table}

% \begin{table}
% \centering
% \captionsetup{justification=centering}
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{@{}l | c c | c r@{}}
% \toprule
% \text{ } & \multicolumn{2}{c}{No Invariants} & \multicolumn{2}{c}{With Invariants} \\  
% \text{ } & Total Proved & Avg. Time & Total Proved & Avg. Time \\  
% \hline
% $\nu$Term &  \\
% SymTerm & \\
% \midrule
% \end{tabular}
% }
% \caption{Total number of methods proved and average time for template with 4 max terms.}
% \label{table:bounds}
% \vspace{-7mm}
% \end{table}

% \begin{table}
% \centering
% \captionsetup{justification=centering}
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{@{}l c c c r@{}}
% \toprule
% \text{ } & Total Proved &  Avg. Time & Only Proved by & Only Proved by\\  
% \text{ } & &  & Existing Code & Our Code \ \ \ \ \\ 
% \hline
% Aprove &  \\
% Ultimate & \\
% DynamiTe & \\
% \midrule
% \end{tabular}
% }
% \caption{Total number of methods proved and average time for template with 4 max terms.}
% \label{table:bounds}
% \vspace{-7mm}
% \end{table}



==> sections/general.tex <==
\section{General Algorithm}
\begin{definition}
    An invariant template $\tempi$ is a given set of candidate invariants.
\end{definition}

\begin{definition}
    A ranking function template $\tempr$ is a given set of candidate ranking functions.
\end{definition}

We present an algorithm that, given a ranking function template, $\tempr$, and an invariant template, $\tempi$, and a loop $\langle \init, \guard, \trans \rangle$, will find a ranking function in $\tempr$ that is valid with w.r.t. $\guard, \invar, \trans$ where $\invar \in \tempi$. The algorithm has two main steps, a generate phase and a refine phase. We will define lattices based on $\tempr$ and $\tempi$ to demonstrate how the algorithm makes progress towards finding a valid ranking function in each step. Then, we will present the algorithm. We will also prove that if the invariant template is closed under intersection and both templates are finite and fit into a decidable SMT theory, the algorithm is complete.

\subsection{Lattice Structures}
We can define lattices corresponding to the search for the ranking function and the invariant to demonstrate the progress that is made in each step.

\begin{definition}
    $\latrfs$ is a meet semi-lattice on the powerset of all possible ranking functions in $\tempr$: $\latrfs = (\mathcal{P} ({\tempr})\preceq, \wedge)$, where $\mathcal{F}_1 \preceq \mathcal{F}_2 \triangleq \mathcal{F}_1 \subseteq \mathcal{F}_2$ and $\mathcal{F}_1 \wedge \mathcal{F}_2 \triangleq \mathcal{F}_1 \cap \mathcal{F}_2$
\end{definition}

\begin{definition}
    $\lati$ is a meet semi-lattice such that $\lati = (\tempi, \preceq, \wedge)$, where $\invar_1 \preceq \invar_2 \triangleq \invar_1 \subseteq \invar_2$ and $\invar_1 \wedge \invar_2 \triangleq \invar_1 \cap \invar_2$
\end{definition}

\subsection{Full Algorithm}
The state of the algorithm is defined by $\langle \rp, \invar \rangle$. At the beginning, $\invar$ is the set of all program states, $\top$ in $\lati$. $\rp$ is initialized to a set of reachable program states at the location in the program directly after the loop guard, before the body of the loop. These states are randomly sampled from random traces of the loop. Given $\tempr$, $\rp$ corresponds to an element in $\latrfs$. As shown in Figure~\ref{fig:overview}, the algorithm iteratively refines the state to better approximate $\reachp$. In each iteration, progress is made going down one of the two lattices in each refine phase. Below is an overview of the algorithm:\\

\begin{algorithmic}[1]
\Procedure{$\fr$}{$\rp, \invar$}
    \State $f \gets \gc(\rp)$
    \If{$\checkr(f, \invar)$} 
        \State \Return f
    \Else
        % \State $c \gets \gcounter(f, \invar)$
        % \State $\invar' \gets \invar$
        % \State $c' \gets c$
        \While{$\true$}
            \State $c \gets \gcounter(f, \invar)$
            \State $\text{is\_refined}, \; \invar \gets \mathsf{refine}(\invar, c)$
            \If{$\text{is\_refined}$}
                \If{$\checkr(f, \invar)$} 
                    \State \Return f
                % \Else 
                %     \State $c \gets \gcounter(f, \invar')$
                \EndIf
            \Else
                \State $\rp \gets \rp \cup \{c\}$
                % \State $\fr(\rp_{new}, \; \invar)$ 
                \State $f \gets \gc(\rp)$
                \If{$\checkr(f, \invar)$} 
                    \State \Return f
                \EndIf
            \EndIf
            
            
        \EndWhile
    \EndIf 
\EndProcedure
\end{algorithmic}

In the above algorithm, $\gc(\rp)$ returns a ranking function that is bounded by 0 and decreases by at least 1 when executing the loop $\langle \init, \guard, \trans \rangle$ on each of the states in $\rp$. This is found using the following SMT query: $$\forall X \in \rp, \forall X' \in \trans(X) \cdot \rf(X) - \rf(X') \geq 1 \wedge \rf(X) \geq 0 $$
Here $\rf$ is a symbolic expression that represents a ranking function in $\tempr$. The only symbolic variables in this query represent the constants in the ranking function. The program states are not symbolic since they are from $\rp$. If this query is unsatisfiable, then there does not exist a ranking function that is bounded and decreasing by at least 1 for every element of $\rp$. Since this is a necessary condition for a ranking function to be valid w.r.t. $\guard, \invar, \trans$, the algorithm terminates, showing that there is no ranking function in $\tempr$ that is valid w.r.t. $\guard, \invar, \trans$ for $\invar \in \tempi$. If the query is satisfiable, then we have a candidate ranking function, $f$.

We now have to check whether $f$ is bounded and decreasing on $\reachp$. Since $\reachp$ is hard to express and $\reachp \subseteq \invar$, in the function $\checkr(f, \invar)$, we check whether $f$ is bounded and decreasing on $\invar$.  $\checkr(f, \invar)$ uses an SMT call where the ranking function constants are not symbolic, but the program state is symbolic. Checking the validity of $f$ w.r.t $\guard, \invar, \trans$ is equivalent to checking the validity of the following statement:
$$\forall X, (\forall X' \in \trans(X), f(X) - f(X') \geq 1 \wedge f(X) \geq 0)$$
This is the SMT query used in $\checkr(f, \invar)$: $$\exists X, (\exists X' \in \trans(X), f(X) - f(X') < 1 \vee f(X) < 0)$$
Note that, when $\guard(X)$ is false, $\trans(x) = \emptyset$, so if this symbolic expression is satisfiable, the satisfying assignment to $X$ will be a state that satisfies the loop guard. If this query is unsatisfiable, then we have proved the validity of $f$ and terminate the algorithm having found a valid ranking function. Otherwise, the satisfying assignment to $X$ is counter-example disproving the validity of $f$. This counter-example is returned by $\gcounter$ and assigned to $c$. 

 After checking the validity of the first candidate ranking function, we enter a loop where in each iteration, we refine the state. First, in line 8, we try to find $\invar'$ such that $\invar'$ is a valid invariant and $\invar' \prec \invar$ and change the algorithm state to $\langle \rp, \invar' \rangle$. If this is not possible, in line 14, we change the algorithm state to $\langle \rp \cup \{c\}, \invar \rangle$. We can prove that $\rp \cup \{c\} \prec \rp$. When refining the algorithm state, we first call $\mathsf{refine}(\invar, c)$. This function is defined below.\\ 
 
% \begin{algorithmic}[1]
% \Procedure{$\mathsf{refine}$}{$\invar, c$}
%     \State $\mathsf{inv\_cex}$ = []
%     \State $\invar' \gets \gi(\rp, c, \mathsf{inv\_cex})$
%     \If{$\checki(\invar')$} 
%         \State \Return t, $\invar$
%     \Else
%         \While{$\true$}
%             \State $c_i, \mathsf{for\_precondition} \gets \gcounterinv(\invar')$
%             \If{$\mathsf{for\_precondition}$}
%                 \State $\invar' \gets \gi(\rp \cup \{c_i\}, c, \mathsf{inv\_cex})$
%             \Else
%                 \State $\invar' \gets \gi(\rp, c, \mathsf{inv\_cex} \cup \{c_i\})$ 
%             \EndIf
%             \If{$\checki(\invar')$} 
%                 \State \Return t, $\invar' \cap \invar$
%             \EndIf
%         \EndWhile
%     \EndIf 
% \EndProcedure
% \end{algorithmic}



\subsection{Proofs}

==> sections/intro-backup.tex <==
\section{Introduction}
Termination analysis is one of the most challenging components of program verification. 
Several techniques for automatically proving termination or non-termination have been explored in the past. These include using various reduction orders, finding recurrent sets, fixpoint logic solving,  etc, using static or dynamic analyses or a combination of both~\cite{aprove, ultimate, dynamite}.
% These techniques exhibit notable performance, but their usability is limited to simple programs including linear assignments and boolean guards, and relatively easier control flow graphs. The dependence of these methods on the program structure prohibits them from providing completeness guarantees in more general cases. 
% This is far from real-world programs which often involve non-linear assignments and complex structures including nested loops and loop sequencing in arbitrary order. 
Finding \textit{ranking functions} is one of the most widely used techniques to prove the termination of programs.  Ranking functions have the property that they are bounded from below for all reachable program states and decrease by a certain amount in each iteration. This poses a problem because computing the exact set of reachable states is undecidable. As a solution, loop invariants are typically used as an over-approximation of the reachable states. Conversely, for checking the validity of a given ranking function, we do not need the strongest invariant. Instead, we need to synthesize an invariant that is \textit{strong enough} to prove the validity of the ranking function. 

% The recent advancement in synthesizing \textit{ranking functions} from the concrete execution traces of programs on randomly generated inputs provides new avenues for limiting the dependence of termination analysis on the program structure and enabling support for analyzing more complicated programs (e.g., non-linear arithmetic, arbitrarily nested loops, etc.)~\cite{nuterm, dynamite}. 
So, to prove the termination of a program, there are two unknowns - the ranking function and the set of reachable states (or a strong enough invariant). Consequently, compared with classical property-guided synthesis~\cite{propinvar,pdr}, we do not have direct access to the target property (a ranking function or an invariant). Instead, we only know the properties of what we are searching for, i.e., the ranking function must be bounded and must reduce on all reachable states, and the invariants must subsume the initial program states and must be inductive. %Finding a way to guide the search for invariants to support termination arguments is non-trivial.


% In some of the existing termination analysis techniques \cite{nuterm, dynamite}, the synthesis of invariants is independent of the synthesis of ranking functions. For example, in \cite{nuterm}, the validity of hard-coded invariants is checked and subsequently utilized. In ~\cite{dynamite}, the invariant generation is outsourced to an external solver, which is not guided by the termination analysis. Because of the independence, these techniques
% can \textcolor{red}{fail} to synthesize the necessary invariants to prove the validity of candidate ranking functions within a reasonable time frame. Another limitation of these existing methods is that they do not provide any completeness guarantees.

% In other techniques\cite{chc}, the synthesis for ranking functions and reachable states is 
% reduced to checking the satisfiability of a formula expressed in fixpoint logic. Although these techniques are usually accompanied by relative completeness guarantees and searching for solutions to this formula leads to a more guided search for both of them, the coupling makes the task more computationally expensive to solve because the search space of the combined query is the product of the individual search spaces. 

In some existing termination analysis techniques \cite{nuterm, dynamite}, the synthesis of invariants is independent of the synthesis of ranking functions. For instance, in \cite{nuterm}, the validity of hard-coded invariants is checked and subsequently utilized, while in ~\cite{dynamite}, the invariant generation is outsourced to an external solver, not guided by the termination analysis. Due to this independence, these techniques may fail to synthesize necessary invariants to prove the validity of candidate ranking functions within a reasonable time frame. Another limitation is the lack of completeness guarantees. Conversely, in other techniques \cite{chc}, synthesis for ranking functions and reachable states is reduced to checking the satisfiability of a formula expressed in fixpoint logic. Although these techniques often come with relative completeness guarantees, the coupling makes the task computationally expensive due to the product of individual search spaces in the combined query.
% 
These methodologies represent two ends of a spectrum, each with its drawbacks and proposed solutions. On one end, techniques like ~\cite{terminator} utilize insights to guide the invariant search based on the current state of the ranking function, potentially providing a good starting point. On the other end, exact solutions to the combined problem require navigating a large search space. Instead, some techniques ~\cite{popl23} compute approximations of fixpoints iteratively improved until convergence, balancing between over-approximation and under-approximation.







% The above two methodologies can be treated as two ends of a spectrum with their disadvantages and proposed solutions. In the first kind of technique, an insight is that one needs specific invariants that can be used to check the validity of the generated ranking function. Techniques like \cite{terminator} rely on this insight and use the current state of the ranking function to guide the invariant search. This potentially provides a good starting state for the invariant search. 
% % 
% On the other end of the spectrum, finding an exact solution to the combined problem of finding a ranking function and the reachable states requires navigating a large search space. Instead of the exact solutions, some proposed techniques~\cite{popl23}compute an approximation of the fixpoints as a primal problem. And conversely, find an under-approximation of the dual problem, i.e., non-termination. These approximations can then be iteratively improved until convergence. 



% to prove the validity of a ranking function as their invariant 
%either take a lot of time to compute invariants that are strong enough to prove the validity of a ranking function or synthesize weak invariants.  
% 

\textbf{Synergy. }We argue that for a given program, although the search for ranking functions and the corresponding invariants must not be agnostic of each other, directly encoding them as a monolithic query can make each step of the search expensive. So, we propose a framework where they are still searched using separate subroutines, but the information gained by each is used by the other, leading to more guided searches. 
Consider a program and a candidate ranking function that cannot prove its termination. So, we will get a counterexample (a program state) where the ranking function does not reduce on executing the loop body starting at the counterexample. However, there are two possibilities - (i) the counterexample program state is unreachable, (ii) the ranking function is invalid. As a first step, assuming that the ranking function is correct, we must search for a new invariant guided by the fact that it must also exclude the current counterexample.  If no possible invariant can exclude it from the above step, we can still use the invariant search to guide the ranking function search. While trying to search for an invariant that excludes the counter-example, the CEGIS loop generates some program states that are conclusively reachable. These states guide the search for a new candidate ranking function.

\textbf{Multiple Loops. }When dealing with multiple loops (nested or sequential) in a single program, the problem increases even further. All the loops in the program must terminate, however, the search for ranking functions and corresponding invariants cannot be independent across different loops. For instance, in the case of nested loops, the invariant of the outer loop defines the over-approximation of the initial set of the inner loop. So, the inner invariant depends on the precision of the outer invariant, and thus also affects the inner ranking function. Conversely, the inner invariant describes the over-approximated transition relation of the outer loop's body and thus affects the search for the outer invariant and ranking function. On the other hand, it is also inefficient to encode all the invariants and the ranking functions as a single query because of the large search space. To address this problem, in addition to having synergy between the searches for ranking function and invariant for one loop, we also use the information from the invariant search in each loop to guide the searches for ranking functions and invariants of other loops in the program.


% In the case of nested loops, there is an additional complication. the ranking functions and invariants that can be found for one loop depend on the invariants found for other loops in a program. Therefore, the searches for ranking functions and invariants for each loop must obtain information from the searches for the invariants of the other loops.
% For single loops, the exact transition relation of the loop body is known, but it is harder and sometimes not possible to compute the transition relation of a loop body that contains additional loops.
% % In the case of nested loops, this problem is even more exacerbated because the presence of loops in the body of outer loops makes it harder to compute its transition relation. 
% In such settings, the invariant of an inner loop is not only needed for the termination of the inner loop but is also needed to reason about the termination of the outer loop. Further, one property of invariants is that they have to subsume the set of states in which the loop may start. This is straightforward in the case of single loops, but with nested loops, the invariants of outer loops affect our estimation of the starting states of inner loops. 
% % These 3 qualities of invariants, over-approximating the reachable states, over-approximating the transition relation, and inclusion of the $\textit{Init}$ set, coupled with the ability to prove
% Finding invariants for all loops (arbitrarily nested) that over-approximate the reachable states, over-approximate the transition relation, include approximations for the starting states of loops, and have the ability to prove the validity of ranking functions is a hard task.

\textbf{This Work.} We introduce a new, general, framework called \toolname, based on a synergistic synthesis of ranking functions and invariants for efficient termination analysis of complex programs containing arbitrary nested loops, disjunctive conditionals,  and non-linear statements. \toolname is data-driven and synthesizes ranking functions from execution traces which makes it less dependent on the exact structure of the loop. It is parameterized by a set of possible invariants $\Gamma$ and a set of possible ranking functions $F$ and can be instantiated with different choices of these sets to obtain different termination analyses. For each loop, counter-examples from the invariant search guide the ranking function search and counter-examples from the ranking function search guide the invariant search. Further, the invariant and ranking function searches for each loop are guided by the analyses of the other loops in the program. Under computability assumptions and assumptions on the structure of $\Gamma$ and $F$, we guarantee completeness: for a given program $P$, if there is a termination proof using the invariants in $\Gamma$ and ranking functions in $F$, then \toolname will find a ranking function $f \in F$ that is valid under an invariant $I \in \Gamma$ for every loop in $P$.% The main idea behind our approach is the .
%Here, for a candidate ranking function, we iteratively try to synthesize invariants such that every new invariant has a higher chance of proving the validity of the given ranking function than the previous one. If no invariant can be found, then that serves 
%Instead, prior knowledge of the target of proving termination can guide the search to synthesize appropriate invariants. 

% \textbf{Challenges. }
We also provide an instantiation of the general framework and introduce some approximations to make the process more efficient. In this instantiation, we are able to increase the information from the invariant search that guides the ranking function search by not only utilizing reachable states, but also counter-example states that may not be reachable. 
% With these optimizations, our implementation of the general framework can match the performance of state-of-the-art termination analysis engines.


% Compared with classical property-guided synthesis~\cite{propinvar,pdr}, we do not have direct access to the target property (a ranking function). Instead, we only know the features of what we are searching for, i.e., the ranking function must be bounded and must reduce on all reachable states. %Finding a way to guide the search for invariants to support termination arguments is non-trivial.
% In the case of nested loops, there is an additional complication.
% For single loops, the exact transition relation of the loop body is known, but it is harder and sometimes not possible to compute the transition relation of a loop body that contains additional loops.
% % In the case of nested loops, this problem is even more exacerbated because the presence of loops in the body of outer loops makes it harder to compute its transition relation. 
% In such settings, the invariant of an inner loop is not only needed for the termination of the inner loop but is also needed to reason about the termination of the outer loop. Further, one property of invariants is that they have to subsume the set of states in which the loop may start. This is straightforward in the case of single loops, but with nested loops, the invariants of outer loops affect our estimation of the starting states of inner loops. 
% % These 3 qualities of invariants, over-approximating the reachable states, over-approximating the transition relation, and inclusion of the $\textit{Init}$ set, coupled with the ability to prove
% Finding invariants for all loops (arbitrarily nested) that over-approximate the reachable states, over-approximate the transition relation, include approximations for the starting states of loops, and have the ability to prove the validity of ranking functions is a hard task.
% Reasoning about the loops in isolation also causes challenges because an invariant strong enough to prove the termination of a loop may not be strong enough for the proof of termination of the overall program. It is not clear how to simultaneously drive the search for multiple loop invariants such that they are sufficient to find (and validate) a ranking function.

% One method for demonstrating the termination of nested loops involves initially establishing the termination of the inner loop in isolation. Subsequently, by utilizing the inner loop's invariant, one can then establish the termination of the outer loop. However, in this case, apart from the challenges of finding a strong enough invariant for the outer loop, the invariant of the inner loop might also be too weak for overall termination analysis. It is not exactly clear how to simultaneously drive the search for both invariants such that the pair of invariants is sufficient to find (and validate) a ranking function. This problem further increases for arbitrary nesting of loops.

% Therefore, this approach may not always yield invariants that are useful for finding or validating a ranking function. In fact, it has been observed that discovering invariants guided by a specific property to be proven is more beneficial than independently finding invariants (\cite{}).

% Another limitation of existing termination algorithms is the lack of theoretical guarantees. Some termination analysis algorithms~\cite{} are proven to be complete, but these are restricted to linear ranking functions, linear invariants, linear programs, or some combination of these. However, this does not cover programs with non-linear assignment statements and loop guards. On the other hand, the termination analysis algorithms~\cite{} that go beyond these restrictions provide limited theoretical guarantees on the completeness of their approach. 

% \noindent
% \textbf{Key Observations. }
% An invariant serves as an over-approximation of the set of reachable states and can be used to construct an over-approximation of the transition relation. 
% % So, a valid ranking function for a loop, must also reduce and be bounded on the execution traces, which leads us to a necessary condition for the validity of a ranking function. 
% So, if a function reduces and is bounded on the invariant and the transition system computed using invariants, then it also must be valid for the loop. This gives us a sufficient condition for the validity of a ranking function. A set of states from execution traces serves as an under-approximation of the reachable states. So, if a function is a valid ranking function for a loop, it must be bounded and reducing on the program states from execution traces. This gives us a necessary condition for the validity of a ranking function. Using this under-approximation, we can generate possible ranking functions and check their validity using the over-approximation of the reachable states. The set of states included in the invariant for which a function, $f$, is not bounded or not reducing can be used to either guide the refinement of the invariant or guide $f$ to satisfy the conditions of being bounded and reducing on more of the reachable states. Using this set to guide both the ranking function search and the invariant search allows both searches to converge faster than simply iterating between the two approximations without having them guide each other.



\textbf{Main contributions}:
\begin{itemize}
    \item We provide a general recipe for the synergistic synthesis of invariants and ranking functions in the form of a framework called \toolname, which can be instantiated with different templates for ranking functions and invariants. To do this, we introduce the concept of an \textit{annotated program} with which we build the necessary formalism needed for synergistic search. \toolname handles complex programs with arbitrarily nested loops, disjunctive conditionals, and non-linear statements. %An annotated program formalizes how invariants can be used to 
    %model the set of reachable states, the transition relation for the loop body, and the $\text{Init}$ sets for inner loops.
    \item We prove relative completeness guarantees for \toolname. For a program, if there exists a ranking function and an invariant in their respective $\textit{templates}$ and there exist complete procedures for the template-specific functions in our algorithm, then our algorithm will prove the termination of the program.
    \item We provide an instantiation of our framework \toolname and evaluate it against the state-of-the-art baselines. We observe that by only finding ranking function termination arguments, we can already match the performance of the state-of-the-art termination analysis tools, which are combinations of many different kinds of termination arguments. In some cases, we can prove the termination of programs which even \cite{aprove} cannot. ????
\end{itemize}


% 
% We will describe how we find invariants to support termination arguments and the need for formal guarantees about completeness using the following observations.
% Given a loop program $L = \texttt{while}(\beta) \texttt{ do }\pro \texttt{ od}$ where $\prog$ is loop-free, let $\reach$ and $\llbracket \prog \rrbracket$ denote the set of reachable states at the beginning of $L$ and a relation capturing the semantics of the loop body $\prog$. One way to prove the termination of $L$ is to find a function $f$ s.t. $f$ is a valid ranking function for $L$ w.r.t $(\reach, \bracs \prog)$. Consider $r, R$ that are under-approximation and over-approximation of $\reach$ respectively, i.e., $r \subseteq \reach \subseteq R$. Note that if $f$ is a valid ranking function for $L$ w.r.t $(\reach, \bracs \pro)$, then it must also be valid w.r.t $(r, \bracs \pro)$. This is thus a necessary condition for the validity of a ranking function w.r.t ($\reach, \bracs \pro$). Similarly, the validity of $f$ w.r.t $(R, \bracs \pro)$ is a sufficient condition for its validity w.r.t $(\reach, \bracs \pro)$. 

% Given a loop program $L = \texttt{while}(\beta) \texttt{ do }\pro \texttt{ od}$, let $\reach \subseteq S$ and $\llbracket \prog \rrbracket \subseteq S \times S$ denote the set of reachable states at the beginning of a loop program $L$ and a relation capturing the semantics of the loop body $\prog$. One way to prove the termination of $L$ is to find a function $f$ s.t. $f$ is a valid ranking function for $L$ w.r.t $(\reach, \bracs \prog)$. Consider $r, R$ that are under-approximation and over-approximation of $\reach$ respectively, i.e., $r \subseteq \reach \subseteq R$, and $t, T$ which are under and over-approximation of $\llbracket \prog \rrbracket$, i.e., $t \subseteq \llbracket \prog \rrbracket \subseteq T$. Note that if $f$ is a valid ranking function for $L$ w.r.t $(\reach, \bracs \pro)$, then it must also be valid w.r.t $(r, t)$. This is thus a necessary condition for the validity of a ranking function w.r.t ($\reach, \llbracket P \rrbracket$). Similarly, the validity of $f$ w.r.t $(R, T)$ is a sufficient condition for its validity w.r.t $(\reach, \llbracket P \rrbracket)$. 
% Such an over-approximation of the reachable states ($R$) is often captured by invariants of the program ($\invar$).

% As noted in Section~\ref{sec:background}, a ranking function must be \textit{Bounded} and \textit{Reducing} w.r.t. reachable states at the beginning of the loop and a transition relation that exactly captures the program semantics. If a function is bounded and reducing on the set of reachable states ($\reach, \trans$), it is also bounded and reducing on an under-approximation of the reachable states and the exact transition relation ($r,t$ such that $r \subseteq \reach \wedge t \subseteq \trans$). Further, if a function is bounded and reducing on an over-approximation of the reachable states and the exact transition relation ($\reach', \trans'$ such that $\reach \subseteq \reach' \wedge \trans \subseteq \trans'$), then it is also bounded and reducing on the reachable states. Such an over-approximation of the reachable states is often captured by invariants.
% Given a  relation $T \subseteq S \times S$, 

% For a function $f$, let $sat(f)  = \{s \ | \ f(s) \geq 0 \wedge f(s) - f(\bracs \pro s) \geq 1\}$.  
% Given a valid invariant($\invar$) for $\prog$, $f$ can prove the termination of $L$ iff $\invar \subseteq sat(f)$. If this is not the case, then the set $X = \invar \setminus sat(f)$ can be used to refine either $\invar$ or $f$. For each element, $s \in X$, there are two cases (i) $s$ is not a reachable state for $L$, in which case, we can try to refine $\invar$ to exclude $s$, or (ii) $s$ is reachable, so, $f$ must be modified appropriately to also be valid on $(s, \bracs \pro s)$.  Therefore, $f$ and $\invar$ can guide each other through the common goal of making $X$ empty and thus finding a valid ranking function and an inductive invariant for the program. We exploit this synergy in our algorithm.

% Note that the above intuition can be generalized to nested loops, where the program $\pro$ is not loop-free. In this case, if $\bracs \pro$ is under-approximated and over-approximated by $t$ and $T$ respectively, then the validity of $f$ w.r.t $(r, t)$ and validity of $f$ w.r.t $(R, T)$ are respectively the necessary and sufficient conditions for proving the termination of $L$. In this case, the definition of $sat(f)$ can be defined as a set of pairs of states on which $f$ reduces, and therefore the difference $X = T \setminus sat(f)$ can be used to guide a more precise under and over-approximations of $\bracs \pro$.

% Moreover, it is easier to synthesize candidate ranking functions w.r.t a subset of reachable states ($r$), as opposed to the complete set of reachable states. Additionally, an invariant, ($\invar$) over-approximates the set of all reachable states and can be represented using a system of equalities and inequalities. Consequently, the validity of a ranking function w.r.t an invariant can be simplified to checking the satisfiability of a first-order formula. We capitalize on these advantages in our algorithm and precisely outline how we utilize under-approximation and over-approximation to synergistically guide the search for ranking functions and invariants.

==> sections/newbg.tex <==
\begin{grammar}
<Expression> $e$ ::= $c$ | $x$ | $e_1 \oplus e_2$ | $\cdots$

<Atomic statements> $\alpha$ ::= $\texttt{skip}$ | $x \leftarrow e$

<Program> $\pro$ ::= $\alpha$ | $\texttt{while}(\beta) \texttt{ do }\pro \texttt{ od}$ | $\pro_1$ ; $\pro_2$ | $\texttt{if}(\beta) \texttt{ then } \prog_1 \texttt{ else }\prog_2$

<Invariant> $\invar$ ::= set of program states

<Annotated Program> $\anno$ ::= $\alpha$ | $\invar \ @ \ \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od}$ | $\anno_1$ ; $\anno_2$ | $\texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2$

<Doubly Annotated Program> $\annoc$ ::= $\alpha$ | $\invar \ @ \ \texttt{while}(\beta) \texttt{ do }\annoc \texttt{ od } c$ | $\annoc_1$ ; $\annoc_2$ | $\texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2$
\end{grammar}

\subsection{$\bracs{\anno}$}
\begin{align*}
    \bracs{\alpha} &\triangleq \bracs{\alpha} \\
    \bracs{\invar \ @ \ \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od}} &\triangleq \invar \times (\invar \cap \llbracket \neg \beta \rrbracket) \\
    \bracs{\anno_1 ; \anno_2} &\triangleq \bracs{\anno_1} \circ\bracs{\anno_2} \\ 
    \bracs{\texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2} &\triangleq \eye(\bracs{\beta}) \circ \bracs{\anno_1} \cup \eye(\bracs{\neg\beta}) \circ \bracs{\anno_2}  
\end{align*}

% \subsection{$\trans(\prog, \anno)$}
% \begin{align*}
%     \trans(\alpha, \cdot) &\triangleq \llbracket \alpha \rrbracket \\
%     \trans(\texttt{while }(\beta) \texttt{ do }\pro \texttt{ od}, \invar @\anno_1) &\triangleq \invar \times (\invar \cap \llbracket \neg \beta \rrbracket) \\
%     \trans(\prog_1 ; \prog_2, \anno_1 :: \anno_2) &\triangleq \trans(\prog_1, \anno_1) \circ \trans(\prog_2, \anno_2)
% \end{align*}

\subsection{$\core{\anno}$}
\begin{align*}
    \core{\alpha} &\triangleq \alpha \\
    \core{(\invar \ @ \ \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od})} &\triangleq \texttt{while}(\beta) \texttt{ do } \core{\anno} \texttt{ od} \\
    \core{(\anno_1 ; \anno_2)} &\triangleq \core{\anno_1} ; \core{\anno_2} \\
    \core{(\texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2)} &\triangleq \texttt{if}(\beta) \texttt{ then } \core{\anno_1} \texttt{ else } \core{\anno_2} \\
\end{align*}

\subsection{$\core{\annoc}$}
\begin{align*}
    \core{\alpha} &\triangleq \alpha \\
    \core{(\invar \ @ \ \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od } c)} &\triangleq \invar \texttt{while}(\beta) \texttt{ do } \core{\anno} \texttt{ od} \\
    \core{(\annoc_1 ; \annoc_2)} &\triangleq \core{\annoc_1} ; \core{\annoc_2} \\
    \core{(\texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2)} &\triangleq \texttt{if}(\beta) \texttt{ then } \core{\annoc_1} \texttt{ else } \core{\annoc_2} \\
\end{align*}

% \subsection{$\step(\ini, \prog, \anno)$}
% \begin{align*}
%     \step(\ini, \prog, \anno) = \{y \ | \ \exists x \in \ini \cdot (x, y) \in \trans(\prog, \anno)\}
% \end{align*}

\subsection{Validity of ranking function and annotated program w.r.t init set}

% \begin{figure}
% \raggedright
    % \fbox{$\ini, \prog \models \anno$}
    % \resizebox{\textwidth}{!}{
    $
    \begin{array}{c}
        % \hspace{3cm}
        \inferrule*[lab={\footnotesize{\textsc{Atomic statements}}}]
        {
        }
        {
        \ini \models \alpha
        } 
        \hspace{1cm}
        \inferrule*[lab={\footnotesize{\textsc{Loop}}}]
        {
        \ini \subseteq \invar \\\\
        % \eye(\invar \cap \bracs{\beta}) \circ \bracs{\anno_1} \subseteq \invar \\\\
        (\invar \cap \bracs{\beta}) \circ \bracs{\anno_1} \subseteq \invar \\\\
        \invar \cap \bracs{\beta} \models \anno_1
        }
        {
        \ini \models \invar @ \texttt{while }(\beta) \texttt{ do }\anno_1 \texttt{ od}
        } 
        \hspace{1cm} 
        \inferrule*[lab={\footnotesize{\textsc{Sequence}}}]
        {
        \ini \models \anno_1 \\\\
        \ini \circ \bracs{\anno_1} \models \anno_2 
        % \post(\eye(\init) \circ \bracs{\anno_1}) \models \anno_2
        }
        {
        \ini \models \anno_1 ; \anno_2
        } 
        \\\\
        \inferrule*[lab={\footnotesize{\textsc{If}}}]
        {
        \ini \cap \bracs{\beta} \models \anno_1 \\\\
        \ini \cap \bracs{\neg\beta} \models \anno_2
        }
        {
        \ini \models \texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2
        } 
        \hspace{1cm} 
        \inferrule*[lab={\footnotesize{\textsc{Ranking function}}}]
        {
        \ini \models \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od} \\\\
        \forall (x, x') \in \bracs{\anno} \cdot \big( \rf(x) - \rf(x') \geq 1 \big) \wedge \big(\rf(x) \geq 0\big)
        }
        {
        \ini \models \texttt{while}(\beta) \texttt{ do }\anno \texttt{ od}, \rf
        } 
    \end{array}
    $
    % }
%     \caption{Validity of Annotations}
%     \label{fig:annovalid}
% \end{figure}


\subsection{$\consume{c, \annoc}$}
% \begin{align*}
%     \consume{c, \alpha} &\triangleq \bracs{\alpha} c \\ 
%     \consume{c, \invar \ @ \ \texttt{while}(\beta) \texttt{ do }\annoc \texttt{ od } c'} &\triangleq c' \text{ if }(c \in \invar) \wedge (c' \in \invar \cap \bracs{\neg \beta})\\
%     \consume{c, \annoc_1 ; \annoc_2} &\triangleq \consume{\consume{c, \annoc_1}, \annoc_2} \\
%     \consume{c, \texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2} &\triangleq \left\{ \begin{array}{rcl}
%         \consume{c, \annoc_1} & \text{if } c \in \bracs{\beta} \\
%         \consume{c, \annoc_2} &  \text{otherwise} 
%         \end{array}\right. 
% \end{align*}

\subsection{$\anno \leq \annoc$}
$
\begin{array}{c}
    % \hspace{3cm}
    \inferrule*[lab={\footnotesize{\textsc{Atomic statements}}}]
    {
    % \consume{c, \alpha} = c'
    }
    {
    \alpha \leq \alpha 
    } 
    \hspace{1cm}
    \inferrule*[lab={\footnotesize{\textsc{Loop}}}]
    {
    \invar' \leq \invar \quad 
    \anno_1 \leq \annoc_1
    }
    {
    \invar' \ @ \ \texttt{while}(\beta) \texttt{ do }\anno_1 \texttt{ od } \leq \invar \ @ \ \texttt{while}(\beta) \texttt{ do }\annoc_1 \texttt{ od } c
    } 
    \\\\ 
    \inferrule*[lab={\footnotesize{\textsc{Sequence}}}]
    {
    \anno_1 \leq \annoc_1 \\\\
    \anno_1 \leq \annoc_1
    }
    {
    \anno_1 ; \anno_2 \leq \annoc_1 ; \annoc_2
    } 
    \hspace{1cm}
    \inferrule*[lab={\footnotesize{\textsc{If}}}]
    {
    \anno_1 \leq \annoc_1 \\\\
    \anno_1 \leq \annoc_1
    }
    {
    \texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2 \leq \texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2
    } 
\end{array}
$

\subsection{$\anno < \annoc$}
$
\begin{array}{c}
    \inferrule*[lab={\footnotesize{\textsc{Loop}}}]
    {
    \invar' \ @ \ \texttt{while}(\beta) \texttt{ do }\anno_1 \texttt{ od } \leq \invar \ @ \ \texttt{while}(\beta) \texttt{ do }\annoc_1 \texttt{ od } c \\\\
    \invar' \subseteq \invar \setminus \{c\} \vee \anno_1 < \annoc_1
    }
    {
    \invar' \ @ \ \texttt{while}(\beta) \texttt{ do }\anno_1 \texttt{ od } < \invar \ @ \ \texttt{while}(\beta) \texttt{ do }\annoc_1 \texttt{ od } c
    } 
    \hspace{1cm} 
    \inferrule*[lab={\footnotesize{\textsc{Sequence}}}]
    {
    \anno_1 ; \anno_2 \leq \annoc_1 ; \annoc_2 \\\\
    \anno_1 < \annoc_1 \vee \anno_1 < \annoc_1
    }
    {
    \anno_1 ; \anno_2 < \annoc_1 ; \annoc_2
    } 
    \\\\
    \inferrule*[lab={\footnotesize{\textsc{If}}}]
    {
    \texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2 \leq \texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2 \\\\
    \anno_1 < \annoc_1 \vee \anno_1 < \annoc_1
    }
    {
    \texttt{if}(\beta) \texttt{ then } \anno_1 \texttt{ else }\anno_2 < \texttt{if}(\beta) \texttt{ then } \annoc_1 \texttt{ else }\annoc_2
    } 
\end{array}
$

\subsection{Semantics of refine}
\begin{align*}
    \refine(\ini, (c,c'), \alpha) &\triangleq \false, \alpha \\
    \refine(\ini, (c,c'), L) & \triangleq \left\{ \begin{array}{rcl}
        \true, L' & \text{where } (L' \prec L ) \wedge (\ini \models L')\\
        \false, L & \text{if } \exists \annoc \cdot \consume{c, \annoc} = c' \ \wedge \  \not\exists L' \cdot L' < \annoc
        \end{array}\right. \\
\end{align*}

==> sections/overview.tex <==
 \section{Overview}
\begin{figure}
    \begin{minipage}{0.35\textwidth}
        % \centering 
        \begin{lstlisting}[numbers=none]
while (x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = y + 1;
}\end{lstlisting} 
        \caption{Example terminating program}
        \label{overview:code1}
    \end{minipage}
    % \vrule
    \begin{minipage}{0.6\textwidth}
        \begin{align*}
            &\rf(x',y',n') \\ 
            &= \max\big(1-(x'+y'), 0\big) + \max(n - x' + 1, 0) \\ 
            &= \max\big(-(2x+2y), 0\big) + \max(n-2x-y+1,0) \\
            &= 0 + \max\big(n-x+1-(x+y),0\big) \\
            &= \max\big(n-x+1-(x+y),0\big)
            % &\geq \max(n-x+1,0) - 1
        \end{align*}
        \caption{Value of Ranking function at the end of one iteration}
        \label{overview:rankingred}
    \end{minipage}
\end{figure}
\ggnds{First paragraph very overwhelming, not needed maybe}
In this section, we present a loop program (Figure~\ref{overview:code1}) that terminates, and the termination can be proved using a ranking function. We then change the program slightly so that it does not impact the termination of the program (Figure~\ref{overview:code2}). However, to show the validity of the ranking function, we now need an invariant of the program. We observe that we can transform the program (Figure~\ref{overview:code3}) to generate an invariant that can prove the validity of the ranking function. We then present a run of our algorithm to generate the invariant and the ranking function for the Program~\ref{overview:code3} simultaneously. 
% \begin{figure}
%     \begin{minipage}{0.3\textwidth}
%         % \raggedright
%         \begin{lstlisting}[numbers=none, basicstyle=\footnotesize]
% while (x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     z = z + 1;
% }\end{lstlisting} 
%         \caption{Example terminating program}
%         % \label{overview:code1}
%     \end{minipage}
%     \vrule
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \begin{lstlisting}[numbers=none, basicstyle=\footnotesize]
% while (x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1;
% }\end{lstlisting} 
%         \caption{Modified program}
%         \label{overview:code2}
%     \end{minipage}
%     \vrule
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \begin{lstlisting}[numbers=none, basicstyle=\footnotesize]
% if(x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1;
% }
% while (x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1; 
% }\end{lstlisting} 
%         \caption{Program transformation}
%         \label{overview:code3}
%     \end{minipage}
% \end{figure}




Consider the program in Figure~\ref{overview:code1}, which terminates for all values of $x, y$, and $n$.
For each iteration, if the loop body is executed, the loop guard is true before executing line 2, i.e., $x+y \geq 0$ and $x \leq n$.\ggnds{change this} 
Focusing on the value of x in successive iterations of the loop, we analyze two cases: (i) $x+y > 0$ and (ii) $x+y = 0$. In the first case, the updated value of $x$ is $x' = 2x + y = x + (x+y) > x$. Since the value of $x$ increases, the loop terminates in this case. In the second case, the updated value of $x$ is $x' = x + (x+y) = x$, and the updated value of $y$ is $y' = y+1 > y$. In all the subsequent iterations after the second case, $x+y > 0$, and hence $x$ always increases. 

\yascom{This paragraph and the subsequent 2 are a bit hard to read because the math is in paragraph form. I think we should show the two cases above in a list so they are separated. In the first element of the list, we present case 1 and say the $x$ increases, in the second element of the list, we present case 2 and say that $x$ always increases after this iteration.}

% The above argument gives an intuition of the termination of the loop, however, it is not an automated method for proving termination. 
% One of the common ways (sufficient but not necessary) to prove the termination of a loop is to find a ranking function.
The ranking function derived from this intuition is
% Consider the ranking function that follows from the above intuition, 
$\rf = \max(1-(x+y), 0) + \max(n - x + 1, 0)$. 
To prove the validity of the ranking function, we need to prove the two properties according to Definition~\ref{def:bgroundranking}, i.e., Bounded and Ranking.
% To prove the validity of the ranking function, we show (i) that the ranking function is bounded from below for all reachable states, and (ii) the value of the ranking function decreases by at least 1 at each iteration. 
% \sgcom{1 is not necessary, any constant works, move the argument that any implies 1 here}. 
Since $\rf$ is a summation of two $\max$ terms, it can easily seen that it is bounded from below by $0$.
The values of the variable \ggnds{typo} at the end of one iteration in terms of the value at the beginning of the loops are $x' = 2x+y, y' = y+1, n' = n$. We need to show : $\rf(x,y,n) - \rf(x',y',n')\geq 1$. From Figure~\ref{overview:rankingred}, $\rf(x',y',n') = \max\big(n-x+1-(x+y), 0\big)$. If $(x+y)>0$, $\max\big(n-x+1-(x+y), 0\big) > \max(n-x+1, 0)-1$ \sgcom{less than equal to?}. If $(x+y)=0$, the first term of $\rf(x,y,z) = 1$, and the second term is equal to $\rf(x',y',n')$ \sgcom{unclear}. So, in both cases, $\rf(x,y,n) - \rf(x',y',n')\geq 1$.  \ggnds{no need to give rf description}

\yascom{I think the reducing property should either be shown just in the figure, or we can have a list of two cases here as well and explain each case in a list so it is more clear.}

% \begin{enumerate}
%     \item $\rf$ is bounded below: $\max(1-(x+y), 0) \geq 0$ and $\max(n-x+1, 0) \geq 0$ implies that $\rf$ is always greater than equal to 0 (and hence bounded below).
%     \item $\rf$ decreases at least by 1 in all iterations: Lt $x, y, n$ be the variables before the start of a iteration and $x', y', n'$ be the variables after the iteration, i.e. $x' = 2x + y$, $y' = y + 1$ and $n' = n$. So, the value of the ranking function changes as:
%     \begin{align*}
%     &\rf(x,y,n) - \rf(x',y',n') \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(1-(x'+y'), 0) - \max(n - x' + 1, 0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(-(2x+2y), 0) - \max(n-2x-y+1,0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(n-x +1 - (x+y), 0)
%     \end{align*}
%     ($\max(-(2x+2y), 0)$ = 0 as $x+y \geq 0$ holds always)\\\\
%     Now, consider the following two cases:
%     \begin{enumerate}
%         \item $x + y > 0$: As $x$ and $y$ are integers, this means that $x + y \geq 1$. \\
%         $x + y \geq 1 \implies \max(1-(x+y), 0) = 0$.\\
%         $x \leq n \implies \max(n-x+1, 0) = n-x+1$\\
%         $n - x + 1 \geq 1 \wedge x + y \geq 1 \implies \max(n-x +1 - (x+y), 0) \leq n - x + 2$ (as $x, y$ and $n$ are integers)
%     \begin{align*}
%     &\rf(x,y,n) - \rf(x',y',n') \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(n-x +1 - (x+y), 0)\\
%             &= 0 + n-x+1 - \max(n-x +1 - (x+y), 0)\\
%             & \geq 1 \; \text{from} \max(n-x +1 - (x+y), 0) \leq n - x + 2
%             % &\geq 1
%     \end{align*}
%         \item $x + y = 0$:
%     \begin{align*}
%     &\rf(x,y,n) - \rf(x',y',n') \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(n-x +1 - (x+y), 0)\\
%             &= \max(1-(0), 0) + \max(n - x + 1, 0) - \max(n-x +1 - (0), 0)\\
%             &= \max(1-(0), 0)\\
%             &= 1 \geq 1
%             % &\geq 1
%     \end{align*}
%     \end{enumerate}
    
    % Let $v1 = \max(1-(x+y), 0) + \max(n-x+1, 0)$. After one iteration, $x = x + 2*y$ and $y = y + 1$. So, $v2 = \max()$
    
    % First, let's break our ranking function into two parts: $r_{f_1} = \max(-x-y+1, 0)$ and $r_{f_2} = \max(n-x+1, 0)$. We have $\rf = r_{f_1} + r_{f_2}$. Now, consider the following two cases:
    % \begin{enumerate}
    %     \item $x + y > 0$: This means $x$ increases in this loop as $x = x + (x + y)$. As $n \geq x$ at the time of entering the loop, the value of $r_{f2}$ is $n - x + 1$ (as this value is greater than 0). Now, as $x$ increases, $n - x + 1$ will surely decrease (and if it goes below 0, the new value of $r_{f2}$ will be 0). So $r_{f2}$ decreases. And as $y$ also increases (by 1) in each iteration, $- x - y + 1$ decreases, and so the new value of $r_{f1}$ can not be more than the old value of $r_{f1}$. This ensures that in this case $r_f = r_{f1} + r_{f2}$ decreases.
    %     \item $x + y = 0$: This means $x$ does not change in this iteration. And so $r_{f2}$ remains constant. As $x + y$ is 0 initially, the value of $r_{f1}$ is 1. Now, as $y$ increases by 1 in each iteration, the new value of $x+y$ will be 1 after the loop, and the new value of $r_{f1}$ would be $\max(-1 + 1, 0) = 0$. So, in this case, $r_{f1}$ always decreases by 1 and $r_{f2}$ remains constant. This ensures that in this case $r_f = r_{f1} + r_{f2}$ decreases.
    % \end{enumerate}
    % In both cases, we can show that the value of \rf decreases.
    
% \end{enumerate}

% The updated values of $x,y$ after one iteration of the loop are $x' = 2*x+y, y' = y+1$. So, $\rf(x', y') = \max(1-(x'+y'), 0) + \max(n-x', 0) = \max(-(2*x+2*y), 0) + \max((n-x)-(x+y))$.Consider two cases depending on the value of $x+y$. In both cases, we can show that the value of \rf decreases.
% Hence, it is a valid ranking function.   
% \begin{enumerate}
%     \item $\rf$ is bounded below: $\max(1-(x+y), 0) \geq 0$ and $\max(n-x, 0) \geq 0$ implies that $\rf$ is always greater than equal to 0 (and hence bounded below).
%     \item $\rf$ decreases at least by 1 on all reachable program states: First, let's break our ranking function into two parts: $r_{f_1} = \max(-x-y+1, 0)$ and $r_{f_2} = \max(n-x+1, 0)$. We have $\rf = r_{f_1} + r_{f_2}$. Now, consider the following two cases:
%     \begin{enumerate}
%         \item $x + y > 0$: This means $x$ increases in this loop. As $n \geq x$ at the time of entering the loop, the value of $r_{f2}$ is $n - x + 1$ (as this value is greater than 0). Now, as $x$ increases, $n - x + 1$ will surely decrease (and if it goes below 0, the new value of $r_{f2}$ will be 0). So $r_{f2}$ decreases. We can also observe that $y$ increases by 1 in each iteration. As both $x$ and $y$ are increasing, $- x - y + 1$ decreases, and so the new value of $r_{f1}$ can not be more than the old value of $r_{f1}$. This ensures that in this case $r_f = r_{f1} + r_{f2}$ decreases.
%         \item $x + y = 0$: This means $x$ does not change in this loop. And so $r_{f2}$ remains constant. As $x + y$ is 0 initially, the value of $r_{f1}$ is 1. Now, from our observation that $y$ increases by 1 in each iteration, the new value of $x+y$ will be 1 after the loop, and the new value of $r_{f1}$ would be $\max(-1 + 1, 0) = 0$. So, in this case, $r_{f1}$ always decreases by 1 and $r_{f2}$ remains constant. This ensures that in this case $r_f = r_{f1} + r_{f2}$ decreases.
%     \end{enumerate}
% \end{enumerate}
\begin{figure}
    \begin{minipage}{0.35\textwidth}
        \centering
        \begin{lstlisting}[numbers=left]
while (x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = z;
    z = z + 1;
}\end{lstlisting} 
        \caption{Code}
        \label{overview:code2}
    \end{minipage}
    \begin{minipage}{0.6\textwidth}
    \centering 
        \begin{tabular}{c|c|c|c|c|c}
            $x$ & $y$ & $z$ & $n$ & $(x+y\geq0) \wedge (x\leq n)$ & \rf \\ 
            \hline 
            1 & -1& -1& 4 & \true & 5 \\ 
            1 &-1& 0& 4& \true &5 \\ 
            1 &0& 1& 4& \true &4 \\ 
            2 &1& 2& 4& \true &3  \\
            5 & 2 & 3 & 4 & \false & - 
        \end{tabular}
        \caption{Trace}
        \label{overview:trace}
    \end{minipage}
    \ggnds{bad captions}
\end{figure}
Now, consider the program in Figure~\ref{overview:code2} which is a small variation of the original program. Since the program is almost similar, intuitively, the same ranking function should be sufficient to prove the termination. However, observe that there is a counter-example: $\{x = 1, y = -1, z = -1, n = 4\}$. The trace (the valuation of all variables just before the loop guard) generated by executing the program on these values is shown in Figure~\ref{overview:trace}. \yascom{I think in Figure 4, we should show the value of rf in the last row to show that it is not decreasing. Maybe we can skip the invariant in this figure because we have not introduced it yet. Later, we can say the invariant we found is not true for the last row in Fig 4.} Note that although the ranking function does not decrease at each iteration, the loop is still terminating. Other than the first iteration, there is a relation between the values of $y$ and $z$, i.e., $y+1 = z$. Since this is not always true for the first iteration of the loop, we transform the program, preserving its semantics. We unroll the loop for the first iteration using an if statement and separate it from the rest of the program (Figure~\ref{overview:code3}).
% \begin{figure}
%     \centering
%     \begin{lstlisting}[numbers=left]
% if(x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1;
% }
% while (x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1; 
% }\end{lstlisting}
%     \caption{Caption}
%     \label{fig:overview:code3}
% \end{figure}

\begin{figure}
    \begin{minipage}{0.35\textwidth}
        \centering 
        \begin{lstlisting}[numbers=left]
if(x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = z;
    z = z + 1;
}
while (x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = z;
    z = z + 1; 
}\end{lstlisting} 
        \caption{Example terminating program}
        \label{overview:code3}
    \end{minipage}
    % \vrule
    \begin{minipage}{0.6\textwidth}
    \small 
        \begin{align*}
            \qquad&\rf(x',y',z',n') \\ 
            &= \max\big(1-(x'+y'), 0\big) + \max(n - x' + 1, 0) \\ 
            &= \max\big(1-2x-y-z), 0\big) + \max(n-2x-y+1,0) \\
            &= \max\big(1-2x-y-\textbf{(y+1)}), 0\big) + \max\big(n-x+1-(x+y),0\big) \\ 
            &= \max(-2x-2y, 0) + \max\big(n-x+1-(x+y),0\big) \\ 
            &= 0 +\max\big(n-x+1-(x+y),0\big) \\
            &= \max\big(n-x+1-(x+y),0\big)
            % &\geq \max(n-x+1,0) - 1
        \end{align*}
        \caption{Value of Ranking function at the end of one iteration}
        \label{overview:rankingred2}
    \end{minipage}
\end{figure}



% \begin{figure}
%     \begin{minipage}{0.4\textwidth}
%         \centering
%         \begin{lstlisting}[numbers=left]
% if(x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1;
% }
% while (x + y >= 0 && x <= n) {
%     x = 2 * x + y;
%     y = z;
%     z = z + 1; 
% }\end{lstlisting} 
%         \caption{Code}
%         \label{overview:code}
%     \end{minipage}
%     \begin{minipage}{0.7\textwidth}
%     \centering 
%         \begin{align}
%             &\rf(x,y,n) - \rf(x',y',n') \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(1-(x'+y'), 0) - \max(n - x' + 1, 0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(-(2*x+2*y), 0) - \max(n-2*x+y,0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - 0 - \max(n-x - (x+y), 0) \\
%             &= \max(1-(x+y), 0) - \max(n-x - (x+y), 0) + \max(n - x + 1, 0)  \\
%             &\geq 1
%         \end{align}
%         \caption{Trace}
%         \label{overview:trace}
%     \end{minipage}
% \end{figure}
Observe that in the transformed program, $y+1 = z$ is an invariant at line 6. Using this invariant we can now prove that the ranking function ($\rf(x,y,z,n) = \max(1-(x+y), 0) + \max(n - x + 1, 0)$) is valid. It is still bounded by 0 from below.
The values of the variables at the end of the loop in terms of the values at the beginning of the loop are $x' = 2x+y, y' = z, z' = z+1, n' = n$. Using the invariant, $\rf(x',y',z',n') = \max\big(n-x+1-(x+y),0\big)$ (derivation in Figure~\ref{overview:rankingred2}). As proved previously, $\rf(x) - \rf(x')\geq 1$ \sgcom{x,y,z,n}
\ggnds{We do not need to give this much motivation, looks too easy}
 
% \begin{enumerate}
%     \item $\rf$ is bounded below: $\max(1-(x+y), 0) \geq 0$ and $\max(n-x+1, 0) \geq 0$ implies that $\rf$ is always greater than equal to 0 (and hence bounded below).
%     \item $\rf$ decreases at least by 1 in all iterations: Let $x, y, z, n$ be the variables before the start of a iteration and $x', y', z', n'$ be the variables after the iteration, i.e. $x' = 2x + y$, $y' = z$, $z' = z + 1$ and $n' = n$. So, the value of the ranking function changes as:
%     \begin{align*}
%     &\rf(x,y,z, n) - \rf(x',y',z', n') \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(1-(x'+y'), 0) - \max(n - x' + 1, 0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(1-2x-y-z), 0) - \max(n-2x-y+1,0) \\ 
%              &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(1-2x-y-\textbf{(y+1)}), 0) - \max(n-2x-y+1,0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(-(2x+2y), 0) - \max(n-2x-y+1,0) \\ 
%             &= \max(1-(x+y), 0) + \max(n - x + 1, 0) - \max(n-x +1 - (x+y), 0)
%     \end{align*}
%     ($\max(-(2x+2y), 0)$ = 0 as $x+y \geq 0$ holds always)

%     Now, we can do the same case analysis as above. \sgcom{Write this in a better way, maybe by linking the proof.}
% \end{enumerate}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image.png}
    \caption{Overview of the algorithm}
    \label{fig:overview}
\end{figure}
% \subsection{Our algorithm - \textcolor{red}{change heading}}
\subsection{Over-approximation and under-approximation of Reachable states }
As presented in Section~\ref{sec:background}, for a ranking function to be valid, for all reachable states, it must be bounded and it must reduce for each iteration. However, for an arbitrary program, the exact set of reachable states ($\reach$) is often unknown and hard to compute. The states observed by running the program a finite number of times ($r$) provide an under-approximation of the reachable states, i.e., $r \subseteq \reach$. 
So, for the validity of a ranking function, it is necessary (but not sufficient) that for all states in $r$, the function reduces at each iteration and is bounded. 

Further, an invariant ($\invar$) is an over-approximation of the reachable states ($\reach$), i.e., $\reach \subseteq \invar$. The strongest invariant is the intersection of all the possible invariants of a program, i.e., $\invar^s = \bigcap_i \invar_i$, where $\{\invar_i\}$ are all the possible invariants. The strongest invariant gives an exact representation of the reachable states, i.e., $\invar^s = \reach$, however, computing the strongest invariant is an undecidable problem.   
Since invariants are over-approximations of the reachable states,
% Only the strongest invariant, i.e., the intersection of all possible invariants, provides an exact representation of the reachable states, computing which is often undecidable. In general, an invariant is an over-approximation of the reachable states, i.e., $\reach \subseteq \invar$. 
for the validity of a ranking function, it is sufficient (but not necessary) to check that for all states in $\invar$, the function reduces at each iteration and is bounded. 

% It is often easy to synthesize valid ranking functions w.r.t a small set of reachable states $r$ as opposed to the complete reachable set. Further, an invariant $\invar$ is usually a prohibitively large set and therefore, is represented using a system of equalities and inequalities. Consequently, checking the validity of a ranking function using an invariant can be reduced to checking the satisfiability of a first-order formula. 
% We leverage these advantages of $\rp$ and $\invar$ in our algorithm in the following way: we maintain an approximation of $\reach$ using $\rp$ (under-approximation) and $\invar$ (over-approximation). We iteratively use $\rp$ to generate a candidate ranking function, and then use the invariant $\invar$ to check the validity of the generated function. If the ranking function is invalid, we get a counter-example, which is either added to the set $\rp$ or is used to improve the invariant $\invar$, leading to a better approximation of $\reach$.
% \\



\noindent
\textbf{Reachability w.r.t Template of Invariants:} An invariant is usually characterized by a function $\invar$. A state $X$ is in the invariant iff $\invar(X) = \true$. So, $\invar(X)$ and $X \in \invar$ can be used interchangeably depending on the context. In our algorithm, we consider invariants of the form $c_0 + \sum_ic_ix_i \geq 0$, where $x_i$ are the program variables and $c_i \in \mathbb{R}$. We refer to the set of all functions of this form as the template $\tempi$ and the set of all valid invariants in this template as $\itemps$ \ggnds{why this notation}.  Since all our invariants are restricted to the template $\tempi$, we introduce the notion of $\reachp$ = $\bigcap \itemps$  as the set of all reachable states \textit{with respect to our template} $\tempi$.

\yascom{Since the lattice is defined with respect to each invariant in our template, I think either the template has to be the conjunction of invariants of that form or we have to make sure the definition of elements of the lattice are conjunctions of invariants from the template. I think it is better to have the template be conjunctions of invariants of this form, but then the definition below has to change.}

\begin{definition}
    \label{def:rp}
    Given $\tempi$, $\reachp$ is the set of states $X$ such that for all $\invar \in \itemps \cdot X \in \invar$.
\end{definition}
\ggnds{no defs please}

As noted previously, the strongest possible invariant is the exact representation of the reachable states, i.e., $\bigcap I_i = \reach$. And as $\itemps \subseteq I_i$, ($\bigcap I_i) \subseteq (\bigcap \itemps)$ which implies $\reach \subseteq \reachp$. This shows that $\reachp$ overapproximates $\reach$.

% Since we are only considering the invariants restricted to our template, 
% However, since all our invariants are restricted to the template $\tempi$, the intersection of all invariants is an over-approximation of the reachable states, i.e., $\reach \subseteq \reachp = \bigcap I_i$, where $I_i$ are valid invariants and $I_i \in \tempi$. 

% Now, we define the validity of a ranking function w.r.t the template ($\tempi$) of invariants as:
% \begin{definition}
% \label{def:overviewrf}
%     $\rf : S \rightarrow \mathbb{I}$ is a valid ranking function w.r.t the template of invariants $\tempi$ if it satisfies the following conditions:
%     \begin{enumerate}
%         % \item \textbf{\textit{Bounded. }} $\forall X \in \reachp \cdot \rf(X) \geq 0$
%         % \item \textbf{\textit{Ranking. }} $\forall X \in \reachp, \forall X' \in T(X) \cdot \rf(X) - \rf(X') \geq 1$ 
%         \item \textbf{Bounded. } $\forall s \in \reachp \cdot B(s) \implies \rf(s) \geq 0$
%         \item \textbf{Ranking. } 
%         $\forall s \in \reachp \cdot B(s) \implies \rf(s) - \rf(\mathcal{P}_2(s)) \geq 1$
%     \end{enumerate} where $\reachp = \bigcap \itemps$ \sgcom{B and P2?}
% \end{definition}

% Since capturing the exact notion of $\reachp$ is not straight-forward.

% \begin{definition}
% \label{def:overviewrfinvar}
%     $\rf : S \rightarrow \mathbb{I}$ is a valid ranking function w.r.t an invariant $\invar \in \tempi$ if it satisfies the following conditions:
%     \begin{enumerate}
%         % \item \textbf{\textit{Bounded. }} $\forall X \in \reachp \cdot \rf(X) \geq 0$
%         % \item \textbf{\textit{Ranking. }} $\forall X \in \reachp, \forall X' \in T(X) \cdot \rf(X) - \rf(X') \geq 1$ 
%         \item \textbf{Bounded. } $\forall s \in \invar \cdot B(s) \implies \rf(s) \geq 0$
%         \item \textbf{Ranking. } 
%         $\forall s \in \invar \cdot B(s) \implies \rf(s) - \rf(\mathcal{P}_2(s)) \geq 1$
%     \end{enumerate} \sgcom{B and P2?}
% \end{definition}

% The examples provided demonstrate that one way to prove the termination of programs automatically is by synthesizing ranking functions. A valid ranking function is characterized by two key properties: (i) it must have a finite lower bound, and (ii) it should decrease by at least a fixed amount in each iteration. 
% If a function $f$ is bounded below by $\theta$, i.e., $\forall x \cdot f(x)\geq \theta$ and decreases at each iteration by $\delta > 0$, i.e., $\forall x \cdot f(x) - f(x')\geq \delta$, then we can synthesize a function $f'$ that is bounded from below by 0 and decreases at each iteration by at least 1. Specifically, $f'(x) \triangleq (f(x) - \theta) / \delta$.   
\noindent
\textbf{Template of Ranking Functions:} In our approach, we try to find a ranking function that is bounded from below by 0 and reduces by at least 1 in every iteration. Specifically, we inspect ranking functions of the form $\max(a_0 + \sum_i a_ix_i, 0) + \max(b_0 + \sum_i b_ix_i, 0)$, where $x_i$ are the program variables and $a_i, b_i \in \mathbb{I}$. We refer to the set of all functions of this form as the template $\tempr$. This template ensures that the ranking function is always greater than or equal to 0. So, we just need to ensure that the ranking function reduces by at least 1 at each iteration.

% From the example, it is also clear that it might not be easy to prove the validity of a ranking function in the absence of an invariant. An invariant is the smallest set of program states that include the input program states and is inductive. We provide formal definitions for the validity of a ranking function and invariant in Section~\ref{}. 
% Similarly, an invariant is usually characterized by a function $\invar$. A state $X$ is in the invariant iff $\invar(X) = \true$. So, $\invar(X)$ and $X \in \invar$ can be used interchangeably depending on the context. In our algorithm, we consider invariants of the form $c_0 + \sum_ic_ix_i \geq 0$, where $x_i$ are the program variables and $c_i \in \mathbb{R}$. We refer to the set of all functions of this form as the template $\tempi$.



It is relatively easier to synthesize ranking functions w.r.t a small set of reachable states $r$ as opposed to the complete reachable set. Further, an invariant $\invar$ is usually a prohibitively large set and therefore, is represented using a system of equalities and inequalities. Consequently, checking the validity of a ranking function using an invariant can be reduced to checking the satisfiability of a first-order formula.  We leverage these advantages in our algorithm. \ggnds{synergy?}

\subsection{Algorithm Overview}
 % As depicted in Figure~\ref{fig:overview}, at each step of our algorithm, we maintain an approximation of $\reachp$ using $\rp$ (under-approximation as $\rp \subseteq \reachp$ always) and $\invar \in \itemps$ (over-approximation). We iteratively use $\rp$ to generate a candidate ranking function from $\tempr$, and then use the invariant $\invar$ to check the validity of the generated function (as defined in Def \ref{def:overviewrfinvar}). If the ranking function is invalid, we get a counter-example, which is either added to the set $\rp$ or is used to improve the invariant $\invar$, leading to a better approximation of $\reachp$.

As depicted in Figure~\ref{fig:overview}, at each step of our algorithm, we maintain a state defined by a tuple $\langle \rp, \invar \rangle$, where $\rp$ is an under-approximation of $\reachp$ and $\invar \in \tempi$ is a valid invariant and an over-approximation of $\reachp$. The set $\rp$ is initialized with randomly generated traces of the given program, and the invariant is initialized with $\true$. Each iteration of our algorithm has two phases:

\begin{enumerate}
    \item \textbf{Generate Candidate Phase}: In this phase, we generate a ranking function ($\rf$) from our template $\tempr$ that follows the Ranking property w.r.t $\guard, \rp, \trans$, i.e. 
    \begin{equation}
        \label{eq:rfcreate}
        \forall X \in \rp, \forall X' \in \trans(X) \cdot \rf(X) - \rf(X') \geq 1
    \end{equation}
    We then check for the validity of ($\rf$) w.r.t $\invar$, i.e,
    \begin{equation}
        \label{eq:rfcheck}
        \forall X \in \invar, \forall X' \in \trans(X) \cdot \rf(X) - \rf(X') \geq 1.
    \end{equation}
    \ggnds{use x,xprime in T}
    \sgcom{use the notation from the discovered paper}
    
    If the above query succeeds, the candidate ranking function is valid using Lemma~\ref{lemma:bground}. 
    Since $\rp \subseteq \invar$, the above query may not be \true. So, we may get a counter-example $c, c'$, such that $c \in \invar, c' \in \trans(c)$ and $\rf(c) - \rf(c') < 1$. 

    \item \textbf{Refine State Phase}: In this phase, we use the counter-example $c$ generated in the Generate Candidate phase to refine the current algorithm state. It may be possible that $c \not\in \reachp$. So, for the validity of the ranking function w.r.t $\reachp$, $c$ may be a spurious counter-example. We first try to strengthen the invariant to $\invar'$ such that $\invar' \subseteq \invar \setminus \{c\}$. If this strengthening does not succeed, we can conclude that the counter-example $c$ is reachable w.r.t $\tempi$, i.e., $c \in \reachp$. So, we add $c$ to the set $\rp$, i.e., $\rp_{new} = \rp \cup \{c\}$.
\end{enumerate}

\begin{table}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c||c|c|}
    \hline 
         &$r^+$ & $\invar$ & $\rf$ & $c$  \\
         \hline
         1&$\{(1,2,3,4), (2,2,3,4)\}$ & $\true$ & $\max(n-x+1,0)$ & $(1,-1,2,4)$ \\  
         \hline 
         2&$\{(1,2,3,4), (2,2,3,4)\}$ & $\textcolor{blue}{y+1\geq z}$ & $\max(n-x+1,0)$ & $(1,-1,-1,4)$ \\ 
         \hline 
         3&$\{(1,2,3,4), (2,2,3,4)\}$ & $\textcolor{blue}{(y+1\geq z) \wedge (y+1\leq z)}$ & $\max(n-x+1,0)$ & $(1,-1,0,4)$ \\  
         \hline
         4&$\{(1,2,3,4), (2,2,3,4), \textcolor{blue}{(1,-1,0,4)}\}$ & $(y\geq z-1) \wedge (y\leq z-1)$ & $\textcolor{blue}{\max(n-x+1,0) + \max(1-x-y, 0)}$ & -   \\
         \hline 
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:overview}
\end{table}

% \subsection{Example}
% \noindent
% \textbf{Algorithm State. }
% At each step of our algorithm, the state is defined by a tuple $\langle \rp, \invar \rangle$, where $\rp$ is an under-approximation of $\reachp$ and $\invar \in \tempi$ is a valid invariant, and an over-approximation of $\reachp$. At each iteration of our algorithm, we generate a ranking function ($\rf$) that satisfies the \textit{Bounded} and \textit{Ranking} property on $\rp$ (necessary condition). We then check for the validity of ($\rf$) w.r.t $\invar$. If it is valid, then we have found our answer. If not, then we either refine our invariant or expand the set $\rp$, thereby updating the algorithm state and improving the approximation of $\reachp$.

% % At each step of our algorithm, we maintain a valid invariant - $\invar$, and a set of states - $\rp$. The set $\rp$ consists of the states that are reachable w.r.t our template of invariants $\tempi$, i.e., $X \in \rp$ iff $\forall \invar \in \tempi \cdot X \in \invar \wedge \valid(\invar)$. 
% The set $\rp$ is initialized with randomly generated traces of the given program and the invariant is initialized with $\true$. Each step of our algorithm is characterized by two meet-semi-lattices - (i) $\lati$ - each point in this semi-lattice is an element from the template $\tempi$, (ii) $\latr$ - each point in this semi-lattice is the set of functions from the set $\tempr$. The elements of both of these semi-lattices are ordered by the $\subseteq$ relation, and meet is defined as the intersection ($\cap$) operation on sets. \sgcom{Lattices enter suddenly and then it is not clear yet why are they introduced}

% Given a program, we perform program transformations like the one presented in the previous example, i.e., unrolling the first iteration of the loop. After performing this transformation, we show the running of our algorithm on the program provided in Figure~\ref{overview:code3}. Broadly, we perform the following steps:



% \sgcom{Make the names of these steps consistent with that in the diagram.}

% \noindent
% \textbf{Synthesize ranking function ($\rp$). }
% This included two substeps:
% \begin{enumerate}
%     \item \textbf{Gen ranking ($\rp$). }
%     We find a candidate ranking function from our template $\tempr$, which reduces at least by 1 on all the states present in the current $\rp$. We define $F(\rp)$ as the set of all the functions in the template $\tempr$ that reduce on all the states in $\rp$, i.e., 
%     $$F(\rp) = \{f \in \tempr \ | \ \forall X \in \rp \cdot f(X) - f(X') \geq 1\}$$
%     \sgcom{what is x prime?}
%     $F(\rp)$ is an element of the lattice $\latr$. The output of this step is an element of the set $F(\rp)$. Although it reduces on all the states in $\rp$, it is not guaranteed to reduce on all reachable states. For instance, at the first step of Table~\ref{tab:overview}, $\rp = \{(1,2,3,4), (2,2,3,4)\}$. This indicates that the state where $x=1, y=2, z=3, n=4$ and $x=2, y=2, z=3, n=4$ are reachable, and hence the candidate ranking function must reduce by at least 1 on these states. Further, the invariant at this state is $\true$, i.e., $\forall x,y,z,n, (x,y,z,n) \in \invar$. We generate a candidate ranking function from the template $\tempr$ such that it reduces by at least 1 on the states in $\rp$. This is done using the following SMT query: solve for $a_i$ such that 
%     \begin{gather*}
%         \forall (x,y,z,n) \in \rp \cdot \big( f(x,y,z,n) - f(x',y',z',n')\geq 1 \big), \quad where \\ 
%         f(x,y,z,n) \ = \ \max(a_0 + a_1x + a_2y + a_3z + a_4n,0) \ + \ \max(b_0 + b_1x + b_2y + b_3z + b_4n,0) \\ 
%         x'=2x+y, \ y'=z, \ z'=z+1, \ n'=n
%     \end{gather*}
%     Using Z3 solver, we get the ranking function $f(x,y,z,n) = \max(n-x+1,0)$

%     \item \textbf{Check ranking ($f, \invar$). } 
%     The inputs to this step are (i) the candidate ranking function generated at the previous step ($f$), and (ii) the current invariant $\invar$. At each step, since the invariant is valid, it is an over-approximation of the reachable set of states. So, if the ranking function reduces on all the states on the invariant, we have found our answer. However, if not, then we get a counter-example $c$, where the ranking function does not reduce by at least 1. This is done by the following SMT query: solve for $x,y,z,n$ such that
%     \begin{gather*}
%         \invar(x,y,z,n) \wedge \big(f(x,y,z,n) - f(x',y',z',n') < 1\big), \quad where \\ 
%         x'=2x+y, \ y'=z, \ z'=z+1, \ n'=n
%     \end{gather*}
%     Solving this query, we get a counter-example: $x=1, y=-1, z=2, c=4$. Note that this state satisfies the current invariant, and the candidate ranking function does not reduce for this state. The counter-example generated at this step can mean two things - (i) it was a spurious counter-example, i.e., it was not a reachable state, however, our invariant was not strong enough, and (ii) the candidate ranking function is incorrect. We first assume that the invariant is weak, and try to refine it in the next step.
% \end{enumerate}

% \noindent
% \textbf{Refine State. }
% From the previous step, either we have found a ranking function and the corresponding invariant that can prove termination of the loop. Otherwise, we get a counter-example which we use to refine our state. This includes two substeps:
% \begin{enumerate}
%     \item \textbf{Refine Invariant. }
%     The inputs to this step are the current invariant $\invar$ and a counter-example $c = (x,y,z,n)$. Our target is to synthesize an inductive invariant $\invar'$ that is stronger than the current invariant $\invar$ and does not include the state $c = (x_c, y_c, z_c, n_c)$. 
%     The current invariant $\invar$ is an element in the semi-lattice $\lati$. If this step succeeds, the new invariant $\invar'$ generated in this step will take us a step lower in the lattice because $\invar' \subseteq \invar \setminus \{c\}$. So, $\invar' \prec \invar$.
%     This is done by repeating the following two substeps alternatively - (i) generating a candidate invariant, and (ii) checking for the validity of the generated invariant.  
%     \begin{enumerate}
%         \item \textbf{Generate invariant ($\invar, \rp, c$). } 
%         We generate a candidate invariant that includes all states in $\rp$ and does not include the state $c$. This is done by solving the following query for the coefficients $c_i$ to get $\invar''$ and then taking a conjunction with $\invar$, i.e., $\invar' = \invar'' \wedge \invar$.
%         \begin{gather*}
%             \neg \invar'(x_c, y_c, z_c, n_c) \wedge \big(\forall (x,y,z,n) \in \rp \cdot \invar'(x,y,z,n) \big) , \quad where \\ 
%             \invar'(x,y,z,n) \ = \ c_0 + c_1x + c_2y + c_3z + c_4n \geq 0
%         \end{gather*}
%         In our running example, the invariant generated by solving the above query is $y-z+1 \geq 0$.
%         The solution obtained by solving the above inequalities is lower than $\invar$ in the lattice $\lati$. However, it is not guaranteed that it is a valid invariant. So, we proceed to the next step - which is checking the validity of the generated invariant. If the query is unsatisfiable, then the invariant cannot be refined such that it removes the counter-example. So, we have established that $c$ is in fact a reachable state.  
    
%         \item \textbf{Check Invariant ($\invar', Init$). }
%         The validity of the invariant $\invar'$ is checked by solving for a counter-example for the following query:
%         \begin{gather*}
%             \big(\forall X \in Init, \invar'(X)\big) \wedge \big(\invar'(X) \implies \invar'(X')\big)
%         \end{gather*}
%         If we do not get a counter-example, we have successfully refined the invariant. Otherwise, we generate a new candidate invariant that removes this new counter-example.
%         In our case, we do not get a counterexample and hence, we have successfully refined the invariant and moved down in the lattice $\lati$. So, we go back to the Check ranking function with the new invariant now. 
%         \end{enumerate}

%         \item \textbf{Update $\rp$ }
%         At this step, we have established that the ranking function is incorrect and we also have the exact counter-example where it should reduce. We add this counter-example to the set $\rp$, i.e., $\rp_{new} = \rp \cup \{c\}$. From this, $\rp \subset \rp_{new}$. So, $F(\rp_{new}) \subset F(\rp)$. So, we move down in the lattice $\latr$. 

%     We repeat these steps until we have found a ranking function $\rf$ and an invariant $\invar$ such that $\rf$ reduces on all the states in $\invar$. At each iteration of our algorithm, we move down in both the lattices $\latr$ and $\lati$.
% \end{enumerate}

% \yascom{I think nested loops should come in the overview to show we can handle them. So maybe we can say something like: This approach can be generalized to nested loops. First, we execute this procedure on the innermost loop. Then, for outer loops, we modify the refine invariant procedure to jointly refine the inner and outer loop invariants. We don't have to give an example, but there should be a paragraph explaining how we adapt the algorithm for nested loops.}

% \subsection{Example}
Consider the program in Figure~\ref{overview:code3}.  The set $\rp$ is initialized with randomly generated traces, in this case, $\rp_0 = \{(1,2,3,4), (2,2,3,4)\}$. The invariant is initialized with the set of all states, i.e., $\invar_0 = \true$. Our algorithm finds the ranking function and the corresponding invariant for this example in the following steps:

\begin{enumerate}
    \item \textbf{Generate Phase \RNum{1}:} We get a candidate ranking function $r_f = \max(n-x+1,0)$ that reduces on all states in $\rp = \{(1,2,3,4), (2,2,3,4)\}$. Then we check its validity with respect to the current invariant $\true$ (using Equation~\ref{eq:rfcheck}) to find a counter-example $c_1 = (1,-1,2,4)$.
    \item \textbf{Refine Phase \RNum{1}:} As we got a counter-example ($c_1 = (1,-1,2,4)$) in our generate phase, we try to refine our current invariant $\true$ to exclude this (as described above). This refinement succeeds, and we get a new invariant $y + 1 \geq z$, which excludes our counter-example $c_1$, also proving that the counter-example was unreachable and thus spurious.
    \item \textbf{Generate Phase \RNum{2}:} As $\rp$ is same as Phase \RNum{1}, the algorithm again generates the same function  $r_f = \max(n-x+1,0)$. But we now check its validity with respect to the new invariant $y + 1 \geq z$ and get a new counter-example $c_2 = (1,-1,-1,4)$.
    \item \textbf{Refine Phase \RNum{2}:} As we got a counter-example ($c_2 = (1,-1,-1,4)$) in our generate phase, we try to refine our invariant $y + 1 \geq z$ to exclude this. This refinement succeeds, and we get a new invariant $y + 1 \geq z \wedge y + 1 \leq z$, which excludes our counter-example $c_2$.
    \item \textbf{Generate Phase \RNum{3}:} As $\rp$ is same as Phase \RNum{1}, the algorithm again generates the same function $r_f = \max(n-x+1,0)$. But we now check its validity with respect to the new invariant $y + 1 \geq z \wedge y + 1 \leq z$ and get a new counter-example $c_3 = (1,-1,0,4)$.
    \item \textbf{Refine Phase \RNum{3}:} As we got a counter-example ($c_3 = (1,-1,0,4)$) in our generate phase, we try to refine our invariant $y + 1 \geq z \wedge y + 1 \leq z$ to exclude this. This refinement fails, proving that this counter-example is reachable (and thus not spurious). So, we add $c_3$ to our set of reachable states $\rp$.
    \item \textbf{Generate Phase \RNum{4}:} As the set $\rp$ got updated, we get a new candidate ranking function $r_f = \max(n-x+1,0) + \max(1-x-y, 0)$ that reduces on all states in $\rp$. Then we check its validity with respect to the current invariant $y + 1 \geq z \wedge y + 1 \leq z$. The validity check succeeds, and $r_f = \max(n-x+1,0) + \max(1-x-y, 0)$ is returned as a valid ranking function for the program.
\end{enumerate}

% \textbf{1 Generation phase. }First, we generate a candidate ranking function that is valid for the states in $\rp$. Solving this, we get the following ranking function $r_{f_1} = \max(n-x+1, 0)$. We then check the validity of this ranking function w.r.t $\invar_0$, and we get the counter-example $c_1 = (1,-1,2,4)$. This is shown in the first row of Table~\ref{tab:overview}.

% \textbf{1 Refine Step. }In the first refine step, we try to refine the invariant using the counter-example generated in the previous step. This is further done in two steps - (i) generate a candidate invariant using $\rp_0$, (ii) check the validity of the invariant. We repeat these steps until we have a valid invariant. In the current example, we get the refined invariant as $\invar_1 = y+1\geq z$. Since the counter-example is not a reachable state, $\rp_1 = \rp$

% \textbf{2 Generation phase. }Since $\rp_1 = \rp_0$, the same ranking function is generated, i.e, $r_{f_2} = r_{f_1}$. This time, we get a counter-example $c_2 = (1,-1,-1,4)$. 

% \textbf{2 Refine Step. }Using the counter-example $c_2$, we refine the invariant to $\invar_2 = (y+1\geq z) \wedge (y+1\leq z)$. Again, $r_{f_2} = r_{f_1}$

% \textbf{3 Generation Step. }Again the same ranking function is generated, i.e., $r_{f_3} = r_{f_2}$. This time we get a counter-example, $c_3 = (1,-1,0,4)$. 

% \textbf{3 Refine Step. }Using the counter-example $c_3$, we first try to refine the invariant. However, in this case, we are not able to refine it any further, i.e., $\invar_3 = \invar_2$. So, we add the counter-example to the set of reachable states, i.e., $\rp_3 = \rp_2 \cup \{c_3\} = \{(1,2,3,4), (2,2,3,4),(1,-1,0,4)\}$. 

% \textbf{4 Generation step. }Using $\rp_3$, we generate a new ranking function, we get $r_{f_4} = \max(n-x+1,0) + \max(1-x-y, 0)$. This is valid w.r.t the invariant $\invar_3$. So, we have found the ranking function and the corresponding invariant that can prove the termination of the given program. 

\subsection{Nested Loops}
\ggnds{some more details}

% \avcom{maybe show for only one nested loop first and then generalise to any number of nestings}

% For a doubly-nested loop program with loops $L_{in}$ and $L_{out}$,  we first use our algorithm to find the ranking function ($r_{fin}$) and an invariant ($I_{in}$) that proves the ranking function. We then use $I_{in}$ to model the inner loop and define the program transitions for $L_{out}$. Then, we try to find a pair of invariants ($I_{out}, I_{in}$) that over-approximates the reachable states of the outer loop.


\begin{figure}
\label{fig:nest}

\begin{lstlisting}[language=TeX, mathescape=true, numbers=left]
y = 2
z = 3
while (y + n + 1 $\geq$ $k^2$ + z) {
    while (x + y $\geq$ 0 && x $\leq$ n) {
        x = 2 * x + y;
        y = z;
        z = z + 1; 
    }
    y++;
    z++;
    n--;
}
\end{lstlisting}
% \caption{A nested loop}
\end{figure}
\ggnds{beautify the figure!}


\begin{table}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c||c|c|}
    \hline 
         &$r^+$ & $(\invar_o, \invar_i)$ & $\rf$ & $c$  \\
         \hline
         1&$\{(2, 3,4,4,1), (2,3,4,4,2)\}$ & $(\true, y+1=z)$ & $\max(n-k,0)$ & $(1,2,4,5,5)$ \\  
         \hline 
         2&$\{(2,3,4,4,1), (2,3,4,4,2)\}$ & $(\textcolor{blue}{y+1\geq z}, y+1=z)$ & $\max(n-k,0)$ & $(1,2,2,5,5)$ \\ 
         \hline 
         3&$\{(2,3,4,4,1), (2,3,4,4,2)\}$ & $(\textcolor{blue}{(y+1\geq z) \wedge (y+1\leq z)},y+1=z)$ & $\max(n-k,0)$ & $(1,2,3,5,5)$ \\  
         \hline
         4&$\{(2,3,4,4,1), (2,3,4,4,2), \textcolor{blue}{(1,2,3,5,5)} \}$&$(y+1=z,y+1=z)$& $\textcolor{blue}{\max(n-k+1,0)}$ & -   \\
         \hline 
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:overview}
\end{table}

Consider a nested loop as shown in Figure~\ref{fig:nest}. 
%Let the outer loop be $L_o$ and the inner loop be $L_i$. 
To prove its termination, our algorithm first finds a ranking function $r_{f_i}$ (and an invariant $\invar_{i}$ that proves its validity) for the inner loop. It then uses the $\invar_{i}$ to over-approximate the program transitions ($\trans$) and the set of reachable states of the inner loop. We also maintain an invariant for the outer loop $\invar_{o}$ (initially set to $\true$). Together, $\invar_{o}$ and $\invar_{i}$ over-approximate the state transition relation of the complete program. At each step of our algorithm, we find a candidate ranking function $r_{f_o}$ that reduces on the traces of the outer loop ($\rp$) (using Equation~\ref{eq:rfcreate}) and then check its validity with respect to the pair of invariants $\{I_i, I_o\}$ using the query:
\begin{equation}
\label{eq:checkrfnested}
    \forall X \in \invar_o, \forall X' \in \trans(X) \cdot \rf(X) - \rf(X') \geq 1
\end{equation}
where $\trans(X)$ is modelled over-approximately using the pair of invariants ($\invar_{o}$, $\invar_{i}$) \sgcom{make clear when you are clear} 

If the check succeeds, it means that the generated candidate ranking function was correct and the algorithm terminates. Else, we use the generated counter-example $c$ to refine our state, i.e. we either refine the pair of invariants $\{I_i, I_o\}$ simultaneously \sgcom{give definition or better intuition of simultaneous refine} to exclude $c$ or add $c$ to $\rp$ if the refine fails.

For the program in Fig. \ref{fig:nest}, our algorithm first finds a ranking function $r_{f_i}$ and an invariant $\invar_{i}$ for the inner loop. Note that the inner loop is the same as our previous example (Fig\ref{fig:overview:code3}), and so we get $r_{f_i} = \max(n-x+1,0) + \max(1-x-y, 0)$ and the invariant $\invar_{i} =  (y+1\geq z) \wedge (y+1\leq z) \equiv (y+1=z)$. Now, to find a ranking function for the outer loop, our algorithm steps through the following iterations: \sgcom{Link the desc to the table}

\begin{enumerate}
    \item \textbf{Generate Phase \RNum{1}:} We get a candidate ranking function $r_{f_o} = \max(n-k,0)$ that reduces on all states in $\rp = \{(2, 3,4,4,1), (2,3,4,4,2)\}$. Then we check its validity with respect to the current pair of invariants $\{\true, y+1=z\}$ (using Equation~\ref{eq:checkrfnested}) to find a counter-example $c_1 = (1,2,4,5,5)$.
    \item \textbf{Refine Phase \RNum{1}:} As we got a counter-example ($c_1 = (1,2,4,5,5)$) in our generate phase, we try to refine our pair of invariants $\{\true, y+1=z\}$ to exclude this (as described above). This refinement succeeds, and we get a new pair of valid invariants $\{y + 1 \geq z, y+1=z\}$ which excludes our counter-example $c_1$ (also proving that the counter-example was unreachable and thus spurious).
    \item \textbf{Generate Phase \RNum{2}:} As $\rp$ is same as Phase \RNum{1}, the algorithm again generates the same function $r_{f_o} = \max(n-k,0)$. But we now check its validity with respect to the new pair of invariants $\{y + 1 \geq z, y+1=z\}$ and get a new counter-example $c_2 = (1,2,2,5,5)$.
    \item \textbf{Refine Phase \RNum{2}:} As we got a counter-example ($c_2 = (1,2,2,5,5)$) in our generate phase, we try to refine our pair of invariants $\{y + 1 \geq z, y+1=z\}$ to exclude this. This refinement succeeds, and we get a new pair of valid invariants $\{y + 1 \geq z \wedge y + 1 \leq z, y+1=z\}$ which excludes our counter-example $c_2$.
    \item \textbf{Generate Phase \RNum{3}:} As $\rp$ is same as Phase \RNum{1}, the algorithm again generates the same function $r_{f_o} = \max(n-k,0)$. But we now check its validity with respect to the new pair of invariants $\{y + 1 \geq z \wedge y + 1 \leq z, y+1=z\}$ and get a new counter-example $c_3 = (1,2,3,5,5)$.
    \item \textbf{Refine Phase \RNum{3}:} As we got a counter-example ($c_3 = (1,2,3,5,5)$) in our generate phase, we try to refine our pair of invariants $\{y + 1 \geq z \wedge y + 1 \leq z, y+1=z\}$ to exclude this. This refinement fails, proving that this counter-example is reachable (and thus not spurious). So, we add $c_3$ to our set of reachable states $\rp$.
    \item \textbf{Generate Phase \RNum{4}:} As the set $\rp$ got updated, we get a new candidate ranking function $r_{f_o} = \max(n-k+1,0)$ that reduces on all states in $\rp$. Then we check its validity with respect to the current pair of invariants $\{y + 1 \geq z \wedge y + 1 \leq z, y+1=z\}$. The validity check succeeds, and $r_{f_o} = \max(n-k+1,0)$ is returned as a valid ranking function for the outer loop.
\end{enumerate}

The approach described above can be generalized to any number of nestings. Say the program has $n$ nested loops $L_1, L_2, \cdots L_n$.  Our algorithm starts with the innermost loop $L_n$ and finds a ranking function and an invariant ($I_n$) that validates it. We then shift to loop $L_{n-1}$. In general, to prove the termination of loop $L_i$, we maintain a set of invariants $\{I_i, I_{i+1}, \cdots I_n \}$ (one for each loop inside 
 and including $L_i$) that over-approximates the program transitions ($\trans$) and the set of reachable states of $L_i$. Then we iteratively try to find a ranking function ($\rf$) from the traces of this loop and keep refining the set of invariants $\{I_i, I_{i+1}, \cdots I_n \}$ \avcom{set?} until we find a ranking function $r_f$ and the set of invariants that can prove the termination of this loop. This is inductively done for all the loops till $L_1$. 

==> sections/preliminaries.tex <==
\section{Preliminaries}
% \section{Definitions}

\label{sec:background}

% We introduce basic definitions and notations that will be used in the rest of the paper.

\myparagraph{Relations} For a pair of binary relations $R_1 \subseteq A \times B$ and $R_2 \subseteq B \times C$, their \emph{composition} is the relation $R_1\relcomp R_2 = \setpred{(a,c)}{\exists b \in B.\ (a,b) \in R_1 \text{ and } (b,c) \in R_2} \subseteq A \times C$. For a set $S \subseteq A$ and a binary relation $R \subseteq A \times B$, $S \relcomp R = \setpred{b \in B}{\exists a \in S.\ (a,b) \in R}$ denotes the \emph{image} of $S$ under $R$. Finally, for a set $A$, the \emph{identity relation} on $A$ is denoted as $\id{A} = \setpred{(a,a)}{a \in A}$.

\myparagraph{While Programs} To illustrate our synergistic synthesis approach, we will consider programs in a simple while programming language whose BNF grammar is given below. In what follows, $x$ is a program variable, $e$ a program expression and $\beta$ a Boolean expression. The syntax of expressions is not given as it is not important to the main ideas of this paper. 
\[
\begin{array}{rcl}
\pro & ::= & \texttt{skip}\ |\ x \leftarrow e\ |\ \pro\:\text{;}\:\pro\ |\ \texttt{if } \beta \texttt{ then } \pro \texttt{ else } \pro\ |\ \texttt{while } \beta \texttt{ do } \pro \texttt{ od} 
\end{array}
\]
A \emph{loop-free} program code is one that does not have any {\tt while}-loops. We will typically use $\pgm,\pgm_1,\pgm_2,\ldots$ to denote programs, $\loopfree,\loopfree_1,\ldots$ to denote loop-free programs, and $\looppgm,\looppgm_1,\ldots$ to denote loops, i.e., programs of the form $\texttt{while } \beta \texttt{ do } \pgm \text{ od}$. Towards defining the semantics for a program $\pgm$, it is useful to introduce the notion of a program state. A \emph{program state} $s$ of $\pgm$ assigns values to each variable of $\pgm$. The set of program states of $\pgm$ will be denoted as $\stat_{\pgm}$. When the program $\pgm$ is clear from the context, we will abuse notation and simply use $\stat$ to denote all possible program states of $\pgm$, which is represented by the invariant $\invar_{\true}$. The semantics of a program $\pgm$ denoted $\bracs{\pgm}$, is a binary relation on $\stat$ that captures how a program state is transformed when $\pgm$ is executed. Assuming standard expressions and their semantics, one can naturally define the semantics of loop-free programs. Loops present a challenge.
% We will use \emph{invariants} to over-approximate their semantics. This is also the reason why we will use relational semantics, as opposed to partial functions.

\myparagraph{Ranking Functions} A ranking function is a real-valued function $\rf$ on the program states that is bounded from below and decreases by a minimum amount in every iteration of the loop. For such a ranking function $\rf$ to be a valid witness for termination, $\rf$ is only required to have these properties on the reachable states (or an over-approximation of the reachable states) of the program rather than all the program states.



==> sections/proofs.tex <==
~\\
\hrule
\hrule

\section{Theorems and proofs}

\begin{definition}
    A program $\mathcal{P}$ is a \textit{loop-program} if $\mathcal{P}$ is of the form 
    $$\mathcal{P} \equiv \mathtt{while}(B) \ \mathtt{do} \ \mathcal{P}' \ \mathtt{od}$$
\end{definition}

\begin{definition}
    For a \lp \ $\prog$ and a set of initial states  $\ini$, $\reach$ is the smallest set that satisfies the following conditions:
    \begin{enumerate}
        \item $\ini \subseteq \reach$
        \item For every $X \in \reach \cdot B(X) \implies (\prog'(X) \in \reach)$
    \end{enumerate}
\end{definition}

\begin{definition}
    For a given \lp \ $\prog$ and initial states \ini, a set of states $\invar$ is a valid invariant if:
    \begin{enumerate}
        \item $\reach(\ini, \prog) \subseteq \invar$
        \item $\forall X \in \invar \cdot B(X) \implies (\prog'(X) \in \invar)$
    \end{enumerate}
\end{definition}

\begin{definition}
    For a given loop-program $\mathcal{P}$ and initial states \ini, a function $f:\mathbb{R}^m \rightarrow \mathbb{R}$ is a valid ranking function if 
    \begin{enumerate}
        \item $\exists \delta > 0 \in \mathbb{R}$ such that $\forall X \in \mathcal{R} \cdot B(X) \implies f(X) - f(\mathcal{P'}(X)) \geq \delta$
        \item $\exists \theta \in \mathbb{R}$ such that $\forall X \in \mathcal{R} \cdot B(X) \implies f(X) \geq \theta$
    \end{enumerate}
\end{definition}

\begin{lemma}
    If $f$ is a valid ranking function, then we can construct another valid ranking function $f'$ such that
    \begin{enumerate}
        \item $\forall X \in \mathcal{R} \cdot B(X) \implies f(X) - f(\mathcal{P'}(X)) \geq 1$
        \item $\forall X \in \mathcal{R} \cdot B(X) \implies f(X) \geq 0$
    \end{enumerate}
\end{lemma}
\begin{proof}
    $f'(X) = (f(X) - \theta) / \delta$
\end{proof}

\begin{definition}
    An invariant template $\tempi$ is a given set of candidate invariants.
\end{definition}

\begin{definition}
    A ranking function template $\tempr$ is a given set of candidate ranking functions.
\end{definition}

\sgcom{Add a note that from now on, it is implicit that we are searching for ranking functions and invariants only from the templates.}

\begin{definition}
    \label{def:rp}
    Given $\tempi$, $\reachp$ is the set of states $X$ such that for all valid invariants $\invar \in \tempi \cdot X \in \invar$.
\end{definition}

\begin{lemma}
    $\reach \subseteq \reachp$
\end{lemma}
\begin{proof}
    For any valid invariant $\invar$, $\reach \subseteq \invar$. Consider any state $x \in \reach$. $x \in \invar$ holds for all possible valid invariants. So, $x \in \invar$ also holds for all possible valid invariants in $\tempi$. From the definition of $\reachp$ (Def. \ref{def:rp}), this means that $x \in \reachp$. Therefore, $\reach \subseteq \reachp$.
\end{proof}



% \begin{definition}
%     $\checkr(f, \invar) = \true$ iff
%     \begin{enumerate}
%         \item $\exists \delta \in \mathbb{R}$ such that $\forall X \in \invar \cdot B(X) \implies f(X) - f(\mathcal{P'}(X)) \geq \delta$
%         \item $\exists \theta \in \mathbb{R}$ such that $\forall X \in \invar \cdot B(X) \implies f(X) \geq \theta$
%     \end{enumerate}
% \end{definition}
% --------- Algorithm ------------------------
\section{Algorithm}
\begin{algorithmic}[1]
\Procedure{$\fr$}{$\rp, \invar$}
    \State $f \gets \gc(\rp)$
    \If{$\checkr(f, \invar)$} 
        \State \Return f
    \Else
        % \State $c \gets \gcounter(f, \invar)$
        % \State $\invar' \gets \invar$
        % \State $c' \gets c$
        \While{$\true$}
            \State $c \gets \gcounter(f, \invar)$
            \State $\text{is\_refined}, \; \invar \gets \mathsf{refine}(\invar, c)$
            \If{$\text{is\_refined}$}
                \If{$\checkr(f, \invar)$} 
                    \State \Return f
                % \Else 
                %     \State $c \gets \gcounter(f, \invar')$
                \EndIf
            \Else
                \State $\rp_{new} \gets \rp \cup \{c\}$
                \State $\fr(\rp_{new}, \; \invar)$ 
            \EndIf
            
            
        \EndWhile
    \EndIf 
\EndProcedure
\end{algorithmic}

The above algorithm takes two inputs: (1) a set of states $\rp$ and (2) a valid invariant $\invar$. At line number 2, we generate a possible candidate for ranking function from $\tempr$ that is positive on $\rp$ and reduces by 1 on $\rp$. At line 3, the call to $\checkr$ checks if this ranking function is valid w.r.t $\invar$. If it is valid, it is returned, and the algorithm stops. If the ranking function is not valid, we get a counterexample ($c$) (Line 7), which is a state present in $\invar$ on which the proposed ranking function $f$ does not decrease by 1. Now, we try to find an invariant that can exclude this counter-example. This is done by the call to Refine at line 8. If $\isref$ is True, it means that the returned invariant $\invar$ is refined to exclude the counter-example $c$. In this case, we again check the validity of our proposed ranking function with this new invariant (call to $\checkr$ at Line 10). If the check passes, we return the function. Else, we go into the next iteration of the while loop, get the new counter-example, and again try to refine the invariant to exclude this new counter-example. We keep doing this until either $\checkr$ for this $f$ passes at Line 10, or $\isref$ comes out as False at Line 8. If $\isref$ comes out as False at any time in the loop, we add our latest counter-example to the set $\rp$ and call the $\mathsf{find\_ranking}$ function again with the updated $\rp$ set ($\rp_{new}$) and the latest invariant found ($\invar$).

\begin{definition}
    A ranking function is valid w.r.t $\invar$ or $\checkr(f, \invar) = \true$ iff
    \begin{enumerate}
        \item $\forall X \in \invar \cdot B(X) \implies f(X) - f(\mathcal{P'}(X)) \geq 1$
        \item $\forall X \in \invar \cdot B(X) \implies f(X) \geq 0$
    \end{enumerate}
    \sgcom{Add something to say that this modified definition (using 1 as diff and 0 as bounds) is what we are enforcing and is not a general requirement.}
\end{definition}


\begin{corollary} If 
    \begin{enumerate}
        \item $\invar$ is a valid invariant
        \item $\checkr(f, \invar) = \true$
    \end{enumerate}
    Then, $f$ is a valid ranking function.
\end{corollary}

\begin{definition}
    \label{def:wrttempi}
    A function $f$ is a valid ranking function w.r.t $\tempi$ if there is a valid invariant $\invar \in \tempi$ such that $\checkr(f, \invar) = \true$
\end{definition}

\begin{definition}
    \label{def:invalidf}
    A function $f$ is an invalid ranking function w.r.t $\tempi$ if there is no valid invariant $\invar \in \tempi$ such that $\checkr(f, \invar) = \true$
\end{definition}

\begin{definition}
    \label{def:refine}
    $\text{is\_refined}, \; \invar' = \mathsf{Refine(\invar, c)}$ has the following semantics:
    \begin{enumerate}
        \item If $\text{is\_refined}$ is True, it means the returned invariant ($\invar' \in \tempi$) is valid, is a proper subset of the specified invariant $\invar$ and excludes the counter-example $c$. That is:
        \begin{enumerate}
            \item $c \not\in \invar''$
            \item $\invar'' \subset \invar$
        \end{enumerate}

         \item If $\text{is\_refined}$ is False, there is no valid invariant in our template $\tempi$ which is a proper subset of $\invar$ and excludes the counter-example $c$. In this case, the returned invariant $\invar'$ is just the original $\invar$.
    \end{enumerate}
\end{definition}
%=====================================================

% ----------------- Refine gives stronger ------------
\begin{lemma}
    \label{lem:refine}
    If
    \begin{enumerate}
        \item $f$ is a valid ranking function w.r.t $\tempi$.
        \item $\invar, \invar' \in \tempi$ are valid invariants. 
        \item $c$ is a counter-example from $\gcounter(f, \invar)$.
        \item $\checkr(f, \invar') = \true$
        \item $\invar' \subset \invar$
    \end{enumerate}
    Then
    \begin{enumerate}[label=\Alph*]
        \item $\mathsf{refine}(\invar, c) = true, \; \invar''$
        \item $c \not\in \invar''$
        \item $\invar'' \subset \invar$
    \end{enumerate}
\end{lemma}

\begin{proof}
From (3), it follows that ($(f(c) - f(\prog'(c)) < 1)$ or $(f(c) < 0)$) and $c \in \invar$. Further, from (4) $\checkr(f, \invar') = \true$. So, we can conclude that $c \notin \invar'$. So, our template has a valid invariant ($\invar'$) such as $c \notin \invar'$ and $\invar' \subset \invar$ (given (5)). This means that our call to $\mathsf{refine}(\invar, c, \tempi)$ will not be unsat and $\isref$ will be True (from the semantics of refine in Def. \ref{def:refine}). Also. the returned refined invariant $\invar''$ will follow (B) and (C) from the semantics of refine.
\end{proof}

\begin{lemma}
    \label{lem:existsabove}
    If 
    \begin{enumerate}
        % \item $\tempi$ is closed under intersection.
        % \item $\tempi$ is a finite set.
        \item $\tempi$ is closed under intersection
        \item $\invar, \invar^* \in \tempi$ are valid
        \item $\checkr(f, \invar^*) = \true$.
    \end{enumerate}
    Then $\invar' = \invar \cap \invar^*$ satisfies the following
    \begin{enumerate}[label=\Alph*]
        \item $\invar' \in \tempi$
        \item $\invar'$ is valid.
        \item $\checkr(f, \invar') = \true$
    \end{enumerate}
\end{lemma}
\begin{proof}
    (A) follows from assumption (1) that $\tempi$ is closed under intersection. \\ \\
    From (2), $\reach \subseteq \invar$ and $\reach \subseteq \invar^*$. So, $\reach \subseteq \invar'$ \\ \\
    Since $\invar$ is valid, $\forall X \in \invar,  B(X) \implies \prog'(X) \in \invar$ \\ 
    Since $\invar' \subseteq \invar$, $\forall X \in \invar',  B(X) \implies \prog'(X) \in \invar \qquad (a)$ \\ \\
    Similarly, $\invar^*$ is valid, $\forall X \in \invar,  B(X) \implies \prog'(X) \in \invar^*$ \\ 
    Since $\invar' \subseteq \invar^*$, $\forall X \in \invar',  B(X) \implies \prog'(X) \in \invar^*  \qquad (b)$ \\ \\
    From (a) and (b), $\forall X \in \invar',  B(X) \implies \prog'(X) \in \invar' \qquad \cdots$ (B) \\ \\
    From (3), $\forall X \in \invar^* \cdot B(X) \implies f(X) \geq 1$ \\ 
    and $\forall X \in \invar^* \cdot B(X) \implies f(X) - f(\prog'(X)) \geq 0$ \\
    Also, $\invar' \subseteq \invar^*$ \\ 
    So, $\forall X \in \invar' \cdot B(X) \implies f(X) \geq 1$ \\ 
    $\forall X \in \invar' \cdot B(X) \implies f(X) - f(\prog'(X)) \geq 0 \qquad \cdots$ (C)
\end{proof}

%================================================

%------------ Lattice Definitions ---------------
\section{Lattice of invariants induced by $\tempi$}

Define a meet semi-lattice $\lati = (\tempi, \preceq, \wedge)$, where $\invar_1 \preceq \invar_2$ iff $\invar_1 \subseteq \invar_2$ and $\invar_1 \wedge \invar_2 \equiv \invar_1 \cap \invar_2$.
% Our template $\tempi$ always follows these constraints:
% \begin{enumerate}
%     \item $\tempi$ is closed under intersection.
%     \item $\tempi$ is a finite set.
%     \item $\{\} \in \tempi$
% \end{enumerate}
% From (2), we can infer that the our lattice $\lati$ is a finite lattice.


 \textbf{Observation:} Our algorithm (defined above) always has a current invariant $\invar$ that it is considering. The loop at Line 6 tries to refine it by calling $\mathsf{Refine}(\invar, c)$ at line 8. If the call to $\mathsf{Refine}$ succeeds, the returned invariant $\invar'$ is a strict subset of $\invar$ ($\invar' \subset \invar$ from the semantics of $\mathsf{Refine}$ (\ref{def:refine})). This means each successful call to $\mathsf{Refine}$ (which actually refines our invariant) takes us down in our lattice $\lati$, i.e. $\invar' \prec \invar$ (from the definition of our lattice and the fact that $\invar' \subset \invar$). We stop if we find an invariant that proves our proposed ranking function $f$ correct (the $\checkr$ at line 10 passes) or we can not refine our invariant further ($\text{is\_refined}$ is false at line 8).
 
\begin{lemma}
\label{lemma:whileterminate}
If $\tempi$ is a finite set, then the while loop at Line 6 terminates.
\end{lemma}
\begin{proof}
If $\tempi$ is a finite set, it follows that:
    \begin{equation}
        \lati \text{ has finite depth}
    \end{equation}
Now, at any iteration of the loop, consider the following two cases:
\begin{enumerate}
    \item $\text{is\_refined}$ is False at Line 8: The control goes to the else case (Line 14), which calls the $\fr$ function again, and the loop terminates.
    \item $\text{is\_refined}$ is True at Line 8: This means that our invariant was refined and say we got a new invariant $\invar'$. If this new invariant satisfies the call to $\checkr$ at Line 10, the loop terminates. If not, then we enter the next iteration of the loop, generate a new counter-example $c$ (Line 7) and call $\mathsf{Refine}$ again. As stated in the observation above, with every call to $\mathsf{Refine}$, we move down the invariant lattice $\lati$. And from (1) above, $\lati$ has finite depth. This shows that the number of times $\mathsf{Refine}$ can succeed is bounded (by the depth of the lattice), and the loop will either terminate when $\checkr$ returns True at some invariant or will always hit a point where $\text{is\_refined}$ is False. Thus, the loop always terminates.
    
\end{enumerate}
\end{proof}

\begin{lemma}
\label{lem:correctinv}
If 
    \begin{enumerate}
        \item $\tempi$ is closed under intersection.
        \item $\tempi$ is a finite set.
        \item $\{\} \in \tempi$ \sgcom{Not sure why is this here}
        \item $f$ is a valid ranking function w.r.t $\tempi$ 
        \item $\invar \in \tempi$ is a valid invariant.
    \end{enumerate}
then, the while loop (starting at Line 6) will always find a valid invariant $\hat{\invar}$ such that:
\begin{enumerate}[label=(\alph*)]
    \item $\hat{\invar} \subseteq \invar$
    \item $\hat\invar \in \tempi$
    \item $\checkr(f, \hat{\invar}) = \true$
\end{enumerate}
That is, in this case, while always terminates by returning $f$ at Line 11 and never by going in the else block starting at Line 14.
\end{lemma}
\begin{proof}
    From (4) and Def. \ref{def:wrttempi}, there exists a valid invariant $\invar^{*}$ such that $\checkr(f, \invar^{*})$ = true.\\
    From (2) and Lemma \ref{lemma:whileterminate}, we know that the while loop always terminates. \\
    As established above, the while (starting from the invariant $\invar$) keeps refining the invariant (or moving down the lattice) until it terminates.
    There are two ways it could terminate:

    \begin{enumerate}
        \item Call to $\checkr(f, \invar')$ succeeds at Line 10 for some $\invar'$: This means that we have found a valid invariant $\hat{\invar} = \invar'$.
        Now:
        \begin{enumerate}[label=(\alph*)]
            \item $\invar' \subseteq \invar$ holds from semantics of $\mathsf{Refine}$ (Def. \ref{def:refine}).
            \item $\invar' \in \tempi$ holds from semantics of $\mathsf{Refine}$ (Def. \ref{def:refine}).
            \item $\checkr(f, \invar') = \true$ holds as that is the condition we assume in this case.
        \end{enumerate}
        
        \item $\isref$ is false at Line 8: We will prove this can never happen. 
        
        For this to happen, $\isref$ should return false for some invariant in our path down the lattice. Say there exists an invariant $\invar_l$ and a counter-example $c_l$ for which $\mathsf{Refine(\invar_l, c_l)}$ returns $\isref$ False. From the definition of $\mathsf{Refine}$ (Def. \ref{def:refine}), this means that there is no valid invariant in $\tempi$ which is a subset of $\invar_l$ and does not include $c_l. \qquad \cdots$ (R1)\\
        
        Now, consider the invariant $\invar_e = \invar_l \cap \invar^{*}$. From Lemma \ref{lem:existsabove}, $\invar_e$ is a valid invariant in $\tempi$ such that $\checkr(f, \invar_e)$ = true. Also:
        \begin{itemize}
            \item As $c_l$ was a counter-example, it follows that ($(f(c_l) - f(\prog'(c_l)) < 1)$ or $(f(c_l) < 0)$). But as $\checkr(f, \invar_e)$ = true, it means that $\invar_e$ does not contain $c_l$. So, $c_l \notin \invar_e$.
            \item As $\invar_e = \invar_l \cap \invar^{*}$, $\invar_e \subseteq \invar_l$. Also, as $c_l \in \invar_l$ and $c_l \notin \invar_e$, $\invar_e \subset \invar_l$.
        \end{itemize} 

        This contradicts (R1) as we have found an invariant $\invar_e$, which is a proper subset of $\invar_l$ and does not include $c_l$. Thus, we conclude that this case will never occur ($\isref$ is never false if $f$ is a valid ranking function, and we terminate by proving that it is valid).
    \end{enumerate}

\end{proof}

\begin{lemma}
If 
    \begin{enumerate}
        \item $\tempi$ is a finite set.
        \item $f$ at line 2 is an invalid ranking function w.r.t $\tempi$.
    \end{enumerate}
then, we will always reach line 14.
\end{lemma}
\begin{proof}
    From (1) and Lemma \ref{lemma:whileterminate}, we know that the while loop always terminates. \\
    There are only two ways in which it could terminate:

    \begin{enumerate}[label=(\alph*)]
        \item Call to $\checkr(f, \invar')$ succeeds at Line 10 for some $\invar'$
        \item  $\isref$ is false at Line 8, and the control reaches line 14
    \end{enumerate}

    (a) can never hold as $f$ is an invalid ranking function w.r.t $\tempi$ (Def. \ref{def:invalidf}). This proves that for invalid ranking functions, the algorithm always reaches line 14.
\end{proof}


% ----------------- While terminates ------------
% \begin{lemma}
%     The while loop at line 9 will always terminate.
% \end{lemma}

% \begin{proof}
%     The while loop terminates if the call to Refine (at line 10) returns false or the call to Check (at line 11) returns true. We show that at least one of these will always occur.
    
%     (for the case when f is a valid ranking function)
%     From \ref{lem:refine}, we can infer that a call to Refine with an invariant $\invar$ always generates a new invariant $\invar''$ such that  $\invar'' \subset \invar$.
% \end{proof}
%================================================

% \begin{lemma} 
% (If $f$ is a valid ranking function at line 2, then we will never enter the else case at line 16. That is, we will always find an invariant in our template for which $\checkr(f, \invar) = \true$)
% If 
%     \begin{enumerate}
%         \item $\tempi$ is closed under intersection.
%         \item $\tempi$ is a finite set.
%         \item 
%         \item $f$ is a valid ranking function w.r.t $\tempi$ 
%         \item $\invar \in \tempi$ is a valid invariant.
%     \end{enumerate}
% If $f$ is a valid ranking function w.r.t $\tempi$, then we can find a valid invariant $\hat{\invar}$ such that $\hat{\invar} \subseteq \invar$, $\hat\invar \in \tempi$ and $\checkr(f, \hat{\invar}) = \true$.
% \end{lemma}



% \begin{proof}
%     Define a semi-lattice $\mathcal{L} = (\tempi, \preceq, \vee)$, where $\invar_1 \preceq \invar_2$ iff $\invar_2 \subseteq \invar_1$ and $\invar_1 \vee \invar_2 \equiv \invar_1 \cap \invar_2$. \\ 
%     \begin{equation}
%         \mathcal{L} \text{ has finite height}
%     \end{equation}
%     This follows from the fact that our $\tempi$ is a finite set. 

%     Since $f$ is a valid ranking function w.r.t $\tempi$, from Definition~\ref{def:wrttempi}, there exists a valid invariant $\invar^* \in \tempi$ such that $\checkr(f, \invar^*) = \true$. 
    
%     From Lemma~\ref{lem:existsabove}, it follows that $\invar' = \invar \vee \invar^*$ is a valid invariant. 
%     \begin{equation}
%         \checkr(f, \invar') = \true 
%     \end{equation}
%     This gives the following two cases:
%     \begin{enumerate}
%         \item $\invar = \invar'$. In this case, let $\hat{\invar} = \invar = \invar'$. From (2), $\checkr(f, \hat{\invar}) = \true$
%         \item $\invar \prec \invar'$. From Lemma~\ref{lem:refine}, $\mathsf{refine}(\invar, c) = \invar''$ such that $\invar \prec \invar''$. From (1), height of the lattice $\mathcal{L}$ is finite. So, the loop at line 9 will always terminate, i.e., we can only ascend for a finite steps in the lattice starting from $\invar$.  \\ 
%         Assume that we enter the else case at line 16 of the algorithm. This means that $\mathsf{refine}(\invar', c') = \false$. So, from the contrapositive of Lemma~\ref{lem:refine}, atleast one of the antecedants of the Lemma is false. (1), (2), (3) are correct, and also $\invar'' \subseteq \invar$, so the only possibility is that $\invar'' = \invar$ and $\checkr(f, invar) = \true$. In this case, in the iteration of the while loop at line 9, prior to entering the else case line 16, we would have terminated the loop at line 12. So, by contradiction, if $f$ is a valid ranking function w.r.t $\tempi$, we will always find an invariant in $\tempi$ such that $\checkr(f, \invar) = \true$
%     \end{enumerate}

    
    
% \end{proof}

\begin{lemma}
    $\rp \subseteq \reachp$
\end{lemma}
\begin{proof} Initially, $\rp$ has elements from trace only
    \begin{enumerate}
        \item $\reach \subseteq \reachp$
        \item $\mathsf{trace} \subseteq \reach$
        \item $\rp \subseteq \mathsf{traces}$
        \item $\therefore, \rp \subseteq \reachp$
    \end{enumerate}
    Then, as the algorithm proceeds, we add the latest counter-example $c$ to the set $\rp$ (Line 14). If we have reached line 14, it means that $\mathsf{Refine}(\invar, c)$ was False at Line 8. We claim that there $c \in \reachp$. Say this is not the case. Then, there must exist a valid invariant $\invar' \in \tempi$ such that $c \notin \invar'$ (From the definition of $\reachp$: Def \ref{def:rp}). Consider $\invar'' = \invar \cap \invar'$ which is a valid invariant (as $\tempi$ is closed under intersection \sgcom{add as assumption above?}). $\invar''$ does not contain $c$ as $c \notin \invar'$. $\invar'' = \invar \cap \invar'$ implies $\invar'' \subseteq \invar$. And $\invar'' \neq \invar$ as $c \notin \invar''$ but $c \in \invar$. So, $\invar'' \subset \invar$. So, we have an invariant $\invar''$ such that $\invar'' \subset \invar$ and $c \notin \invar''$. This contradicts the fact that  $\mathsf{Refine}(\invar, c)$ was False at Line 8 (from semantics of $\mathsf{Refine}$ in Def. \ref{def:refine}). This proves that $c$ is indeed in $\reachp$ and so all points that we add in $\rp$ are in $\reachp$. This proves that $\rp \subseteq \reachp$.
\end{proof}

% \begin{definition}
    
% \end{definition}


\begin{theorem}
    If there exists a function $f \in \tempr$, such that $f$ is a valid ranking function w.r.t $\tempi$, then our algorithm will always find a function $f' \in \tempr$ such that $f'$ is a valid ranking function w.r.t $\tempi$ 
\end{theorem}

\begin{proof}
    Define a meet semi-lattice on the powerset of all possible ranking functions in $\tempr$: $\latrfs = (\mathcal{P} ({\tempr})\preceq, \wedge)$, where $\mathcal{F}_1 \preceq \mathcal{F}_2$ iff $\mathcal{F}_1 \subseteq \mathcal{F}_2$ and $\mathcal{F}_1 \wedge \mathcal{F}_2 \equiv \mathcal{F}_1 \cap \mathcal{F}_2$. From the theorem statement, there exists a $f^* \in \tempr$, such that $f^*$ is a valid ranking function w.r.t $\tempi$. $f^*$ being a valid ranking function w.r.t $\tempi$ means that there is a valid invariant $\invar^* \in \tempi$ such that $\checkr(f^*, \invar^*)$ is true. At the ith iteration of our algorithm, we have a set $r_i^+$. Now, let $F_i = F(r_i^+)$ be the set of all ranking functions that decrease by 1 on all elements of $r_i^+$ and is also bounded below by 0. Since for all i, $r_i^+ \subseteq \reachp$ (above lemma), $f^* \in F_i$. This is because as $\invar^*$ is a valid invariant, $\reachp \subseteq \invar^*$ (by Def. \ref{def:rp}), which means $r_i^+ \subseteq \invar^*$ and so $f^* \in F_i$ as $\checkr(f^*, \invar^*)$ is true.

    From the algorithm, $r_i^+ \subset r_{i+1}^+$, $F_{i+1} \subset F_i$. Now, since our lattice $\mathcal{L}$ has a finite depth (because the set $\tempr$ is finite \sgcom{add this as an assumption for the theorem?}), the algorithm must terminate. From the algorithm, it can terminate in the following two cases:
    \begin{enumerate}
        \item A correct ranking function was found, which proves the theorem.
        \item At line 2, $F(r_i^+) = \{\}$. This is not possible as $f^*$ is always a member of $F(r_i^+)$.
    \end{enumerate}
    This proves our theorem.
\end{proof}

\hrule

\section{Nested loops}
Double loop program:
\begin{align*}
    \mathcal{P} \equiv \mathtt{while} & (B_o) \ \mathtt{do} \\ 
    & f_1 \\ 
    & \mathtt{while}(B_i) \ \mathtt{do} \\ 
    & \quad f_2 \\ 
    & \mathtt{od} \\ 
    f_3 \\ 
    \mathtt{od}
\end{align*}
% \noindent
$$\checkr(f, (I_o, I_i)) \equiv \forall x_1, x_2 \cdot B_o(x_1) \wedge I_o(x_1) \wedge \neg B_i(x_2) \wedge I_i(x_2)  \wedge I_i(f_1(x_1)) \implies f(x_1) - f(f_3(x_2)) \geq 1$$

Given a program $P$ and $Init$, Correctness of a pair of invariants $(I_o, I_i)$: 
\begin{enumerate}
    \item $Init \subseteq \invar_0$ holds (init property for outer invariant)
    \item $\forall x. \; (\invar_o(x) \wedge \mathsf{B}_o(x)) \implies \invar_i(f_1(x))$ (init property for inner invariant)
    \item $\forall x. \; (\invar_i(x) \wedge \mathsf{B}_i(x)) \implies \invar_i(f_2(x))$ (inductive property for inner invariant)
    \item $\forall x. \; (\invar_i(x) \wedge \neg \mathsf{B}_i(x)) \implies \invar_o(f_3(x))$ (inductive property for outer invariant)
\end{enumerate}
% \\
If $(I_o, I_i)$ and $(I'_o, I'_i)$ are valid invariants, then $(I_o \cap I_o', I_i \cap I_i')$ is also valid invariant.
\\ \\
\noindent 
Given all valid invariants $(I_o, I_i)$, the set of reachable states is $\reach = (\bigcap I_o, \bigcap I_i)$ \\ 
Given all valid invariants $(I_o, I_i)$ such that all $I_o \in \tempi$ and $I_i \in \tempi'$, the set of reachable states is $\reachp = (\bigcap I_o, \bigcap I_i)$

A counter-example of the above query: we get $c_1, c_2$ - for $x_1, x_2$ respectively.

Two possibilities:
\begin{enumerate}
    \item $\mathsf{refine}(I_o, c_1) = I_o'$ such that $I'_o \subseteq I_o \setminus \{c_1\}$ and $I_o'$ is a valid outer invariant.
    \item $\mathsf{refine}(I_i, c_2) = I_i'$ such that $I'_i \subseteq I_i \setminus \{c_2\}$ and $I_i'$ is a valid inner invariant.
\end{enumerate}
But these are not exhaustive possibilities. It may not be possible to refine either invariant by keeping the other constant. So, we need to run a common refine:
$\mathsf{refine}((I_o, I_i), (c_1, C_2)) = (I_o', I_i')$ such that
\begin{enumerate}
    \item $I_o' \subseteq I_o \setminus \{c_1\} \vee I_i' \subseteq I_i \setminus \{c_2\}$
    \item $I_o' \subseteq I_o$
    \item $I_i' \subseteq I_i$
    \item $(I_o', I_i')$ is a valid invariant
\end{enumerate}
Now we can claim that if we were not able to refine the invariants, the counter-example $(c_1, c_2)$ was reachable.
SMT query for the above refine:\\
$\exists I_o', I_i', \forall x_1, x_2$ such that the following are true:
\begin{enumerate}
    \item $x_1 \in Init \implies x_1 \in I_o'$
    \item $I'_o(x_1) \wedge B_o(x_1) \implies I'_i(f_1(x_1)))$
    \item $I'_i(x_2) \wedge \neg B_i(x_2) \implies I'_o(f_3(x_2))$
    \item $I'_i(x_2) \wedge B_i(x_2) \implies I'_i(f_2(x_2))$
    \item $\neg I'_o(c_1) \vee \neg I'_i(c_2)$
\end{enumerate}


Now we can state and prove all the three lemmas:
\begin{definition}
    An element of the lattice is a pair $(I_o, I_i)$. \\ 
    $(I_o, I_i) \preceq (I_o', I_i') \equiv (I_o \subseteq I_o' \wedge I_i \subseteq I_i')$ \\
    $(I_o, I_i) \wedge (I_o', I_i') \equiv (I_o \cap I_o', I_i \cap I_i')$
\end{definition}

\begin{lemma}
    If the ranking function is correct, we will eventually find a correct pair of invariants.
\end{lemma}
\begin{proof}
    \begin{enumerate}
        \item We keep going down the lattice, and this process terminates 
        \item At each point in the lattice, we have an element lower down in the lattice, which can prove the ranking function.
    \end{enumerate}
\end{proof}

\begin{lemma}
    If the ranking function is incorrect, the counter-example is in $\reachp$
\end{lemma}
\begin{proof}
    From the semantics of refine, it will give false only when there is no pair $(I_o, I_i)$ which can exclude the counter-example when we went down the lattice. We can show from the contrapositive of the previous lemma that there will be no invariant in the whole lattice which can remove $(c_1, c_2)$ and is also a valid invariant. From the definition of $\reachp$, we can say that counter-example is also in $\reachp$.
\end{proof}

\begin{lemma}
    If there is a valid ranking function in $\tempr$, we will eventually find it. 
\end{lemma}
\begin{proof}
    The set $\rp$ always keeps getting bigger. And $\rp \subseteq \reachp$. So, corresponding to $\rp$, the set of all candidate ranking functions $F$ that reduce on $\rp$ is non empty and keeps getting smaller at each iteration. Since there is no infinite descending chain, this will terminate, and the valid ranking function is always an element of $F_i$
\end{proof}

==> sections/tikz-figs/proof.tex <==
\begin{tikzpicture}
    % Draw the oval shape
    \node[ellipse, draw, minimum width=2.5cm, minimum height=4cm, label=below:$\mathcal{L}_\annopgm$] (oval) {};
    
    % Draw the points inside the oval
    \node[circle, fill=black, inner sep=2pt, label=above left:$\annopgm$] at (-0.5,0.5) {};
    \node[circle, fill=black, inner sep=2pt, label=below:$\annopgm'$] at (-0.1, -0.5) {};
    % \node[circle, fill=green!70!black, inner sep=2pt, label=right:$\annopgm^*$] at (0.4, 0.8) {};
    \draw[->, decorate, decoration={snake, amplitude=0.5mm, segment length=5mm}, line width=0.3mm] (-0.5,0.5) -- (-0.15, -0.4);

    \node[ellipse, draw, minimum width=2.5cm, minimum height=4cm, label=below:$\mathcal{L}_\tempr$] (oval) at (3,0) {};

    \node[circle, fill=black, inner sep=2pt, label={above:$\func(\rp,\tempr)$}] at (3.5,0.5) {};
    \node[circle, fill=black, inner sep=2pt, label={below:$\func(\rp_{new},\tempr)$}] at (2.9, -0.5) {};

    \draw[->, decorate, decoration={snake, amplitude=0.5mm, segment length=5mm}, line width=0.3mm] (3.5,0.5) -- (2.9, -0.4);
    % \node[circle, fill=green!70!black, inner sep=2pt, label=below:$\annopgm'$] at (-0.1, -0.5) {};
    % \node[circle, fill=green!70!black, inner sep=2pt, label=right:$\annopgm^*$] at (0.4, 0.8) {};
    % \draw[->, decorate, decoration={snake, amplitude=0.5mm, segment length=5mm}] (-0.5,0.5) -- (-0.15, -0.4);
\end{tikzpicture}

==> sections/tikz.tex <==
% \tikzstyle{process} = [rectangle, 
% minimum width=3cm, 
% minimum height=1cm, 
% text centered, 
% text width=3cm, 
% draw=black, 
% fill=blue!30]

% \tikzstyle{inparrow} = [thick,->,>=stealth]
% \tikzstyle{arrow} = [->,>=stealth]


% \begin{tikzpicture}[node distance=2cm]

% \node (rfg) [process] {Ranking Function Generator};
% \node (rfc) [process, below of=rfg, yshift=-1.5cm] {Ranking Function Verifier};
% \node (ivg) [process, right of=rfc, xshift=4cm] {Invariant Generator};

% \draw [inparrow] (-1,2) -- (rfg);
% \draw [inparrow] (0,2) -- (rfg);
% \draw [inparrow] (1,2) -- (rfg);
% \draw [arrow] (rfg) -- (rfc) node[pos=0.5, right] {$r_f$};
% % \draw [arrow] (ivg) -- (rfg);
% \draw [inparrow] (rfc) -- ++(0,-1.5) node[pos=1, below] {$r_f$};

% \path (rfc) edge[->, bend left] (ivg) node[pos=1, below] {$cex$};
% \path (ivg) edge[->, bend left] (rfc) node[pos=1, below] {$r_f$};

% % \node (start) [startstop] {Start};
% % \node (in1) [io, below of=start] {Input};
% % \node (pro1) [process, below of=in1] {Process 1};
% % \node (dec1) [decision, below of=pro1, yshift=-0.5cm] {Decision 1};

% % \node (pro2a) [process, below of=dec1, yshift=-0.5cm] {Process 2a
% % text text text text
% % text text text 
% % text text text};

% % \node (pro2b) [process, right of=dec1, xshift=2cm] {Process 2b};
% % \node (out1) [io, below of=pro2a] {Output};
% % \node (stop) [startstop, below of=out1] {Stop};

% % \draw [arrow] (start) -- (start);
% % \draw [arrow] (start) -- (in1);
% % \draw [arrow] (in1) -- (pro1);
% % \draw [arrow] (pro1) -- (dec1);
% % \draw [arrow] (dec1) -- node[anchor=east] {yes} (pro2a);
% % \draw [arrow] (dec1) -- node[anchor=south] {no} (pro2b);
% % \draw [arrow] (pro2b) |- (pro1);
% % \draw [arrow] (pro2a) -- (out1);
% % \draw [arrow] (out1) -- (stop);

% \end{tikzpicture}

\begin{table}
    \begin{tabular}{|p{0.35\textwidth}|p{0.6\textwidth}|}
        \hline
        \begin{lstlisting}[numbers=left, basicstyle=\footnotesize]
while (x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = y + 1;
}
        \end{lstlisting}
        &
        \begin{align*}
            \rf(x',y',n') & = \max\big(1-(x'+y'), 0\big) + \max(n - x' + 1, 0) \\
            & = \max\big(-(2x+2y), 0\big) + \max(n-2x-y+1,0) \\
            & = \max\big(n-x+1-(x+y),0\big)
        \end{align*}
        \\
        \hline
        \begin{lstlisting}[numbers=left, basicstyle=\footnotesize]
while (x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = z;
    z = z + 1;
}
        \end{lstlisting}
        &
        \begin{tabular}{|c|c|c|c|c|c|}
            \hline
            $x$ & $y$ & $z$ & $n$ & $(x+y\geq0) \wedge (x\leq n)$ & \text{rf} \\
            \hline
            1 & -1 & -1 & 4 & \text{true} & 5 \\
            1 & -1 & 0 & 4 & \text{true} & 5 \\
            1 & 0 & 1 & 4 & \text{true} & 4 \\
            2 & 1 & 2 & 4 & \text{true} & 3 \\
            5 & 2 & 3 & 4 & \text{false} & - \\
            \hline
        \end{tabular}
        \\
        \hline
        \begin{lstlisting}[numbers=left, basicstyle=\footnotesize]
if(x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = z;
    z = z + 1;
}
while (x + y >= 0 && x <= n) {
    x = 2 * x + y;
    y = z;
    z = z + 1;
}
        \end{lstlisting}
        &
        \begin{align*}
            \rf(x',y',z',n') & = \max\big(1-(x'+y'), 0\big) + \max(n - x' + 1, 0) \\
            & = \max\big(1-2x-y-z, 0\big) + \max(n-2x-y+1,0) \\
            & = \max\big(1-2x-y-(y+1), 0\big) + \max\big(n-x+1-(x+y),0\big) \\
            & = \max(-2x-2y, 0) + \max\big(n-x+1-(x+y),0\big) \\
            & = 0 + \max\big(n-x+1-(x+y),0\big) \\
            & = \max\big(n-x+1-(x+y),0\big)
        \end{align*}
        \\
        \hline
    \end{tabular}
\end{table}

